PRIVEE: A Visual Analytic Workflow for Proactive Privacy Risk Inspection of Open Data

Open data sets that contain personal information are susceptible to adversarial attacks even when anonymized. By performing low-cost joins on multiple datasets with shared attributes, malicious users of open data portals might get access to information that violates individuals' privacy. However, open data sets are primarily published using a release-and-forget model, whereby data owners and custodians have little to no cognizance of these privacy risks. We address this critical gap by developing a visual analytic solution that enables data defenders to gain awareness about the disclosure risks in local, joinable data neighborhoods. The solution is derived through a design study with data privacy researchers, where we initially play the role of a red team and engage in an ethical data hacking exercise based on privacy attack scenarios. We use this problem and domain characterization to develop a set of visual analytic interventions as a defense mechanism and realize them in PRIVEE, a visual risk inspection workflow that acts as a proactive monitor for data defenders. PRIVEE uses a combination of risk scores and associated interactive visualizations to let data defenders explore vulnerable joins and interpret risks at multiple levels of data granularity. We demonstrate how PRIVEE can help emulate the attack strategies and diagnose disclosure risks through two case studies with data privacy experts.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/attack_scenarios_old.tex <==
%\section{Red-Teaming for Conceptualizing Attack Scenarios} \label{section:red_teaming}
\section{Requirement Analysis through Attack Scenario} \label{section:red_teaming}

\kaustav{In Progress}
In order to understand the requirements for addressing the disclosure risks, we decided to conduct a red-team exercise. A red-team exercise can be generally defined as a structured process to better understand the capabilities and vulnerabilities of a system by viewing the problems through the lenses of an adversary\cite{zenko2015red}. 
A red-team exercise can be generally defined as a structured process to better understand the capabilities and vulnerabilities of a system by viewing the problems through the lenses of an adversary\cite{zenko2015red}. In the context of security and privacy, red-team exercises follow the cyber kill chain by playing the role of an ethical hacker and emulating the possible attack scenarios\cite{hutchins2011in%\section{Red-Teaming for Conceptualizing Attack Scenarios} \label{section:red_teaming}
\section{Requirement Analysis through Attack Scenario} \label{section:red_teaming}

\kaustav{In Progress}
In order to understand the requirements for addressing the disclosure risks, we decided to conduct a red-team exercise. A red-team exercise can be generally defined as a structured process to better understand the capabilities and vulnerabilities of a system by viewing the problems through the lenses of an adversary\cite{zenko2015red}. 
A red-team exercise can be generally defined as a structured process to better understand the capabilities and vulnerabilities of a system by viewing the problems through the lenses of an adversary\cite{zenko2015red}. In the context of security and privacy, red-team exercises follow the cyber kill chain by playing the role of an ethical hacker and emulating the possible attack scenarios\cite{hutchins2011intelligence}. With the help of researchers in data privacy and urban informatics, we performed a red-teaming exercise by inspecting the open datasets for vulnerabilities. We engaged in a cold-start exploration process, followed by more focused exploitation of datasets with privacy-relevant attributes, for developing a shared mental model of the problems related to the vulnerabilities. The intuition here was that the datasets with universally known quasi-identifiers, like age, race, gender, etc., can lead to the disclosure of sensitive information when joined with other such datasets. 





\begin{figure*}[t]
\begin{center}
\includegraphics[width=\textwidth]{figures/workflow.pdf}
\vspace{-4mm}
 \caption{\label{figs:PRIVEE}\textbf{PRIVEE is an end-to-end risk inspection workflow for open datasets} that informs the defender in the analytical loop about potential disclosure risks in the presence of joinable datasets. Interactive visualization plays a crucial role in bootstrapping the risk inspection process via risk profiling, triaging and explaining risk signatures, and ultimately detecting instances of true disclosure at a record-level.}
\end{center}
\vspace{-6mm}
\end{figure*}

\par \noindent \textbf{Exploiting vulnerable entry points:} In the cyber kill chain, there is an initial reconnaissance step, where attackers try to \textit{find vulnerable entry points} into any target system~\cite{hutchins2011intelligence}. Following this step, we bootstrapped our red-teaming activity by first defining an initial set of privacy-relevant attributes, like, age, race, gender, age group, and location, to name a few. 
During our initial exploration, we collected  $39,507$ datasets from around $500$ data portals and observed through an automated analysis that about $5404$ datasets have some combinations of quasi-identifiers. Many datasets are related to non-human objects like buildings, animals etc. We filtered out these datasets along with other non-relevant datasets, leading to the development of a seed set of $426$ datasets, including $151$ individual record-level~(e.g., records of people committing crimes) and $275$ aggregated record-level~(e.g., records of schools) datasets. 

Next, we experimented with different combinations from the metadata dictionary to find relevant datasets from the seed selection\kaustav{RQ1: Find entry points}. We used various combinations of the popular tags like health, crime, demographics, etc., to narrow down to an even smaller set of datasets\kaustav{RQ3: Triage possible combinations}. Analysis of these datasets led to some interesting observations where some of the datasets have a highly skewed distribution of records across different categories of the quasi-identifiers. For example, the dataset \textit{Whole Person Care Demographics 2}\cite{WholePersonDemographics2:online} from the \textit{County of San Mateo Datahub portal}\cite{SMCDatahub:online} has only $1$ record for a $26$-year old female of the race Hawaiian/Alaskan. This can lead to identity disclosure and potentially disclose sensitive information about this individual if joined with other individual record-level datasets. Similar examples were observed in the datasets from other portals, like the dataset \textit{Austin Public Health Diabetes Self-Management Education Participant Demographics 2015-2017} has only $1$ record for a 16-year old Hispanic/Latino female who also uses the Medicare insurance\kaustav{RQ4: Evaluate disclosures}. 



% Thus, an analysis using a curated set of quasi-identifiers and popular keywords led to two entry points into the forest of open datasets which can lead to disclosure due to linking attack. One entry point can be the a filtered set of datasets which can be joined to reveal disclosures while the other one can be a set of datasets with highly skewed distribution of records for the quasi-identifiers.

%During the initial reconnaissance step, we observed that there can be multiple entry points into the open data systems which can be vulnerable to disclosure due to linking attacks. 
%Datasets selection is an integral part of this process. During the initial reconnaissance step in the red-team activity, we classified datasets based on: individual records: where each record corresponds to a single individual, like arrests dataset, medical records etc, and {aggregated records:} where each record corresponds to the aggregated values for a certain category, like disease infection in a county, education levels in a district etc.


%A possible way of attack is to find datasets with low/unique records and then evaluate their joinability risk with other datasets to find disclosures. We observed that the dataset \textit{Austin Public Health Diabetes Self-Management Education Participant Demographics 2015-2017} has only $1$ record with age=$16$, Gender=Female and Race=Hispanic/Latino and uses the Medicare insurance. These can be again joined with other datasets to disclose more sensitive attributes of this individual.

%Analysis of the datasets at the record level during the red-teaming exercise revealed that the presence of unique records or records in the low count can cause disclosure of sensitive information too. The idea behind this attack scenario is to find such datasets from the open data portals which can be joined with other individual record-level datasets to reveal sensitive information. For example, if we find an aggregated dataset with a very low count of a certain race category in a specific location, then we can find individual-level datasets for the same location and join them to disclose sensitive information about the individual. The motivations for this scenario may be similar to that of the earlier attack scenario but the chances of finding disclosures increases since the number of available aggregated dataset is far more than the available individual level datasets.

%The importance of this attack scenario is amplified by the examples we observed during the red-teaming exercise. The dataset Whole Person Care Demographics 2\cite{WholePersonDemographics2:online} from the County of San Mateo Datahub portal\cite{SMCDatahub:online} has only $1$ record for the race="Hawaiian/Alaskan", age=$26$ and sex="Female". Similarly, the dataset \textit{Austin Public Health Diabetes Self-Management Education Participant Demographics 2015-2017}\cite{AustinPublicHealth} has only $1$ record with age=$16$, Gender=Female and Race=Hispanic/Latino and uses the Medicare insurance. With such specific information, these datasets can be joined with other individual level datasets from the same location to reveal more sensitive information about this person.



\par \noindent \textbf{Exploiting dataset joins}: After building an initial collection of vulnerable datasets, we aimed to understand the consequence of an attacker joining them and getting access to sensitive information.
Join is a fundamental operation that connects two or more datasets, and joinability is the measure to determine if two datasets are linkable by any number of join keys~\cite{dong2021efficient,chia2019khyperloglog}. When these join keys coincide with protected attributes like age, race, location, etc., the outcome of the join can potentially reveal sensitive information about an individual or even disclose the individual's identity.
As a next step in the red-teaming exercise, we randomly selected vulnerable pairs of datasets from multiple open data portals, like NYC Open Data\cite{NYCOpenData:online}, Open Data Kansas City\cite{KansasCityOpenData:online}, City of Dallas Open Data\cite{DallasOpenData:online}, etc. and analyzed them for~\textit{joinability risks}, in terms what kind of sensitive information may be leaked by these joins \kaustav{RQ3: Triage possible combinations}. These two datasets  had $39$ shared attributes along with quasi-identifiers like age, race and sex. Several iterations of the selection of joinable pairs along with different combinations of the shared attributes as the join key led to the discovery of disclosure between the datasets \textit{Juvenile Arrests} and \textit{Adult Arrests} from the \textit{Fort Lauderdale Police Open Data Portal}\cite{FortLauderdaleOpenData:online}. We observed that two individuals, aged $15$ and $21$, mentioned separately in these datasets, were involved in the same incident of larceny on $20$\textsuperscript{th} March, $2018$ at the Coral Ridge Country Club Estate, N Federal Hwy, Fort Lauderdale.
We repeated this exercise and found other examples where dataset joins ultimately led to either identity disclosure or disclosure about information that can be considered as private and sensitive.




%The idea behind this attack scenario is to use the attribute space of the open datasets in order to find the joinable ones. This can be achieved by selecting a set of open datasets and analyzing the similarity on the metadata level of these datasets. The risk of joinability becomes higher if a pair of datasets are similar in their attribute space. These datasets can be then joined using the common attributes as the join key in order to find examples of disclosure using the record level of granularity. This method can be highly effective since during the red-teaming exercise, we observed that the first step towards finding data disclosures starts with joinable datasets. 
% \kaustav{Use this section in the background section} Government organizations collect information about its citizens and some of these datasets are made public through open data portals like NYC Open Data\cite{NYCOpenData:online}, Open Data Kansas City\cite{KansasCityOpenData:online}, City of Dallas Open Data\cite{DallasOpenData:online} etc. These portals enable users to access a vast trove of datasets, use them and distribute them freely\cite{opendatadefinition}. An attacker can find joinable datasets among these open datasets and use them to find disclosures, if any. Joinable datasets are any combination of datasets which have some similar attributes between them and common records can be found using those attributes. An attacker may be highly motivated in using this scenario because if sensitive information is disclosed about any individual by joining multiple individual record-level datasets, their privacy may be compromised to a great extent. Moreover, since governments and other data collection organizations provide assurances that the data collected would be kept confidential, any disclosure would lead to significant consequences including the violation of these assurances\cite{OpenDataPolicyNYC:online, OpenDataPolicyKansas:online, OpenDataPolicyTexas:online}.


%As a next step, we analyzed the datasets with high risk of joinability at the record level, where we performed join operations on these pairs of datasets using different sets of attributes as the join key. This led to some interesting observations like that of two individuals, aged $15$ and $21$ and  mentioned separately in datasets \textit{Juvenile Arrests} and \textit{Adult Arrests} from the Fort Lauderdale Police Open Data Portal\cite{FortLauderdaleOpenData:online}, were involved in the same incident of larceny on $20$\textsuperscript{th} March, $2018$ at the Coral Ridge Country Club Estate, N Federal Hwy, Fort Lauderdale. This is a step towards identity disclosure of the individuals mentioned in this open dataset. Another example of disclosures observed at the record level was when the datasets \textit{APD Field Interview Cards Dataset by Neighborhood} and \textit{APD Traffic Citations by Neighborhood} from Albany Police Department Open Data portal were joined using quasi-identifiers like \textit{age}, \textit{sex}, \textit{neighborhoodxy} and \textit{date}, it was observed that a $23$-year old male was stopped for a routine field interview on $23$\textsuperscript{rd} January, $2021$ at $2$:$45$ am (observed from the first dataset) and received a citation at $2$:$48$ am at the same location for failing to stop at stop sign (observed from the second dataset). This is also a step towards the disclosure of sensitive information of an individual, leading to attribute disclosure.


%The effectiveness of this method can be demonstrated by the datasets Arrests\cite{ArrestsFortLauderdale:online} and Citations\cite{CitationFortLauderdale:online} from the Fort Lauderdale Police Department Open Data portal\cite{FortLauderdaleOpenData:online}. These datasets have $20$ attributes in common, including some of the privacy-related attributes like age, race and gender along with the unique identifier case\_id, thus making it a highly joinable pair. After joining these datasets, we observe that the  Arrests dataset stated that a 29 year old White Male was arrested for "M.O. 16-1 POSSESSION OF MARIJUANA LESS THAN 20 GR'' at 16:55 hrs on 2018-03-12 at "NW 2ND AV, FORT LAUDERDALE" under case id "341803039721", while a record in the Citation dataset stated that a person with similar attributes was charged with "EXPIRED TAG LESS THAN 6 MOS" at the same location at 17:12, under the same case id. This is a case of attribute disclosure where criminal records can be disclosed by joining datasets from open data portals.











%The defender's dilemma states that defenders have to be right 100\% of the time whereas attackers only have to be right once\cite{Changing21:online}. This translates to the fact that the defenders have to be ever vigilant against potential attacks, thus leading to a fear-based approach. A better method would be using the attacker's perspective, where red-team exercises follow the cyber kill chain to find indicators of compromise and evaluate the potential risks\cite{Movingfr87:online, hutchins2011intelligence}. A red-team exercise can be generally defined as a structured process to better understand the capabilities of an system by viewing the problems through the lenses of an adversary\cite{zenko2015red}. This can be a faster and more useful way of finding risks, hence we have used this approach to imitate the red-team activities and evaluate the possible attack scenarios for finding disclosure by joining datasets available through open data portals.  

%Initial reconnaissance is the first step in the cyber kill chain, where the attackers try to find vulnerable entry points into the target system. We have translated this step in the context of open datasets as finding privacy-related attributes which may lead to disclosure of sensitive information. We have used a tool named Urban Forest, developed by some of the co-authors of this paper, to find such attributes from the datasets of the domain health, education and crime. Some of these attributes like age, gender and race were then used to find datasets which may be vulnerable to linking attacks. We found interesting observations like the dataset \textit{Overdose Information Network Data CY January 2018 - Current Monthly County State Police} has only $1$ record with 1 person with attribute:Ethnicity=“Hispanic”, Gender Desc = "Female", Age Range="40-49". Similarly, in the dataset \textit{Austin Public Health Diabetes Self-Management Education Participant Demographics 2015-2017}, there is only $1$ record with age=16, Gender=Female and Race=Hispanic/Latino and uses the Medicare insurance. This make it surprisingly easy to identify an individual, leading to identity disclosure. We also observed datasets like Lobbyist Data - Historical - Lobbyist Categorized Expenditures Report - 2010 and Lobbyist Data - Lobbyist Categorized Expenditures Report (Deprecated October 2015) have common attributes like first\_name, middle\_initial,last\_name, client\_name and joining these datasets we can derive the expenditures made by around 197 lobbyists of Chicago, over the years. Another example: there is only 1 record with age=19, gender=Male in the dataset \textit{Demographics for Public Health, Policy, and Planning} with additional information available about the city and the language spoken by this individual, which makes it surprisingly easy to identify this person. Also, joining the datasets \textit{Immunization data for all students, kindergarten through 12th grade}, \textit{2014-2015 school year and Kindergarten Immunization Data, 2014-2015}, we can get additional details like Percent\_complete\_for\_diphtheria\_tetanus, Percent\_complete\_for\_pertussis, Percent\_complete\_for\_measles\_mumps\_rubella,Percent\_complete\_for polio, Number\_out\_of\_compliance, Number\_incomplete\_for\_HepatitisB and others.
%Our red-team exercises started with the manual analysis of the datasets from the open data portals in order to identify some of the privacy-related attributes which may lead to the disclosure of sensitive information, almost similar to the initial reconnaissance step employed during such activities. This was followed by a depth-first approach, where first, we used the datasets available from some of the popular data portals to ascertain if there can be any possible leak of sensitive information and then, different methods were tested for their validity and effectiveness in finding disclosures. After successfully finding few examples symptomatic of disclosure risks, these techniques were then implemented across multiple data portals in order to find similar examples.  We then summarized these methods to observe two major attack scenarios and thus, developed a visual analytic workflow which defenders can use to emulate these attack scenarios and formulate their defense plan. 


% %The attack scenarios have been described using the classification scheme developed by Elliot and Dale\cite{elliot1999scenarios} which uses motivation, means, attack type, matching variables, likelihood of success and the likelihood of attempt among some of the main components for classification. \aritra{Emphasize the fact that we took on the role of a red team for understanding attack scenarios and accordingly develop defense strategies. Unclear how we are using the classification scheme.}

% \aritra{VERY IMPORTANT: You are not giving the impression that we carried out the red-teaming tasks. We discussed several times that the way to discuss our workflow is to exactly communicate what we did: we carried out the red-teaming tasks manually, found examples that are symptomatic of disclosure risks and then developed a visual analytic workflow that can be used by defenders to replicate the attack strategies and take appropriate measures for risk analysis and disclosure prevention.} \kaustav{Highlighted the red-teaming exercise. }



% \subsection{Attack Scenarios}


% \textbf{Attack through joinable datasets} \label{section:attack_scenario1}


%For example, suppose an attacker observes that there is a crime related dataset in a certain open data portal and it has quasi-identifiers like age, gender, race and location. The attacker can use these quasi-identifiers as the matching variables and join this dataset with other similar individual record-level datasets to find disclosures that will help to identify the individuals present in this dataset. During our read-teaming activity, a real world example was found with the datasets Arrests\cite{ArrestsFortLauderdale:online} and Citations\cite{CitationFortLauderdale:online} from the Fort Lauderdale Police Department Open Data portal\cite{FortLauderdaleOpenData:online}, both of which have the quasi-identifiers age, gender, race, ethnicity and the identifier case-id. A record in the Arrests dataset stated that a 29 year old White Male was arrested for "M.O. 16-1 POSSESSION OF MARIJUANA LESS THAN 20 GR'' at 16:55 hrs on 2018-03-12 at "NW 2ND AV, FORT LAUDERDALE" under case id "341803039721", while a record in the Citation dataset stated that a person with similar attributes was charged with "EXPIRED TAG LESS THAN 6 MOS" at the same location at 17:12, under the same case id. This can be considered a case of possible attribute disclosure.





%Some data portals do not release data points (or mask/suppress them) where the count is very low, thus protecting against this attack scenario to some extent\cite{DataAggrregationGuidelines:online}. Moreover, chances of finding a risky aggregated dataset and a corresponding individual level dataset are quite low. Hence, some degree of automation is required in this scenario, since manually analyzing the multitudes of combinations may be a cumbersome task. Similar to the previous attack scenario, revealing sensitive information through this attack scenario may still invade the privacy of the citizens participating in surveys performed by government organizations, also dealing a blow to the credibility of these organizations in handling sensitive data. <add a line for visual analytic workflow)

telligence}. With the help of researchers in data privacy and urban informatics, we performed a red-teaming exercise by inspecting the open datasets for vulnerabilities. We engaged in a cold-start exploration process, followed by more focused exploitation of datasets with privacy-relevant attributes, for developing a shared mental model of the problems related to the vulnerabilities. The intuition here was that the datasets with universally known quasi-identifiers, like age, race, gender, etc., can lead to the disclosure of sensitive information when joined with other such datasets. 





\begin{figure*}[t]
\begin{center}
\includegraphics[width=\textwidth]{figures/workflow.pdf}
\vspace{-4mm}
 \caption{\label{figs:PRIVEE}\textbf{PRIVEE is an end-to-end risk inspection workflow for open datasets} that informs the defender in the analytical loop about potential disclosure risks in the presence of joinable datasets. Interactive visualization plays a crucial role in bootstrapping the risk inspection process via risk profiling, triaging and explaining risk signatures, and ultimately detecting instances of true disclosure at a record-level.}
\end{center}
\vspace{-6mm}
\end{figure*}

\par \noindent \textbf{Exploiting vulnerable entry points:} In the cyber kill chain, there is an initial reconnaissance step, where attackers try to \textit{find vulnerable entry points} into any target system~\cite{hutchins2011intelligence}. Following this step, we bootstrapped our red-teaming activity by first defining an initial set of privacy-relevant attributes, like, age, race, gender, age group, and location, to name a few. 
During our initial exploration, we collected  $39,507$ datasets from around $500$ data portals and observed through an automated analysis that about $5404$ datasets have some combinations of quasi-identifiers. Many datasets are related to non-human objects like buildings, animals etc. We filtered out these datasets along with other non-relevant datasets, leading to the development of a seed set of $426$ datasets, including $151$ individual record-level~(e.g., records of people committing crimes) and $275$ aggregated record-level~(e.g., records of schools) datasets. 

Next, we experimented with different combinations from the metadata dictionary to find relevant datasets from the seed selection\kaustav{RQ1: Find entry points}. We used various combinations of the popular tags like health, crime, demographics, etc., to narrow down to an even smaller set of datasets\kaustav{RQ3: Triage possible combinations}. Analysis of these datasets led to some interesting observations where some of the datasets have a highly skewed distribution of records across different categories of the quasi-identifiers. For example, the dataset \textit{Whole Person Care Demographics 2}\cite{WholePersonDemographics2:online} from the \textit{County of San Mateo Datahub portal}\cite{SMCDatahub:online} has only $1$ record for a $26$-year old female of the race Hawaiian/Alaskan. This can lead to identity disclosure and potentially disclose sensitive information about this individual if joined with other individual record-level datasets. Similar examples were observed in the datasets from other portals, like the dataset \textit{Austin Public Health Diabetes Self-Management Education Participant Demographics 2015-2017} has only $1$ record for a 16-year old Hispanic/Latino female who also uses the Medicare insurance\kaustav{RQ4: Evaluate disclosures}. 



% Thus, an analysis using a curated set of quasi-identifiers and popular keywords led to two entry points into the forest of open datasets which can lead to disclosure due to linking attack. One entry point can be the a filtered set of datasets which can be joined to reveal disclosures while the other one can be a set of datasets with highly skewed distribution of records for the quasi-identifiers.

%During the initial reconnaissance step, we observed that there can be multiple entry points into the open data systems which can be vulnerable to disclosure due to linking attacks. 
%Datasets selection is an integral part of this process. During the initial reconnaissance step in the red-team activity, we classified datasets based on: individual records: where each record corresponds to a single individual, like arrests dataset, medical records etc, and {aggregated records:} where each record corresponds to the aggregated values for a certain category, like disease infection in a county, education levels in a district etc.


%A possible way of attack is to find datasets with low/unique records and then evaluate their joinability risk with other datasets to find disclosures. We observed that the dataset \textit{Austin Public Health Diabetes Self-Management Education Participant Demographics 2015-2017} has only $1$ record with age=$16$, Gender=Female and Race=Hispanic/Latino and uses the Medicare insurance. These can be again joined with other datasets to disclose more sensitive attributes of this individual.

%Analysis of the datasets at the record level during the red-teaming exercise revealed that the presence of unique records or records in the low count can cause disclosure of sensitive information too. The idea behind this attack scenario is to find such datasets from the open data portals which can be joined with other individual record-level datasets to reveal sensitive information. For example, if we find an aggregated dataset with a very low count of a certain race category in a specific location, then we can find individual-level datasets for the same location and join them to disclose sensitive information about the individual. The motivations for this scenario may be similar to that of the earlier attack scenario but the chances of finding disclosures increases since the number of available aggregated dataset is far more than the available individual level datasets.

%The importance of this attack scenario is amplified by the examples we observed during the red-teaming exercise. The dataset Whole Person Care Demographics 2\cite{WholePersonDemographics2:online} from the County of San Mateo Datahub portal\cite{SMCDatahub:online} has only $1$ record for the race="Hawaiian/Alaskan", age=$26$ and sex="Female". Similarly, the dataset \textit{Austin Public Health Diabetes Self-Management Education Participant Demographics 2015-2017}\cite{AustinPublicHealth} has only $1$ record with age=$16$, Gender=Female and Race=Hispanic/Latino and uses the Medicare insurance. With such specific information, these datasets can be joined with other individual level datasets from the same location to reveal more sensitive information about this person.



\par \noindent \textbf{Exploiting dataset joins}: After building an initial collection of vulnerable datasets, we aimed to understand the consequence of an attacker joining them and getting access to sensitive information.
Join is a fundamental operation that connects two or more datasets, and joinability is the measure to determine if two datasets are linkable by any number of join keys~\cite{dong2021efficient,chia2019khyperloglog}. When these join keys coincide with protected attributes like age, race, location, etc., the outcome of the join can potentially reveal sensitive information about an individual or even disclose the individual's identity.
As a next step in the red-teaming exercise, we randomly selected vulnerable pairs of datasets from multiple open data portals, like NYC Open Data\cite{NYCOpenData:online}, Open Data Kansas City\cite{KansasCityOpenData:online}, City of Dallas Open Data\cite{DallasOpenData:online}, etc. and analyzed them for~\textit{joinability risks}, in terms what kind of sensitive information may be leaked by these joins \kaustav{RQ3: Triage possible combinations}. These two datasets  had $39$ shared attributes along with quasi-identifiers like age, race and sex. Several iterations of the selection of joinable pairs along with different combinations of the shared attributes as the join key led to the discovery of disclosure between the datasets \textit{Juvenile Arrests} and \textit{Adult Arrests} from the \textit{Fort Lauderdale Police Open Data Portal}\cite{FortLauderdaleOpenData:online}. We observed that two individuals, aged $15$ and $21$, mentioned separately in these datasets, were involved in the same incident of larceny on $20$\textsuperscript{th} March, $2018$ at the Coral Ridge Country Club Estate, N Federal Hwy, Fort Lauderdale.
We repeated this exercise and found other examples where dataset joins ultimately led to either identity disclosure or disclosure about information that can be considered as private and sensitive.




%The idea behind this attack scenario is to use the attribute space of the open datasets in order to find the joinable ones. This can be achieved by selecting a set of open datasets and analyzing the similarity on the metadata level of these datasets. The risk of joinability becomes higher if a pair of datasets are similar in their attribute space. These datasets can be then joined using the common attributes as the join key in order to find examples of disclosure using the record level of granularity. This method can be highly effective since during the red-teaming exercise, we observed that the first step towards finding data disclosures starts with joinable datasets. 
% \kaustav{Use this section in the background section} Government organizations collect information about its citizens and some of these datasets are made public through open data portals like NYC Open Data\cite{NYCOpenData:online}, Open Data Kansas City\cite{KansasCityOpenData:online}, City of Dallas Open Data\cite{DallasOpenData:online} etc. These portals enable users to access a vast trove of datasets, use them and distribute them freely\cite{opendatadefinition}. An attacker can find joinable datasets among these open datasets and use them to find disclosures, if any. Joinable datasets are any combination of datasets which have some similar attributes between them and common records can be found using those attributes. An attacker may be highly motivated in using this scenario because if sensitive information is disclosed about any individual by joining multiple individual record-level datasets, their privacy may be compromised to a great extent. Moreover, since governments and other data collection organizations provide assurances that the data collected would be kept confidential, any disclosure would lead to significant consequences including the violation of these assurances\cite{OpenDataPolicyNYC:online, OpenDataPolicyKansas:online, OpenDataPolicyTexas:online}.


%As a next step, we analyzed the datasets with high risk of joinability at the record level, where we performed join operations on these pairs of datasets using different sets of attributes as the join key. This led to some interesting observations like that of two individuals, aged $15$ and $21$ and  mentioned separately in datasets \textit{Juvenile Arrests} and \textit{Adult Arrests} from the Fort Lauderdale Police Open Data Portal\cite{FortLauderdaleOpenData:online}, were involved in the same incident of larceny on $20$\textsuperscript{th} March, $2018$ at the Coral Ridge Country Club Estate, N Federal Hwy, Fort Lauderdale. This is a step towards identity disclosure of the individuals mentioned in this open dataset. Another example of disclosures observed at the record level was when the datasets \textit{APD Field Interview Cards Dataset by Neighborhood} and \textit{APD Traffic Citations by Neighborhood} from Albany Police Department Open Data portal were joined using quasi-identifiers like \textit{age}, \textit{sex}, \textit{neighborhoodxy} and \textit{date}, it was observed that a $23$-year old male was stopped for a routine field interview on $23$\textsuperscript{rd} January, $2021$ at $2$:$45$ am (observed from the first dataset) and received a citation at $2$:$48$ am at the same location for failing to stop at stop sign (observed from the second dataset). This is also a step towards the disclosure of sensitive information of an individual, leading to attribute disclosure.


%The effectiveness of this method can be demonstrated by the datasets Arrests\cite{ArrestsFortLauderdale:online} and Citations\cite{CitationFortLauderdale:online} from the Fort Lauderdale Police Department Open Data portal\cite{FortLauderdaleOpenData:online}. These datasets have $20$ attributes in common, including some of the privacy-related attributes like age, race and gender along with the unique identifier case\_id, thus making it a highly joinable pair. After joining these datasets, we observe that the  Arrests dataset stated that a 29 year old White Male was arrested for "M.O. 16-1 POSSESSION OF MARIJUANA LESS THAN 20 GR'' at 16:55 hrs on 2018-03-12 at "NW 2ND AV, FORT LAUDERDALE" under case id "341803039721", while a record in the Citation dataset stated that a person with similar attributes was charged with "EXPIRED TAG LESS THAN 6 MOS" at the same location at 17:12, under the same case id. This is a case of attribute disclosure where criminal records can be disclosed by joining datasets from open data portals.











%The defender's dilemma states that defenders have to be right 100\% of the time whereas attackers only have to be right once\cite{Changing21:online}. This translates to the fact that the defenders have to be ever vigilant against potential attacks, thus leading to a fear-based approach. A better method would be using the attacker's perspective, where red-team exercises follow the cyber kill chain to find indicators of compromise and evaluate the potential risks\cite{Movingfr87:online, hutchins2011intelligence}. A red-team exercise can be generally defined as a structured process to better understand the capabilities of an system by viewing the problems through the lenses of an adversary\cite{zenko2015red}. This can be a faster and more useful way of finding risks, hence we have used this approach to imitate the red-team activities and evaluate the possible attack scenarios for finding disclosure by joining datasets available through open data portals.  

%Initial reconnaissance is the first step in the cyber kill chain, where the attackers try to find vulnerable entry points into the target system. We have translated this step in the context of open datasets as finding privacy-related attributes which may lead to disclosure of sensitive information. We have used a tool named Urban Forest, developed by some of the co-authors of this paper, to find such attributes from the datasets of the domain health, education and crime. Some of these attributes like age, gender and race were then used to find datasets which may be vulnerable to linking attacks. We found interesting observations like the dataset \textit{Overdose Information Network Data CY January 2018 - Current Monthly County State Police} has only $1$ record with 1 person with attribute:Ethnicity=“Hispanic”, Gender Desc = "Female", Age Range="40-49". Similarly, in the dataset \textit{Austin Public Health Diabetes Self-Management Education Participant Demographics 2015-2017}, there is only $1$ record with age=16, Gender=Female and Race=Hispanic/Latino and uses the Medicare insurance. This make it surprisingly easy to identify an individual, leading to identity disclosure. We also observed datasets like Lobbyist Data - Historical - Lobbyist Categorized Expenditures Report - 2010 and Lobbyist Data - Lobbyist Categorized Expenditures Report (Deprecated October 2015) have common attributes like first\_name, middle\_initial,last\_name, client\_name and joining these datasets we can derive the expenditures made by around 197 lobbyists of Chicago, over the years. Another example: there is only 1 record with age=19, gender=Male in the dataset \textit{Demographics for Public Health, Policy, and Planning} with additional information available about the city and the language spoken by this individual, which makes it surprisingly easy to identify this person. Also, joining the datasets \textit{Immunization data for all students, kindergarten through 12th grade}, \textit{2014-2015 school year and Kindergarten Immunization Data, 2014-2015}, we can get additional details like Percent\_complete\_for\_diphtheria\_tetanus, Percent\_complete\_for\_pertussis, Percent\_complete\_for\_measles\_mumps\_rubella,Percent\_complete\_for polio, Number\_out\_of\_compliance, Number\_incomplete\_for\_HepatitisB and others.
%Our red-team exercises started with the manual analysis of the datasets from the open data portals in order to identify some of the privacy-related attributes which may lead to the disclosure of sensitive information, almost similar to the initial reconnaissance step employed during such activities. This was followed by a depth-first approach, where first, we used the datasets available from some of the popular data portals to ascertain if there can be any possible leak of sensitive information and then, different methods were tested for their validity and effectiveness in finding disclosures. After successfully finding few examples symptomatic of disclosure risks, these techniques were then implemented across multiple data portals in order to find similar examples.  We then summarized these methods to observe two major attack scenarios and thus, developed a visual analytic workflow which defenders can use to emulate these attack scenarios and formulate their defense plan. 


% %The attack scenarios have been described using the classification scheme developed by Elliot and Dale\cite{elliot1999scenarios} which uses motivation, means, attack type, matching variables, likelihood of success and the likelihood of attempt among some of the main components for classification. \aritra{Emphasize the fact that we took on the role of a red team for understanding attack scenarios and accordingly develop defense strategies. Unclear how we are using the classification scheme.}

% \aritra{VERY IMPORTANT: You are not giving the impression that we carried out the red-teaming tasks. We discussed several times that the way to discuss our workflow is to exactly communicate what we did: we carried out the red-teaming tasks manually, found examples that are symptomatic of disclosure risks and then developed a visual analytic workflow that can be used by defenders to replicate the attack strategies and take appropriate measures for risk analysis and disclosure prevention.} \kaustav{Highlighted the red-teaming exercise. }



% \subsection{Attack Scenarios}


% \textbf{Attack through joinable datasets} \label{section:attack_scenario1}


%For example, suppose an attacker observes that there is a crime related dataset in a certain open data portal and it has quasi-identifiers like age, gender, race and location. The attacker can use these quasi-identifiers as the matching variables and join this dataset with other similar individual record-level datasets to find disclosures that will help to identify the individuals present in this dataset. During our read-teaming activity, a real world example was found with the datasets Arrests\cite{ArrestsFortLauderdale:online} and Citations\cite{CitationFortLauderdale:online} from the Fort Lauderdale Police Department Open Data portal\cite{FortLauderdaleOpenData:online}, both of which have the quasi-identifiers age, gender, race, ethnicity and the identifier case-id. A record in the Arrests dataset stated that a 29 year old White Male was arrested for "M.O. 16-1 POSSESSION OF MARIJUANA LESS THAN 20 GR'' at 16:55 hrs on 2018-03-12 at "NW 2ND AV, FORT LAUDERDALE" under case id "341803039721", while a record in the Citation dataset stated that a person with similar attributes was charged with "EXPIRED TAG LESS THAN 6 MOS" at the same location at 17:12, under the same case id. This can be considered a case of possible attribute disclosure.





%Some data portals do not release data points (or mask/suppress them) where the count is very low, thus protecting against this attack scenario to some extent\cite{DataAggrregationGuidelines:online}. Moreover, chances of finding a risky aggregated dataset and a corresponding individual level dataset are quite low. Hence, some degree of automation is required in this scenario, since manually analyzing the multitudes of combinations may be a cumbersome task. Similar to the previous attack scenario, revealing sensitive information through this attack scenario may still invade the privacy of the citizens participating in surveys performed by government organizations, also dealing a blow to the credibility of these organizations in handling sensitive data. <add a line for visual analytic workflow)



==> sections/evaluation_old.tex <==
\section{Evaluation}
% \section{Usage Scenario for Data Subjects} \label{section:scenario3}
% \label{section:scenario1}


% Sophia is a resident of San Mateo County in California. The county officials assured her that the citizens' data are not published directly to its open data portal \cite{SMCDatahub:online}, instead they are aggregated using different attributes like age, race, sex etc. Sophia was worried if her health data could be disclosed online, so she selected the aggregated datasets tagged with the keyword "health" in the interface PRIVEE and then selected the data portal of the San Mateo county (see Figure \ref{figs:scenario3}a). She also selected few privacy-related attributes like \textit{age}, \textit{sex} and \textit{race} since she was informed that the datasets are aggregated using these attributes (Figure \ref{figs:scenario3}b) (\textbf{T1}). 
% While analyzing the vulnerabilities in the data distributions, Sophia observed that the dataset \textit{Whole Person Care Demographics 2} \cite{WholePersonDemographics2:online} had only $1$ record where the race was "Hawaiian/Alaskan" (Figure \ref{figs:scenario3}c) (\textbf{T2}). This finding was a great cause of concern for Sophia since she identified herself as Hawaiian, and any dataset with a similar race category could potentially expose her health records. Thus, she started analyzing the risk of joining this dataset with all the individual-record level datasets available through PRIVEE, as shown in Figure \ref{figs:scenario3}c (\textbf{T4}). Since there would be around 151 dataset combinations (the number of individual-record level datasets available), she decided to filter those combinations with a higher risk score ($\geq 130$), using the filter available in the risk score distribution histogram. She decided to join these dataset pairs on the privacy-related attributes along with the location attribute \textit{geocodedcolumnn} since she wished to find datasets that contain information relevant to her location. She observed that none of the top-4 dataset pairs yield any common record when joined on these attributes (Figure \ref{figs:scenario3}d). Thus, Sophia concluded that though the aggregated dataset \textit{Whole Person Care Demographics 2} has a meager count of a particular race, it does not lead to any disclosure (\textbf{T5}).

\subsection{Case Study with primary collaborator} \label{section:case_study1}
% Refer to Lam et al.'s "Empirical studies in information visualization: Seven scenarios" and Sedlmair et al.'s "Design Study Methodology: Reflections from the Trenches and the Stacks" to justify that there are two forms of validation: Case study and Informal usability testing and analyst feedback
In this sub-section, we report one of the case studies which our data privacy collaborator and co-author co-developed using the web interface of PRIVEE. He is a senior researcher with more than  $15$ years of experience in privacy-preserving data analysis and used PRIVEE as a privacy auditor. Specifically, he wanted to find out if there are any possible disclosure risks with the datasets published in the open data portals of police departments, where data about people committing crimes are recorded. It is important to note that some of the numbers mentioned this these usage scenarios might change if the respective data owners update the datasets. 

%\subsection{Finding disclosure risk: privacy auditor's perspective (T1a, T2, T3)}
Our collaborator began by choosing the Albany Police Department\cite{AlbanyPolice:online} and observed $6$ individual-level datasets on the Projection View
~(Figure~\ref{figs:case_study1}a) (\textbf{T1}).
He decided to analyze all the possible combinations of these datasets using the projection plot. Datasets \textit{APD Arrests Dataset by Neighborhood} and \textit{APD Arrests Datasets by Patrol Zone} had the highest risk score and shared a common unique identifier, namely \textit{arrestid} ~(Figure~\ref{figs:case_study1}b)
(\textbf{T3}). This dataset pair had the highest risk score since they shared $16$ joining attributes, including $2$ privacy-related attributes. Since \textit{arrestid} had the highest entropy among the other attributes, our collaborator decided to join these datasets based on \textit{arrestid} and observed that there may be $1607$ common records, i.e., $1607$ individuals may be present in both the datasets and new information may be disclosed by joining them (\textbf{T4}). For example, \textit{arrestid} APD*$210001493$ mentioned the arrest of a 21 year old white female in both the datasets. On closer analysis, he observed that these two are almost similar datasets, and the attributes \textit{neighborhood} and \textit{patrolzone} can be disclosed by joining them, leading to potential leakage of sensitive information. Our collaborator appreciated the triage capability of PRIVEE and commented:  ``these visualizations are helping people to quickly identify what they would like to focus on".

He followed this with analysis of the next pair of datasets, \textit{APD LEAD Dataset} and \textit{APD Arrests Dataset by Patrol Zone} and observed that they have common quasi-identifiers like \textit{race}, \textit{age} and \textit{sex}
~Figure~\ref{figs:case_study1}b). 
He then joined these datasets using these quasi-identifiers but found no common records, concluding that these datasets can be combined safely without actual, record-level disclosure (\textbf{T4}). 

He repeated this operation for another pair of datasets \textit{APD Arrests Dataset by Neighborhood} and \textit{APD Field Interview Cards Dataset by Neighborhood} by adding the location attribute \textit{neighborhoodxy}
~(Figure~\ref{figs:case_study1}b)
(\textbf{T3}). He observed $887$ common records, implying that these individuals may be identified through these datasets who were stopped for field interview and later arrested by the police. He observed that the latter dataset does not provide any information about the reason for the field interview. But, joining this with the former dataset shows that a $28$-year old white male was interviewed in the Washington Park neighborhood at $09$:$08$ hrs on $1$\textsuperscript{st} December, $2020$ and was later arrested for trespassing on enclosed property at $12$:$32$ hrs (arrestid: APD*$200001760$). He found similar examples by joining the datasets \textit{APD Field Interview Cards Dataset by Neighborhood} and \textit{APD Traffic Citations by Neighborhood} 
~(Figure~\ref{figs:case_study1}b)
, where an individual of the the same age and gender received a citation on the same date and at the same location at $2$:$48$ am, just $3$ minutes after the incident from the first dataset, similar to the example shown in Figure~\ref{figs:disclosure_example}a ~(see the two arrows in Figure \ref{figs:case_study1}d)
(\textbf{T4}). 

In his role as a privacy auditor, our collaborator flagged these datasets for record-level disclosure of sensitive information, an outcome of PRIVEE that can be used by data custodians for making decisions about applying anonymization methods for minimizing the disclosure risks. Our collaborator observed that he had not seen a tool with similar capabilities for interactive risk calibration and triage, and  commented: "\textit{this is a great visual tool to explore privacy risks of open data, with the ability to visualize privacy risk and see matches across datasets in a dynamic manner}".

\begin{figure*}[t]
\begin{center}
\includegraphics[width=\textwidth]{figures/case_study1.pdf}
\vspace{-4mm}
 \caption{\label{figs:case_study1}\textbf{Case Study with long-term collaborator:} (a) the expert selected the datasets from the Albany Police Open Data portal, which are shown in the Projection View, along with the popular attributes in these datasets, (b) the Risk Assessment View showed the pairwise combinations of these datasets and their joinability risk, (c) one of the pairs when joined on the quasi-identifiers age, sex, neighborhoodxy and date showed only $4$ matching records, (d) analyzing the records showed an example of identity disclosure where a person was stopped for field interview and was cited just three minutes later (Section~\ref{section:case_study1})}
\end{center}
\vspace{-4mm}
\end{figure*}
%"This is very useful because it gives you direct visualization of what is there in the these datasets and the extent to which it can potentially lead to privacy breaches."

%"The visualization are helping people to quickly identify what they would like to focus on"

 

% \section{Case Study}



% In this section, we discuss a case study we developed using our tool \textit{PRIVEE} in conjunction with a domain expert who is also a co-author of this paper. Their expertise is in information privacy and secure computation technologies. \aritra{who is this expert what is his background and experience, is he a co-author?)}It is important to note that some of the numbers mentioned this these usage scenarios may change if the datasets are updated by the respective data owners.

% %\subsection{Finding disclosure risk: privacy auditor's perspective (T1a, T2, T3)}


 
% Police datasets can potentially damage an individual's social life if their sensitive information is disclosed. Amy, an independent privacy auditor, wants to find out if there are any possible disclosure risk with the datasets published in the open data portals of police departments. She selects the data portal for Albany Police Department\cite{AlbanyPolice:online} in \textit{PRIVEE} and observes $6$ individual-level datasets on the dataset joinability view (see Fig \ref{figs:scenario1}a) \textbf{(T1a)}. She decides to analyze all the possible combinations of these datasets by selecting all the dots in the projection plot. This shows all the possible dataset combinations along with their joining attributes but sorted according to their risk scores (see Fig \ref{figs:scenario1}b) (refer Section \ref{section:risk_score_calculation}) for detailed description). She observes that the datasets \textit{APD Arrests Dataset by Neighborhood} and \textit{APD Arrests Datasets by Patrol Zone} have the highest risk score and share a common unique identifier, namely \textit{arrestid} (\textbf{T2}). This dataset pair has the highest risk score since they share $16$ joining attributes, including $2$ privacy-related attributes (refer Section \ref{section:risk_score_calculation} for detailed calculation). Since \textit{arrestid} has the highest entropy among the other attributes, Amy decides to join these datasets based on \textit{arrestid} and observes that there may be $1607$ common records, i.e., $1607$ individuals may be present in both the datasets and new information may be disclosed by joining them (see Fig \ref{figs:scenario1}c) (\textbf{T3}). For example, \textit{arrestid} APD*$210001493$ mentions the arrest of a 21 year old white female in both the datasets. On closer analysis, she observes that these two are almost similar datasets, the attributes \textit{neighborhood} and \textit{patrolzone} can be disclosed by joining these datasets. This is an example of attribute disclosure using datasets from open data portals.

% Now she analyzes the next pair of datasets \textit{APD LEAD Dataset} and \textit{APD Arrests Dataset by Patrol Zone} and observes that they have common quasi-identifiers like \textit{race}, \textit{age} and \textit{sex} (see Fig \ref{figs:scenario1}b) (\textbf{T2}). Amy tries to join these datasets using these quasi-identifiers but finds that there are no common records, thus implying that these datasets can be combined safely on these quasi-identifiers (\textbf{T3}). She also repeats this same procedure for the next pair of datasets \textit{APD Arrests Dataset by Neighborhood} and \textit{APD LEAD Dataset} and observes that there are no common records between them, hence derives the same conclusion (see Fig \ref{figs:scenario1}b) (\textbf{T2},\textbf{T3}). She performs this operation one more time for the next pair of datasets \textit{APD Arrests Dataset by Neighborhood} and \textit{APD Field Interview Cards Dataset by Neighborhood} and also adds the location attribute \textit{neighborhoodxy} (see Fig \ref{figs:scenario1}b) (\textbf{T2}). She observes $887$ common records, which implies that these individuals may be identified through these datasets who were stopped for field interview and later arrested by the police. She observes that though the later dataset does not provide any information about the reason for the field interview, joining this with the former dataset shows that a $28$-year old white male was interviewed in the Washington Park neighborhood at $09$:$08$ hrs on $1$\textsuperscript{st} December, $2020$ and was later arrested for trespassing on enclosed property at $12$:$32$ hrs (arrestid: APD*$200001760$). This is an example of disclosure using quasi-identifiers present in open datasets (\textbf{T3}). She found more such examples by joining the datasets \textit{APD Arrests Dataset by Patrol Zone} and \textit{APD Field Interview Cards Dataset by Neighborhood}  where a $26$-year old black female was interviewed at $11$:$23$ hrs on $11$\textsuperscript{th} December, $2020$ and was later arrested at $21$:$25$ hrs for "assault with intent to cause physical injury" (arrestid: APD*$200001826$) (\textbf{T3}). Next, she joined the datasets \textit{APD Field Interview Cards Dataset by Neighborhood} and \textit{APD Traffic Citations by Neighborhood} on the attributes \textit{age}, \textit{sex}, \textit{neighborhoodxy}and  \textit{date} and observed $4$ common records between them (see Fig \ref{figs:scenario1}d) (\textbf{T2}). 




% She observed that $23$-year old male was stopped for field interview on $23$\textsuperscript{rd} January, $2021$ at $2$:$45$ am and since field interviews are normal routine stop and search activities by the police, this may seem a regular incident, but the other dataset informed her that an individual of the same same age and gender received a citation on the same date and at the same location at $2$:$48$ am, just $3$ minutes after the incident from the first dataset (see the two arrows in Fig \ref{figs:scenario1}d). Since these both records seem to belong to the same person, this is a possible identity disclosure and it was discovered using a combination of date and quasi-identifiers like location coordinates, age and gender (\textbf{T3}).

% \begin{comment}

% As a domain expert, Amy believed that this kind of disclosures may be present in other police data portals too. Hence, she selected the Fort Lauderdale Police Open Data Portal\cite{FortLauderdaleOpenData:online} and selected all the 5 datasets for analysis. 
% %She observed that the datasets Adult Arrests and Arrests have the highest risk score and also share unique identifiers like incidentid and caseid. She joined these datasets on these unique identifiers and other quasi-identifiers like race, age and sex, and observed 27479 common records. This implies that sensitive information about 27479 individuals may be compromised by joining these datasets (not loaded on interface). She also observed that the next pair of datasets Arrests and Juvenile Arrests also share the unique identifiers like incidentid and caseid and observed 5180 common records, i.e., 5180 individuals may be identified by joining these datasets and their sensitive information can be compromised.<insert example; interface does not show all of the lines>
% She joined datasets \textit{Adult Arrests} and \textit{Juvenile Arrests} based on the unique identifiers \textit{incidentid} and \textit{caseid} and observed $347$ common records. Though adult arrests and juvenile arrests should not have any common records as they serve completely different age groups, Amy observed that for the incident id $341803044797$ and caseid $341803044797$, the Adult Arrests dataset lists the age as $21$ while the Juvenile Arrests dataset lists the age as $15$. This implies that two people, age $15$ and $21$ were involved in larceny on $20$\textsuperscript{th} March, $2018$ with the exact charge being "LARC-GRAND THEFT 300 LESS THAN 5K DOLS".  More sensitive information like this can also be observed in other common records where the \textit{incidentid} and \textit{caseid} are $341807108870$ and it discloses the fact that two people, aged $17$ and $21$, were involved in a theft of motor vehicle (VEH THEFT-GRAND THEFT OF MOTOR VEHICLE) on $8$\textsuperscript{th} of July, $2018$. She also joins the dataset pair \textit{Arrest} and \textit{Citations} on the unique identifier \textit{case\_id} and observes $2760$ common records. For example, a $28$ year old black male was arrested for larceny on $26$\textsuperscript{th} September $2021$ at NW $10$\textsuperscript{th} Ave, was also cited for disobeying stop/yield sign and driving while license is suspended at NW $9$\textsuperscript{th} Street, around $3$ miles away from the arrest location(case\_id: $342109159680$). Other dataset pairs like \textit{Citations} and \textit{Juvenile Arrests} have $90$ common records when joined on the unique identifier \textit{case\_id}, where a $17$-year old white male was first charged with disobeying red light and was later arrested for possession of cannabis over $20$ grams on $4$\textsuperscript{th} August, $2015$, both at N Federal Hwy, Fort Lauderdale.
% \end{comment}



% PRIVEE helped Amy rapidly implement the attack scenario with joinable datasets in order to find disclosure risks (see Section\ref{section:attack_scenario1}). Thus, she concluded that since there are several possible disclosures by linking the datasets available through the open data portal of this police department, she would recommend to the police administrators that this portal is thoroughly analyzed for further disclosures before releasing any new datasets.


% \begin{comment}

% \subsection{Finding disclosure risk: data custodian's perspective (T1a, T2, T3)} \label{section:scenario2}
% \begin{figure*}
% \begin{center}
% \includegraphics[width=\textwidth]{figures/scenario2.pdf}
% \vspace{-4mm}
%  \caption{\label{figs:scenario2}\textbf{Disclosure risk: data custodian perspective} (a) The wordcloud for the New Orleans police datasets shows victimage as a frequent attribute, hence user select victimage along with other similar attributes (b) Joins two datasets on these attributes along with the location attribute (c) Though the addresses are partially masked, it can be observed that a $22$ year-old black male was charged with attempted armed robbery and attempted simple robbery against a $27$ year-old at the same location on different dates. (Section \ref{section:scenario2}) }
% \end{center}
% \vspace{-6mm}
% \end{figure*}
% \kaustav{Tasks are similar to the first usage scenario but in this scenario, the user updates the privacy related attributes based on what he sees in the wordcloud}
% Kabir, a data custodian with the police department of the City of New Orleans is tasked with the release of the Electronic Police Report for the year $2021$. He wishes to know if there could be any disclosure risk by using the electronic police reports from the previous years. In our interface \textit{PRIVEE}, Kabir selects the open data portal of New Orleans and loads all the available datasets\cite{NewOrleans:online}. He observes from the wordcloud that the attribute \textit{victim\_age} has a higher frequency, hence selects this attribute along with other similar attributes like \textit{offender\_age}, \textit{offender\_gender}, \textit{victim\_gender}, \textit{victim\_race} and \textit{offender\_race} as the privacy-related attributes (Figure \ref{figs:scenario2}a) (\textbf{T1a}).





% Now, he selects all these datasets and analyzes all the possible combinations of these datasets in the Risk Explanation View (\textbf{T2}). Since the police electronic reports across all the years have similar attributes, he started with the datasets \textit{Electronic Police Report 2015} and \textit{Electronic Police Report 2016} and joined them on his previously-selected privacy-related attributes along with the attribute \textit{location} (see Figure \ref{figs:scenario2}b) (\textbf{T2}). At this point, Kabir made an interesting observation that though the addresses used in these datasets are partially masked (see the arrow in Figure \ref{figs:scenario2}c), there are $21$ common records when joined on these attributes. For example, a $22$ year old Black Male was charged with "ATTEMPTED ARMED ROBBERY (GUN)" against a $27$ year old White Male at 6XX Tchoupitoulas St on 2015-07-13 at 01:00 hrs and again on 2016-04-30 at 03:00 hrs with "ATTEMPT - SIMPLE ROBBERY" (see Figure \ref{figs:scenario2}c). Kabir notes this as an example of identity disclosure (\textbf{T3}).



% Next, he joins the datasets \textit{Electronic Police Report 2016} and \textit{Electronic Police Report 2017} on the same attributes and to his surprise, finds $26$ common records despite the fact that the addresses are partially masked (\textbf{T2}, \textbf{T3}). For example, a $25$ year old Black Male was charged with "VIOLATIONS OF PROTECTIVE ORDERS" against a $23$ year old Black Female at 6XX Canal St on 2016-12-10 at 12:29 hrs and again on 2017-11-27 at 02:18 hrs with "DOMESTIC ABUSE BATTERY". He again notes this an example of identity disclosure (\textbf{T3}).

% Next, he joins the datasets \textit{Electronic Police Report 2017} and \textit{Electronic Police Report 2018} on the same attributes and again finds $43$ common records (\textbf{T2}, \textbf{T3}). For example, a $41$ year old Black Male was charged with "SHOPLIFTING", witnessed by a $32$ year old Black Female at 82XX Earhart Bd on 2017-06-06 at 19:50 hrs and again on 2017-11-27 at 02:18 hrs. A similar incident was reported at the same location by the offender and witness of the same attributes on 2018-02-20 at 12:26 hrs (\textbf{T3}). Thus, Kabir concludes that there may be disclosure risk using the previous years' police report datasets, hence those risks need to be carefully analyzed before releasing a new police report dataset.

% \end{comment}

\subsection{Case Study with other collaborator}\label{section:case_study2}
In this sub-section, we report another case study which our collaborator developed using the PRIVEE web interface. He is a senior researcher and university professor with over 25 years of experience in the fields of big data, cyber security and scientific visualization. Though he was consulted during the ideation stage of the PRIVEE workflow, he was presented with the interface for the first time during the case study process. He was focused on evaluating how easy it was for data custodians to find examples of disclosures through PRIVEE and subsequently audit their data repository. 

Our collaborator started by choosing the New Orleans Open Data portal~\cite{NewOrleans:online} and observed $7$ datasets on the Projection View. Since these datasets were so similar in their attribute space, they were displayed using an overlapping circle with the number of datasets inscribed. Using the attribute distribution bar chart, he observed that none of the default privacy-related attributes (age, race, gender) were present in this group of datasets. However, on analyzing the word cloud, he made an interesting observation that attributes like \textit{victim age} and \textit{offender age} were present in these datasets~\textbf{(T1)}. From his background knowledge, he knew that these attributes are generally present in police datasets. Hence he updated the list of privacy-related attributes to select some of the similar attributes like \textit{victim age}, \textit{victim gender}, \textit{victim race}, and \textit{offender age}. Since PRIVEE helps to triage the joinable groups of datasets based on the data defender's definition of privacy relevance, the Projection View was updated to reflect the change in privacy-related attributes. 

He selected all these seven datasets in order to compare the joinability risks of the $21$ possible pairwise combinations in the Risk Assessment View~\textbf{(T3)}. Since he wanted to focus only on the high-risk pairs, he filtered out the low-risk pairs using the Risk Score Distribution histogram. Next, he selected the first pair of datasets, \textit{Electronic Police Report 2018} and \textit{Electronic Police Report 2019}, and observed that some attributes like \textit{location}, \textit{victim age}, \textit{offender age}, \textit{victim race}, and \textit{offender race} were automatically suggested as the attributes for the join key. PRIVEE suggests these attributes based on a custom algorithm that focuses on the attributes profile and the definition of privacy-relevance by the data defender (Section \ref{sub_section:metrics_joinability_risk}). Joining these datasets, our collaborator observed that there are no matching records between these datasets.

He further selected the next pair of datasets, namely \textit{Electronic Police Report 2018} and \textit{Electronic Police Report 2016}, and joined them using the join key attributes suggested by PRIVEE. He observed that these datasets have $23$ matching records, which can be evaluated using the modified parallel sets visualization in the Disclosure Evaluation View \textbf{(T4)}. He made an interesting observation that matching records have a similar racial profile between the victim and the offender. Next, he selected another pair of datasets, namely \textit{Electronic Police Report 2016} and \textit{Electronic Police Report 2015}, but augmented the PRIVEE-suggested join key attributes and made the following selection: \textit{location}, \textit{victim age}, \textit{offender age}, \textit{victim race}, \textit{victim gender}, \textit{offender gender} \textbf{(T3)}. He joined these datasets and observed $14$ matching records in the Disclosure Evaluation View. He inspected further details about a certain record and observed that a 22-year-old black male was charged with attempted robbery with a gun against a 27-year-old white male at 6XX Tchoupitoulas St on 13th July 2015 at 01:00 hrs and again on 30th April 2016 at 03:00 hrs with attempted simple robbery. Next, from the feature suggestions offered by PRIVEE~\textbf{(T5)}, he selected the attribute \textit{disposition}, which shows the status of a particular incident. He observed that only one record was open in 2015 but closed in 2016. On inspecting further details, he found out that an incident of a runaway female juvenile of age 17 was reported at 85XX Dinkins St on 26th February 2015, and the same incident was closed through a supplemental report one and half years later on 7th December 2016.

Our collaborator commented that this is an example of identity disclosure where individuals were identified using PRIVEE even when the addresses were partially masked in de-identified datasets. During the case study, he was also shown an earlier version of the PRIVEE interface. He commented that the new changes "\textit{improved the rich functionalities}" of PRIVEE and added that this interface could "\textit{help experienced data custodians analyze disclosure risks and potentially find examples of disclosures}".

\begin{figure*}[t]
\begin{center}
\includegraphics[width=\textwidth]{figures/case_study1.pdf}
\vspace{-4mm}
 \caption{\label{figs:case_study2}\textbf{Case Study 2} This view shows the relationship between the join key attributes in the matching records using a modified parallel set visualization \kaustav{duplicate;placeholder image}}
\end{center}
\vspace{-4mm}
\end{figure*}

\subsection{Case Study 3}\label{section:case_study3}
In this sub-section, we report another case study

==> sections/old/data_collection_and_analysis_process.tex <==
\section{Open Data Analysis Process}

\aritra{Disagree with this section. The analysis and visualizations must be combined in units of tasks and design requirements, derived from the Ts. As part of these design requirements you should describe the complementary roles of automation and visualization.}

During the red-teaming exercise, we collected multiple open datasets. In this section, we structure the process undertaken to analyze these datasets, leading to the subsequent development of the interface for PRIVEE. 
% \subsection{Collecting Datasets}
% During our initial exploration, we collected  $39,507$ datasets from around $500$ data portals along with their metadata like tags, the number of records, attribute names, etc., which can help guide the selection of a seed set of relevant datasets \textbf{(T1)}. We observed through an automated analysis that about $5404$ datasets have some combinations of quasi-identifiers like age, gender, race, and location. Many datasets are related to non-human objects like buildings, animals, etc. We filtered out these datasets along with other non-relevant datasets, leading to the development of a seed set of $426$ datasets, including $151$ individual record-level~(e.g., records of people committing crimes) and $275$ aggregated record-level~(e.g., records of schools) datasets. Different experiments were conducted on these datasets to develop a strategy to help find disclosures when datasets are joined together.

\subsection{Finding Joinable Datasets}~\label{section:joinable_groups}
\kaustav{subsections titles are in continuous tense since these section are being mapped with their corresponding subsections in Section 6 (Design of PRIVEE)}
Two datasets can have some attributes which are shared between both datasets. Since the joinability of two datasets is actually a function of these \textit{shared attributes}, the intuition here is that the datasets with similar attributes should be more joinable. But the names of attributes of these open datasets are often noisy and inconsistent, making it computationally difficult to perform a binary search for the presence or absence of certain attributes. At the same time, the attribute names capture the semantic similarity between multiple datasets that might capture a similar context. We use a word-embedding approach that simultaneously satisfies the need to capture datasets' joinability and their semantic similarity.

\subsubsection{Converting Data Attributes to Word Embeddings}
Word embeddings can be defined as real-valued, fixed-length, dense, and distributed representations that can capture the lexical semantics of words~\cite{bakarov2018survey, almeida2019word}. Hence, we converted the data attributes into their corresponding word embedding form using Python's spaCy library~\cite{Spacy}. 

These vector word embedding representations of the attributes help to perform multiple useful operations like addition, subtraction, distance calculation, etc.; hence we used them to form a vector representation for the attribute space of each dataset~\cite{almeida2019word}. All the datasets were represented by a corresponding vector representation of their attributes at this stage. The vectors with a smaller distance between themselves signify datasets with similar attributes, hence more joinable.

\subsubsection{Adding Weights for Privacy-related attributes}
At this stage, all the data attributes have equal importance in the vector representation of a dataset. So, a dataset A with the attribute \textit{version number} may be marked similar to another dataset B with an attribute named \textit{version}. But these attributes may not have much significance in the context of privacy. Hence, we decided to add weights to some of the privacy-related attributes identified from the seed dataset corpus. Attributes like \textit{age}, \textit{race}, \textit{gender}, \textit{age at arrest} were selected, and adding more weights to these attributes signifies that datasets having these attributes may be marked as more joinable. Any disclosure using these datasets can be considered a high-risk, which will help triage the dataset pairs down the stream.


Cosine similarity is widely used to measure the similarity between words and documents~\cite{thongtan2019sentiment, dai2015document}. But word embeddings are mere representations of the words, and multiplying them with numeric weights would not increase the cosine similarity between two datasets. Hence we introduced a \textit{weight vector} where we assign a weight if the privacy-related attributes selected by the data defender are present in the dataset. Suppose dataset A has the \textit{age} attribute while Dataset B has the \textit{age} and \textit{race} attributes. If the data defender selects the privacy-related attributes [\textit{age, gender, race}], then the corresponding weight vectors would be $[x,0,0]$ and $[x,0,x]$ respectively, where $x$ represents the weight assigned to the privacy-related attributes. We concatenate these weight vectors with the corresponding word embedding vectors to get the final vector representation of each dataset. More details about the experiments conducted to identify the privacy-related attributes and the optimal weights can be found in the supplementary materials.


\subsubsection{Projecting the datasets and finding Clusters}
Each dataset has now been represented by a vector with more than $300$ elements/dimensions. Comparing these datasets using a 2-D or 3-D plot would be challenging if all the dimensions were used. Hence we used the t-SNE dimensionality reduction algorithm to reduce the vectors of $300$ dimensions into two dimensions, which will be easy to plot on a 2-D scatterplot~\cite{van2008visualizing}. 

A 2-D projection of the datasets might not readily reveal dataset groupings. We experimented with clustering algorithms like KMeans~\cite{vassilvitskii2006k}, DBSCAN~\cite{ester1996density,schubert2017dbscan}, Birch~\cite{zhang1996birch}, and OPTICS~\cite{ankerst1999optics, schubert2018improving}. After careful analysis of the clusters' quality and the cluster density scores, we selected the DBSCAN algorithm for PRIVEE. Additional details about the experiment can be found in the supplementary materials.

\subsubsection{Evaluating the clusters}
There can be multiple groups of similar/joinable datasets, which would lead to the creation of multiple clusters. A data defender may find it challenging to evaluate all of these clusters. Hence we have employed a few cluster evaluation techniques to rank these clusters \textbf{(T3)}. 

One of such metrics is the \textit{Calinski-Harabasz Index} which is defined as the ratio of the between-cluster dispersion and the inter-cluster dispersion,  where dispersion means the sum squared distance between the samples and the barycenter~\cite{calinski1974dendrite}. A higher score signifies that the different clusters are far away, implying better cluster formation. We designed an experiment to evaluate the difference in the results from this metric along with other metrics like Silhouette Score~\cite{rousseeuw1987silhouettes} and Davies-Bouldin Index~\cite{davies1979cluster} and selected the Calinski-Harabasz Index as the metric of choice. Further details about this experiment can be found in the supplementary materials. We perform automated calibration of cluster quality using the Calinksi-Harabasz Index metric that ensures we can efficiently guide defenders in finding meaningful, joinable datasets.


\subsection{Finding vulnerable datasets}~\label{section:vulnerable_entry_points}
Another potential entry point is finding vulnerable datasets from the open data ecosystem that can be joined with other datasets to find more information about the vulnerable records. To identify such datasets, we analyzed all the seed datasets and recorded the frequency distribution of the values of the attributes \textbf{(T2)}.

This helped us identify those datasets with a low record for a particular value of the privacy-related attributes. We even improved this further to rank these datasets based on their degree of vulnerability. Datasets with more such vulnerable attributes are ranked higher than those with only one such vulnerable attribute.

\subsection{Analyzing the risk in dataset pairs} \label{section:risk_score_calculation}
There can be multiple pairwise combinations of datasets from a group of joinable datasets. Moreover, the vulnerable datasets can also be joined with other individual record-level datasets to find possible disclosures. For example, a group of $10$ datasets can lead to $45$ possible pairwise combinations, and a vulnerable dataset can be linked with all the individual record-level datasets, resulting in $151$ pairwise combinations. In order to help the data defenders triage these combinations, we have implemented three metrics \textbf{(T4)}:

\subsubsection{Metric based on attribute profile}
Shannon’s entropy is a measure of the uncertainty of a random variable~\cite{cover1999elements}. It has been widely used as a privacy metric~\cite{serjantov2002towards,diaz2002towards,oganian2003posteriori,alfalayleh2014quantifying}, as higher entropy of an attribute in a dataset signifies more unique values for that attribute, thus resulting in higher disclosure risk. Hence, we used this metric to help defenders find joinable attributes for a pair of datasets. For each pair of datasets, we calculated Shannon's entropy of each of their shared attributes according to equations~\ref{equation:entropy_A} and~\ref{equation:entropy_B}. We used equation~\ref{equation:entropy} to calculate the final entropy score for that attribute. The intuition here is that the attributes with higher entropy can be offered as suggestions to the defender for the join key; hence the shared attributes are sorted according to their final entropy score in descending order.
\begin{equation}
    H(X_{A}) = -\sum_{i=1}^{n} P(x_{A_{i}}) \ln P(x_{A_{i}})
    \label{equation:entropy_A}
\end{equation}
\begin{equation}
    H(X_{B}) = -\sum_{j=1}^{m} P(x_{B_{j}}) \ln P(x_{B_{j}})
    \label{equation:entropy_B}
\end{equation}
\begin{equation}
    H(X) = \max\{H(X_{A}), H(X_{B})\}
    \label{equation:entropy}
\end{equation}
where:
\begin{description}
\item [$H(X)$] = entropy of an attribute present in two datasets A and B
\item [$X_{A}$] = attribute X in dataset A,
\item [$X_{B}$] = attribute X in dataset B,
\item [$x_{A_{i}}$] = each category of the attribute $X_{A}$ in dataset A,
\item [$x_{B_{j}}$] = each category of  the attribute $X_{B}$ in dataset B.
\item 
\end{description}

\subsubsection{Metric based on dataset pairs in a join}~\label{section:joinability_risk}
Since the joinability of two datasets depends upon the number of shared features/attributes between them, the joinability risk score can be calculated as a function of the number of shared attributes and the number of privacy-related attributes between a pair of candidate datasets. The formulae for the \textit{joinability risk score} can be defined as follows:
\begin{equation}
    \text{risk} = \alpha * p + (c-p)
    \label{equation:risk_score}
\end{equation}
where:
\begin{description}
\item [$\alpha$] = a constant, representing the empirical risk ratio
\item [p] = the number of privacy-related attributes,
\item [c] = the number of shared attributes
\end{description}
The joinability risk score depends on the empirical risk ratio, and to determine its value, we designed an experiment to calculate the risk scores of all the possible combinations of joinable pairs from the seed datasets ($\Comb{426}{2} = 90,525$ combinations). 
This experiment was repeated multiple times, each time with a different value of the risk ratio, ranging from $1$ to $100$. We observed that the value $\alpha = 50$ works well to separate the dataset pairs with privacy-related attributes and pairs without them. Hence the empirical risk ratio was fixed at the value of $50$. If two datasets have $15$ shared attributes and only $2$ of them are privacy-related attributes, the risk score can be calculated as $113$, as per equation \ref{equation:risk_score}. A higher joinability risk score signifies that this dataset pair is highly joinable, which can be a step closer to finding disclosures.
We have included further details about these experiments in the supplementary materials.

\subsubsection{Metric based on dataset relevance}
Joining a vulnerable dataset with all the individual record-level datasets is a reasonable idea since further details may be observed about a vulnerable record when joined with these datasets. But some datasets, though they can be joined together, may not contain any records for the vulnerable values. Hence we have developed a \textit{relevance score} to rank those datasets higher than those that do not have these vulnerable records. Record points are the unique values for a specific attribute, while vulnerable record points are those record points that have very few records for them, as shown in equation \ref{equation:record_points}. Some of the sample record points are shown in Table \ref{table:record_points}. The relevance score can be defined as a percentage of the number of vulnerable record points from dataset A present in dataset B, as described in equation \ref{equation:relevance_score}. The intuition here is if the same vulnerable records of a vulnerable dataset are present in another dataset, that dataset pair becomes quite a risk, thus leading to possible disclosures.  
\begin{equation}
    \text{record point} = [a, v, c]
    \label{equation:record_points}
\end{equation}
\begin{equation}
    \text{relevance score} = |V_{A} \cap R_{B}| / |V_{A}|
    \label{equation:relevance_score}
\end{equation}
where:
\begin{description}
\item [a] = attribute name,
\item [v] = value of the attribute,
\item [c] = count of the records with this value of the attribute,
\item [$V_{A}$] = vulnerable record points in Dataset A (where c is low),
\item [$R_{B}$] = record points in Dataset B,
\item [$|x|$] = the cardinality of the variable x,
\end{description}

\begin{table}[h!]
    \centering
    \begin{tabular}{|c|c|}
    \hline
     \textbf{Record points} & \textbf{Description} \\ 
     \hline
     [“age”, 11, 1] & For the age=11, there is only 1 record \\ 
     \hline
     [“age”, 15, 5] & For the age=15, there are 5 records \\
     \hline
     [“gender”, “other”, 2] & For the gender=“other, there are 2 records \\
    \hline
    \end{tabular} %\break
    \caption{Sample record points}
    \label{table:record_points}
\end{table}

\subsection{Identifying disclosures} \label{section:mutual_information} \label{section:disclosure_detection}
The goal of PRIVEE is to help data defenders find evidence of possible disclosures by analyzing the dataset pairs \textbf{(T5)}. We have developed two methods in this regard:

\subsubsection{Based on the low frequency of matching record}
\textit{Matching records} are the number of records in the joined dataset. The presence of matching records can indicate the possible disclosures at the record level. But the number of matching records may vary according to the choice of joining attributes and the type of records present in the datasets. For example, dataset A and dataset B, when joined on attributes $x$ and $y$, may have $200$ matching records, but when joined on the attributes $x$, $y$ and $z$, may have only $20$ matching records. This implies that the attribute combination $x$, $y$, and $z$ have a better chance of discovering an actual disclosure than the combination $x$ and $y$. PRIVEE employs an algorithm for the automatic selection of the join keys, which can also be augmented by the data defender. This algorithm selects a combination of those shared attributes which are also present in a pre-calculated list of privacy-related attributes along with the shared attributes with high entropy level.   We have also observed that matching records may contain duplicates if the original datasets have duplicate or blank entries. 

\subsubsection{Based on the mutual information between the joining attributes}
The selection of the joining attributes is an iterative process in PRIVEE. We use normalized mutual information to suggest other features that defenders can use for detecting disclosures. Mutual information measures the amount of information one random variable contains about another~\cite{cover1991entropy} and quantifies the mutual dependence of the two attributes of a dataset. We calculated the normalized mutual information between the joining attributes and the other attributes of the joined dataset. Next, we find the top-$5$ attributes with the highest mutual information score and let defenders consider those features for detecting matches \textbf{(T6)}.


%% ------ Old content --------
% \subsection{Datasets curation}
% As mentioned earlier, we have collected a seed set of 426 datasets. These datasets were further curated in order to determine their granularity. 151 of these datasets individual record-level (e.g., records of people committing crimes) while 275 were aggregated record-level (e.g., records of schools). We also collected the tags related to each of the datasets since we realized that users may like to view datasets related to a certain tags like health, education crime etc.

% \subsection{Finding Similar Datasets}
% The intuition here is that datasets with similar attributes should be more joinable since the joinability of the two datasets is a function of their shared attributes. But the names of attributes of these open datasets are often noisy and inconsistent, making it computationally difficult to perform a binary search for the presence or absence of certain attributes. At the same time, the attribute names capture the semantic similarity between multiple datasets that might capture a similar context. We use a word-embedding approach that simultaneously satisfies the need to capture the joinability and semantic similarity of datasets.

% \par \noindent \textbf{Applying Word2Vec with Data Attributes:} Word2Vec is available from the Python spaCy library. It converts each data attribute into a numeric vector form\cite{Spacy}. These vectors are then used to form a high-dimensional vector representation of the attribute space of a dataset which can be used to analyze their similarity. For example, the attributes "age" and "race" were represented by two different vectors of size 1 X 300, which were again used to form a vector representation for the attribute combination "age race". Hence, we used the t-SNE dimensionality reduction algorithm, which converts these high dimensional vectors into lower-dimensional embedding, using the cosine similarity between vectors~\cite{van2008visualizing}.  

% \textit{Weight selection for privacy-related attributes:\label{subsection:weight_selection}} We use the default privacy-related attributes collected during the red-teaming activity in the process of finding joinable groups of datasets. We first created a weight vector representing the presence of these attributes, along with the vectors obtained from Word2Vec. For example, if Dataset A has only the age attribute while Dataset B has the age and race attributes, then the corresponding vectors for the presence of the privacy-related attributes [age, gender, race] would be $[x, 0,0]$ and $[x,0,x]$ respectively, where $x$ represents the weight assigned to the privacy-related attributes. Once we obtained this weight vector, we concatenated this with the vector obtained from training a Word2Vec model on our datasets. 

% \par \noindent \textbf{Clustering in the projected space:} A 2-D projection of the datasets might not readily reveal dataset groupings. Hence, we used the DBSCAN clustering algorithm to computationally analyze these vectors and find groups of datasets between them\cite{ester1996density,schubert2017dbscan}.  This helped to effectively find groups of datasets joined together on their shared attributes. We also evaluated the different clustering algorithms and how they perform in this scenario. Using different values of the weights and the privacy-related attributes age, gender, and race, the DBSCAN and OPTICS clustering algorithms performed more or less similar. Still, the algorithms KMeans and Birch did not give any meaningful clusters \cite{ankerst1999optics,vassilvitskii2006k,zhang1996birch}.  But we chose DBSCAN algorithm in this interface since it has better scores than OPTICS at different combinations of the privacy-related attributes.

% \par \noindent \textbf{Clustering evaluation:} We designed an experiment to ascertain the optimum value for $x$ by evaluating the cluster results using metrics like the \textit{Calinski-Harabasz Index}. The latter  is defined as the ratio of the between-cluster dispersion and the inter-cluster dispersion,  where dispersion means the sum squared distance between the samples and the barycenter\cite{calinski1974dendrite}. Higher score signifies that the clusters are far away, which implies better clusters. After comparing the results at different weights, $x=8$ and $x=17$ were chosen as the candidate weights for the vector for the privacy-related attributes. Since the clusters may change dynamically with the change in privacy-related attributes, the candidate weights (weight = $8$ and $17$) are used to generate the clusters. We also perform automated calibration of cluster quality using the Calinksi-Harabasz Index metric that ensures we can efficiently guide defenders in finding meaningful, joinable datasets.  We have included more details about these experiments in the supplementary materials.

% \subsection{Vulnerable Datasets}
% % \begin{figure}
% % \begin{center}
% % \includegraphics[width=\columnwidth]{figures/vulnerable_entry_points_v2.pdf}
% % \vspace{-4mm}
% %  \caption{\label{figs:vulnerable_entry_points}\textbf{Diagnosis of vulnerable entry points.} (a), (b), (c):  filters help in the selection of datasets based on their metadata and the data portals, and (d) exposing the vulnerabilities in the data distributions, where bins with too few records are colored in red.}
% % \end{center}
% % \vspace{-8mm}
% % \end{figure}

% The red-teaming exercise helped us exploit multiple entry points into the open data ecosystem and demonstrated the need for guiding defenders' risk analysis strategy with meaningful selections. As a defense strategy and a corresponding design requirement, PRIVEE achieves tasks T1~(metadata-based selection) and T2~(selections based on vulnerable data sets) by providing defenders the \textit{flexibility} to explore multiple reconnaissance strategies.

% \par \noindent \textbf{Selections based on tags and privacy-relevance}: We observed that the open datasets are already enriched with metadata information like the popular tags relevant to them. Thus, we designed a tag selection filter where defenders can select the tags pertinent to them. But, a defender, unaware of the popular keywords, may not effectively filter the seed datasets. Hence, PRIVEE can guide the user through the dataset selection process using a sorted bar chart view which highlights the frequency of each of the tags (\textbf{T1})~(Figure \ref{figs:vulnerable_entry_points}c). We use the red color throughout the interface to indicate risk or vulnerability.
% We used a metadata dictionary of privacy-related attributes which can aid in finding datasets of interest (\textbf{T1}). Individual-level datasets were analyzed and a list of attributes was identified which are related to the quasi-identifiers age, gender, and race.  Some of the privacy-related attributes are as follows: "age\_group", "vic\_age\_group", "susp\_age\_group", "perp\_age\_group", "vict\_age","age\_1", "age\_at\_release", "admission\_age", "age\_class", "subject\_age", "patient\_age", "age\_range", "offender\_age", "officer\_age", "age\_at\_arrest","sex", etc.. Users can choose any combination of these attributes through \textit{PRIVEE} as an initial selection that can be modified later.

% \par \noindent \textbf{Selections based on data granularity}: The $426$ datasets seed datasets we collected belong to $102$ data portals. In PRIVEE,  we allow defenders to analyze the risk profiles of the datasets by the specification of any preferred data portal~(Figure \ref{figs:vulnerable_entry_points}b) (\textbf{T1}).
% Risk profile may be different for datasets with \textit{individual records} where each record corresponds to a single individual, like arrests dataset, medical records; or with
% \textit{aggregated records, } where each record corresponds to the aggregated values for a certain category, like disease infection in a county, education levels in a district etc. PRIVEE offers the option to select a subset of these pre-labeled datasets~(i.e., as individual level or aggregate level) based on the granularity of the records, thus augmenting the dataset selection process with user's input (\textbf{T1})~(Figure \ref{figs:vulnerable_entry_points}a).  

% \par \noindent \textbf{Sorting vulnerable distributions}: PRIVEE helps the data defenders discover vulnerable datasets by showing the distribution of the privacy-related attributes. The vulnerable record categories are highlighted in bright red, thus guiding the user towards selecting datasets with such vulnerabilities (\textbf{T2})~(Figure \ref{figs:vulnerable_entry_points}d). PRIVEE also performs an automatic analysis of these distributions and sorts the datasets based on the degree of vulnerability present. For example, if a Dataset A has only $2$ records for race="Hawaiian" while Dataset B has $1$ record for age=19-20 and $1$ record for the race="Black", Dataset B will be displayed first, followed by Dataset A.

% \subsection{Metrics for evaluating joinability risk} \label{section:risk_score_calculation}

% \textbf{Based on attribute profile:} Shannon’s entropy is a measure of the uncertainty of a random variable ~\cite{cover1999elements}. It has been used as a privacy metric~\cite{serjantov2002towards,diaz2002towards,oganian2003posteriori,alfalayleh2014quantifying}, as higher entropy of an attribute in a dataset means more unique values for that attribute, thus resulting in higher disclosure risk. We used this metric to help defenders find joinable attributes for a pair of candidate datasets. For each pair of datasets, we calculated Shannon's entropy of each of their shared attributes according to equations \ref{equation:entropy_A} and \ref{equation:entropy_B}. We used equation \ref{equation:entropy} to calculate the final entropy score for that attribute. The intuition here is that the attributes with higher entropy can be offered as suggestions to the defender for the join key; hence the shared attributes are sorted according to their final entropy score in descending order.
% \begin{equation}
%     H(X_{A}) = -\sum_{i=1}^{n} P(x_{A_{i}}) \ln P(x_{A_{i}})
%     \label{equation:entropy_A}
% \end{equation}
% \begin{equation}
%     H(X_{B}) = -\sum_{j=1}^{m} P(x_{B_{j}}) \ln P(x_{B_{j}})
%     \label{equation:entropy_B}
% \end{equation}
% \begin{equation}
%     H(X) = \max\{H(X_{A}), H(X_{B})\}
%     \label{equation:entropy}
% \end{equation}
% where:
% \begin{description}
% \item [$H(X)$] = entropy of an attribute present in two datasets A and B
% \item [$X_{A}$] = attribute X in dataset A,
% \item [$X_{B}$] = attribute X in dataset B,
% \item [$x_{A_{i}}$] = each category of the attribute $X_{A}$ in dataset A,
% \item [$x_{B_{j}}$] = each category of  the attribute $X_{B}$ in dataset B.
% \item 
% \end{description}
% \textbf{Based on dataset pairs in a join:}
% %Joining attributes are the number of common attributes between two datasets. 
% Since the joinability of two datasets depends upon the number of shared features/attributes between them, the joinability risk score can be calculated as a function of the number of shared attributes and the number of privacy-related attributes between a pair of candidate datasets. The formulae for the joinability risk score can be defined as follows:
% \begin{equation}
%     \text{risk} = \alpha * p + (c-p)
%     \label{equation:risk_score}
% \end{equation}
% where:
% \begin{description}
% \item [$\alpha$] = a constant, representing the empirical risk ratio
% \item [p] = the number of privacy-related attributes,
% \item [c] = the number of shared attributes
% \end{description}

% % \begin{figure*}
% % \begin{center}
% % \includegraphics[width=\textwidth]{figures/risk_assessment_v2.pdf}
% %  \caption{\label{figs:risk_and_disclosure}\textbf{Comparison of joinability risk and detection of disclosures.} (a) the distribution of the privacy-relevant attributes in the joinable dataset pairs and (b) their risk score distribution. (c) a joinable pair with a sorted bar chart of the shared attributes between them while (d) their joinability risk. (e) visualizing the shared records when the datasets are joined using the privacy-relevant attributes while (f) the data distribution of the attributes having high mutual information with the joining attributes. (g) a record with where an individual can be identified even if the location is partially masked.}
% % \end{center}
% % \vspace{-2mm}
% % \end{figure*}

% The joinability risk score depends on the empirical risk ratio, and to determine its value, we designed an experiment to calculate the risk scores of all the possible combinations of joinable pairs from the seed datasets ($\Comb{426}{2} = 90,525$ combinations). 
% %Since there are a total of $426$ datasets, this experiment calculated the risk score of $\Comb{426}{2}$ i.e., $90,525$ pairwise combinations of datasets. 
% This experiment was repeated multiple times, each time with a different value of the risk ratio, ranging from $1$ to $100$. We observed that the value $\alpha = 50$ works well to separate the dataset pairs with privacy-related attributes and pairs without them. Hence the empirical risk ratio was fixed at the value of $50$. If two datasets have $15$ shared attributes and only $2$ of them are privacy-related attributes, the risk score can be calculated as $113$, as per equation \ref{equation:risk_score}. A higher joinability risk score signifies that this dataset pair is highly joinable, which can be a step closer to finding disclosures.
%  We have included further details about these experiments in the supplementary materials.

% \subsection{Metrics for evaluation of disclosures} \label{section:mutual_information}


% \textbf{Based on the low frequency of matching records:} Matching records are the number of records in the joined dataset. The presence of matching records can indicate the possible disclosures at the record level. But the number of matching records may vary according to the choice of joining attributes and the type of records present in the datasets. For example, Dataset $A$ and Dataset $B$, when joined on attributes $x$ and $y$, may have $200$ matching records, but when joined on the attributes $x$, $y$ and $z$, may have only $20$ matching records. This implies that the attribute combination $x$, $y$, and $z$ have a better chance of discovering an actual disclosure than the combination $x$ and $y$. We have also observed that the number of matching records may contain duplicates if the original datasets have duplicate or blank entries. 

% \noindent\textbf{Based on the mutual information between the joining attributes:} The selection of the joining attributes is an iterative process in PRIVEE. We use normalized mutual information to suggest other features which defenders can use for detecting disclosures. Mutual information is the measure of the amount of information one random variable contains about another~\cite{cover1991entropy} and quantifies the mutual dependence of the two attributes of a dataset. We calculated the normalized mutual information between the joining attributes and the other attributes of the joined dataset. Next, we find the top-$5$ attributes with the highest mutual information score and let defenders consider those features for detecting matches.

==> sections/old/design_of_privee.tex <==
\section{Design of PRIVEE}
In this section, we describe the design process of PRIVEE along with the reasons for the visualization choices.

\aritra{all the subsections can become sections on their own. Try to avoid sub-subsectios as much as possible. Also, if you notice the naming of the subsubsectios: under Projection view, you have projection plot. It makes no sense. And then you have Attribute Distrubtion at the same level, that is not a visualization type. Whenever patterns like these exist, these are symptomatic of confusion in the author's thought process and articulation. The remedy is to think carefully about what the top-level sections should be. Again, rather than I telling you what to do, you can read relevant design study and application papers and come up with ideas about better structuring of the content.}

\subsection{Projection View: Finding joinable datasets}
The design of PRIVEE is inspired by \textit{Shneiderman's Visual Information-Seeking Mantra}: Overview first, zoom and filter, then details-on-demand~\cite{shneiderman2003eyes}. The Projection View provides an overview of the datasets and the joinable groups between them \textbf{(T3)}. These groups can be modified based on the information from different components of this view, which are described as follows:

\subsubsection{Projection Plot}
Given a set of datasets, defenders need to find groups of datasets that can be joined together \textbf{(G3)}. As discussed in this paper by Gnadesikan et al., clusters or groups can be represented using a projection plot~\cite{gnanadesikan1982projection}. Hence, we have developed a multi-dimensional projection plot to represent the joinable groups, as illustrated in Figure~\ref{figs:projection_view}. Here,  each red dot represents a dataset in the group of $10$ joinable datasets from the initial selection of datasets. The dots not in this group are represented by grey color.  


This view contains small multiples of the projection plots, where each plot represents a group of joinable datasets. It helps the data defender quickly compare the different groups from a single view. The dual color encoding scheme (red-grey) helps visually differentiate between the datasets in a group and the other datasets. Initially, a scatterplot with different colors for the different clusters was also considered for this view. However, it was realized that due to the limits of perception, it is challenging to assign perceptually different colors to each cluster when the number of clusters is large. Hence, a small multiple design approach was chosen with the two-color encoding scheme.

\subsubsection{Attribute Distribution}
Understanding the cluster signatures is crucial in understanding the reason behind the genesis of a joinable group \textbf{(T3)}. Since we have construed these dataset groups based on their similarity in their attribute space, it is essential to understand the frequency of the attributes present in these groups. Hence, bar charts become the natural choice for displaying the most frequent attributes in a group along with their frequency. Though these bar charts are sorted according to the attribute frequency in descending order, the frequencies of the privacy-related attributes are shown at the top since these attributes are given more weightage while developing the groups. Understanding the difference in frequency distribution can help the data defenders understand the reason behind the formation of different clusters. These attributes are color-coded (in crimson red) throughout the interface.


However, bar charts can have the limitation of visual scalability where only a certain number of bars can be shown due to space constraint~\cite{eick2002visual}. This will limit the data defenders' understanding of the cluster signatures to only the top few attributes.

\subsubsection{Word Cloud}
In order to overcome the limitation of visual scalability of the bar charts, we also introduce word clouds of the attributes. All the attributes present in at least two datasets in a joinable group are represented in this word cloud, with the size visual channel representing their frequency. One can also observe the coherence between the attribute distribution bar chart and the word cloud since the attributes with the most frequency in the bar chart are also shown in a larger size in the word cloud. 

Besides overcoming the visual scalability limitation of the bar chart, the word cloud also helps the data defenders look for other attributes of interest that may have a lower frequency than the other attributes but may have much larger relevance in the context of privacy. For example, attributes like \textit{victim\_age} and \textit{offender\_age} may not be significant for a general user. However, a data defender working with law enforcement may find them interesting since these attributes are used in the police datasets. The privacy-related attributes are not color-coded here since the objective behind the word clouds is to help the defenders explore other attributes and select potential privacy-related attributes. Color coding may introduce an unintended bias towards these attributes.
\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{figures/projection_view.pdf}
\vspace{-4mm}
 \caption{\label{figs:projection_view}\textbf{Projection View} This view shows a combination of the projection plot, the word cloud of attributes and their frequency distribution in the bar chart\kaustav{placeholder image}}
\end{center}
\vspace{-8mm}
\end{figure}

\subsubsection{Filter Bar}
We made an experience-based decision to select all the $151$ individual record-level datasets when a user visits PRIVEE for the first time. Thus, the projection view is loaded with the clusters for each joinable group from these datasets. A defender can progressively inspect each joinable group \textbf{(T3)}, starting from the top~(most vulnerable) to the bottom~(least vulnerable). Each group is represented by a projection plot, a bar chart, and a word cloud. But a defender may wish to select a different set of datasets based on the observations from the initial overview. Inspired by \textit{Shneiderman's mantra} of overview first, followed by zoom and filter, PRIVEE allows the defenders to filter the initial set of datasets based on various options. 

The filter bar, located conveniently at the top of the interface, contains a search option for the different tags and options to select the data portals and the dataset granularity \textbf{(T1)}. Defenders can select any combination of the tags from the tags search option, which is enriched with a modified bar chart showing the frequency distribution of the tags. Though the tags are sorted in descending order, the grey bar in the background (achieved by tweaking a linear-gradient bar) provides an idea of the frequency distribution of these tags among the seed collection of $426$ datasets.

PRIVEE also offers a wide choice of $102$ data portals, and the defenders may choose any combination of these portals. Another filter offers the option to filter datasets based on their granularity (individual or aggregate level records). The update button helps implement these filter choices by reloading the Projection View based on the datasets selected through these filters. This replicates the \textit{mantra} of overview implementation first, followed by zoom and filter strategy, as the defender can now work on only their desired subset of datasets. Since rendering the visual elements of the Projection View is computationally costly, this design choice mainly helps avoid the multiple re-renders of the view.


\subsection{Vulnerable Datasets View: Finding risky datasets}
The vulnerable datasets are another entry point into the open data ecosystem. Though there can be various vulnerabilities, we focus on the datasets with a very low count of records regarding a specific privacy-related attribute. Following \textit{Shneiderman's mantra}, this view shows an overview of the datasets and the distribution of the values of their privacy-related attributes through a bar chart. Smaller bars, for example, a bar representing only one record for the gender female, are highlighted in red. In contrast, the other bars are highlighted in grey, following the two-color scheme used in the Projection View. We believe that this two-color strategy will help the defenders find vulnerable attribute distribution faster. 

The datasets are sorted in ascending order with respect to the number of such vulnerable attributes. For example, a dataset with two such attributes will be ranked higher than a dataset with one vulnerable attribute. In case of a tie, the value counts of these attributes' vulnerable bins are considered secondary sorting criteria. This visualization design helps the defenders find vulnerable datasets and the vulnerable record value \textbf{(T2)}. Defenders can also filter the datasets present in this view using the filters available in the filter bar and update the attributes of interest based on their domain knowledge.


\subsection{Risk Assessment View: Analyzing the risk in dataset pairs}
PRIVEE's goal is to compare the joinability risks of different dataset pairs (G3). Defenders can either select a joinable group of datasets or a vulnerable dataset to update the Risk Assessment View. However, the number of possible pairwise combinations of the candidate datasets can be pretty high; hence PRIVEE can help a data defender analyze the risk of these datasets at the dataset and feature levels. The Risk Assessment View uses visual analytic components to encode these metrics so that data defenders can pro-actively analyze the risk between the candidate datasets. This view also implements Shneiderman's mantra since it provides the on-demand details for the datasets chosen from the Projection View or the Vulnerable Datasets View.
\begin{figure*}[t]
\begin{center}
\includegraphics[width=\textwidth]{figures/risk_view.pdf}
\vspace{-4mm}
 \caption{\label{figs:risk_view}\textbf{Risk View} This view shows the dataset pairs ranked according to their joinability risk score, along with the shared attributes between them\kaustav{placeholder image}}
\end{center}
\vspace{-4mm}
\end{figure*}
\subsubsection{Shared Attributes}
Since the joinability risk between two datasets depends on the attributes and the nature of these attributes, an initial design sketch suggested using a large rectangular box for the shared attributes, followed by the names of the datasets on either side of the box. The box was again divided into smaller rectangles, where each small rectangle represented a shared attribute. However, we realized that this leads to the loss of information about the hierarchy among these shared attributes. These attributes may not be equally important as a join key used to join these two datasets. We explored that the entropy of these attributes can be a suitable indicator of the importance of these attributes in the join key. Hence, a sorted bar chart was developed where the different shared attributes were encoded with the horizontal position visual channel while their relative entropy was encoded with the vertical position visual channel (Figure~\ref{figs:risk_view}). The bars for the privacy-related attributes are again colored in violet, while the other bars were colored in grey, thus following the similar two-color strategy used in the other views.

\subsubsection{Joinability Risk}
In order to highlight the joinability risk between these dataset pairs, PRIVEE has a joinability risk bar beside the shared attributes \textbf{(T4)}, as shown in Figure~\ref{figs:risk_view}. This bar is filled with a linear gradient between grey (less risk) and red (high risk). The same dual-color scheme is used in this context to achieve the goal of showing the joinability risk on a gradient \textbf{(G3)}. The exact risk score is highlighted using a black vertical bar.

Other design ideas were also explored before zeroing on this design. A text representation of the exact risk score was considered initially, which was later dropped since the defender may not need the exact value of the risk score. Another design similar to the star rating options available on e-commerce websites was also implemented. But this design suffered from the limitation of granularity, where two dataset pairs with different risk scores had to be assigned the same star rating (due to approximation). A gradient bar was finally chosen since it displays the granularity of the score despite providing a suitable level of abstraction.

A combination of the dataset names, shared attributes bar charts, and joinability risk bar is repeated for each dataset pair. Defenders can choose the dataset pair of their choice by selecting it through a radio button.

PRIVEE also offers a high-level view of the risk score distribution using a histogram in the top area of the Risk View. This histogram helps the defender understand the risk score distribution and allows them to filter based on low/high-risk scores \textbf{(T4)}.

\subsubsection{Attributes selection}
PRIVEE also helps the defenders understand the distribution of the privacy-relevant attributes in the dataset pairs' shared attributes. A horizontal bar chart beside the Risk Score Distribution histogram shows the distribution of the privacy-relevant attributes only, where these attributes are encoded using the vertical position visual channel while their frequency is encoded using the horizontal position visual channel. This orientation helps to utilize the horizontal space and helps alleviate space constraints to a certain extent.

Defenders can select any number of the shared attributes as the join key to join the datasets and evaluate them for disclosure. Selected attributes are highlighted using a bolder font weight. We realized that a defender might try different combinations of the shared attributes as the join key; hence it is important to track which attributes were selected while joining the last time. This is encoded using the color channel, where golden yellow is used to highlight all the attributes used as the join key in the earlier join activity.

\subsection{Disclosure Evaluation View: Identifying disclosures}
The goal G4 relates to the identification of the different cases of disclosure. This can be achieved by evaluating the matching records for a dataset pair with respect to a particular joining key. 
\begin{figure*}[t]
\begin{center}
\includegraphics[width=\textwidth]{figures/matches_view.pdf}
\vspace{-4mm}
 \caption{\label{figs:matches_view}\textbf{Matches View} This view shows the relationship between the join key attributes in the matching records using a modified parallel set visualization \kaustav{placeholder image}}
\end{center}
\vspace{-4mm}
\end{figure*}
\subsubsection{Matching records}
Matching records are the common records between two datasets when joined with a particular join key. Two types of disclosure can be observed using these records: identity disclosure and attribute disclosure. In identity disclosure, only a few records of a particular value of a specific attribute may help identify a certain person. While in attribute disclosure, all the records may have a similar value for a particular attribute. Both of these disclosures can be understood from a modified parallel sets visualization. Parallel sets is a visualization method for the interactive exploration of categorical data, which shows the data frequencies instead of the individual data points~\cite{kosara2006parallel}. We adopted and extended this technique for visualizing the relationship among the different categories of the privacy-relevant attributes in the joined dataset, yet retaining the granularity of the dataset at the record level. As illustrated in Figure~\ref{figs:matches_view}, each joining attribute is represented using a stacked bar, where the height of the stacks represents the frequency of the respective categories. A histogram replaces the stacked bar for numerical attributes to show their distribution. In this case, the numerical data is divided into four equal bins to map them with the categories of the other attributes. The categories in the different stacked bars are connected using weighted lines. Each line's weight/thickness represents the number of records in the joined dataset belonging to both categories. A simple click interaction on any of these lines opens a pop-up window showing the details of the highlighted record.

This design again follows Shneiderman's mantra, where PRIVEE first provides an overview of the matched records, then allows the defender to explore them by highlighting them, and finally lets the defender view the details of the records on demand. 

\subsubsection{Feature suggestions}
PRIVEE uses the normalized mutual information score to find the attributes similar to these joining attributes. As shown in Figure~\ref{figs:matches_view}, the data distribution of the attributes with the most mutual information with the joining attributes is shown on the left and right-hand sides of the modified parallel sets visualization. These attributes can be used as suggestions for improving the initial set of joining attributes (\textbf{T6}). Bar charts are used for showing the distribution of categorical attributes, while histograms are used for numerical attributes. These data distributions, along with the ranking of these attributes, helps boost the defender's understanding of the risky feature set, which can be used for the join key.


%% -------------- Old content -----------------
% \subsection{Filter Area}
% During early discussion with domain experts, it was evident that users may want to select a subset of datasets instead of all the dataset available to them, in order focus more on possible disclosure risk local to a certain type of dataset. PRIVEE has multiple filter options, baked right right at the top bar of the screen. The filter options include 

% \begin{enumerate}
% \item \textit{Type of dataset:} During dataset analysis, it was observed that datasets can have two type of records:
% \begin{itemize}
% \item \textit{individual records:} where each record corresponds to a single individual, like arrests dataset, medical records etc.
% \item \textit{aggregated records:} where each record corresponds to the aggregated values for a certain category, like disease infection in a county, education levels in a district etc.
% \end{itemize}
% Users can filter the datasets according to their type of records (see Figure \ref{figs:interface}a). PRIVEE has a collection of around $151$ individual-record level datasets and around $275$ aggregated-record level datasets.
% \item \textit{Popular tags:} The data portals label each datasets with few tags which generally portray the popular keywords related to each dataset. During the selection of datasets, the tags were analyzed for their frequency in this collected datasets. This sorted list of tags are available in the filter area (see Figure \ref{figs:interface}a) where the users can filter the datasets based on their tags/keywords of choice.
% \item \textit{Data portals:} As mentioned earlier, data experts may be interested in analyzing the datasets from a certain data portal only. This can be achieved by selecting the relevant data portals from the list of the portals available in the filter area (see Figure \ref{figs:interface}f). A complete list of the portals can be found in the appendix.
% \item \textit{Type of plot:} PRIVEE has two different types of plots available in order to cater to different attack scenarios. In order to implement the attack scenario through joinable datasets (Section \ref{section:attack_scenario1}), PRIVEE has projection plots along with the clusters, word cloud and the bar chart of the popular attributes. But in order to implement the attack scenario through unique records (Section \ref{section:attack_scenario2}), a different view of histograms can be loaded using the options available through the filter area (see Figure \ref{figs:interface}a)
% \end{enumerate}
% \subsection{Projection Plot}
% We show the cluster signatures that help defenders focus on joinable subsets in this view. The main component is a multidimensional projection plot, where, as illustrated in Figure \ref{figs:joinable_groups}a, each red dot represents a dataset in the group of $45$ joinable datasets from the candidate set chosen by a data defender. The dots, not in this group, are represented by grey color. To drill down into the features responsible for the clusters, we use a dual-encoding approach, with a word cloud showing the most frequent attributes for each joinable group and a bar chart showing the frequency of privacy-relevant attributes first, followed by others. This encoding is to help familiarize a defender with any cluster with respect to both its general context and its privacy relevance. We use a small-multiple approach for this combination of projection, word-cloud, and bar chart. A defender can progressively inspect each cluster, starting from the top~(most vulnerable) to the bottom~(least vulnerable).

% The word cloud in Figure \ref{figs:joinable_groups}b shows the presence the attributes \textit{victimgender} and \textit{victimrace}. Suppose defenders have a background knowledge that these attributes are generally present in police datasets. In that case, they can augment the initial list of privacy with these attributes along with other similar attributes like \textit{victimage} and  \textit{offenderage}. This interaction will lead to a dynamic grouping based on the user's understanding of the privacy-related attributes, which helps form a further fine-tuned group of highly joinable datasets. The fine-tuning is evident from \ref{figs:joinable_groups}c, which shows the new group with a smaller subset of $6$ datasets. The bar chart in Figure \ref{figs:joinable_groups}d shows that almost all the datasets in this group contain all the privacy-related attributes, thus helping the defender prioritize further inspection of this joinable group~(\textbf{T3}). 

% \subsection{Risk View}

% The number of possible pairwise combinations of the candidate datasets can be pretty high and PRIVEE can help a data defender analyze the risk of these datasets at the dataset and feature levels. The Risk Assessment View uses visual analytic components to encode these metrics so that data defenders can pro-actively analyze the risk between the candidate datasets.

% Each dataset pair is represented using a sorted bar chart, where the x-axis represents the shared attributes between them and the y-axis means the entropy score of each of these attributes. This encoding helps the user visually compare the number of shared attributes present in each dataset pair along with their risk profile. The bars for the privacy-related attributes are colored in salmon red to provide a quick visual guide towards understanding the relative importance of these attributes compared to the other shared attributes. Users can select any attribute combinations from this bar chart to join the datasets and evaluate them for actual disclosures. As illustrated in Figure \ref{figs:risk_and_disclosure}c,  the datasets \textit{Electronic Police Report 2016} and \textit{Electronic Police Report 2015} have $21$ shared attributes, including all of the $4$ privacy-related attributes.

% This high number of shared attributes leads to a high joinability risk score, as determined from equation \ref{equation:risk_score}. This information has been encoded in a colored gradient bar, as shown in Figure \ref{figs:risk_and_disclosure}e. The color gradient helps abstract the actual joinability risk score into a normalized format so that data defenders can visually determine the severity of the risk. Each of the dataset pairs is ranked according to their joinability risk score so that the ones with the higher joinability risk are shown at the top.

% PRIVEE also has a risk description section which can help the data defenders understand the overall risk profile of the dataset pairs in a joinable group of candidate datasets. Figure \ref{figs:risk_and_disclosure}a shows the distribution of the privacy-related attributes and highlights the fact that the privacy-related attributes are present in $10$ of the dataset pairs in this view. Figure \ref{figs:risk_and_disclosure}b shows the distribution of the actual risk score so that the user can map their real joinability risk to the abstracted version shown in the colored gradient bar (Figure \ref{figs:risk_and_disclosure}b). This distribution can also be used as a filter to view only those pairs of datasets within a specific range of risk scores (high/low).

% Ranking the different dataset combinations helps the defender to analyze the risk associated with each of the combinations (\textbf{T4}). The visual cues can help the defender choose a combination more prone to disclosure risk. After comparing these risks of the different pairwise combinations of datasets, defenders can select any pair with some of the joining attributes to understand the eventual join outcome.

% \subsection{Disclosure Evaluation View}
% In this view, we visualize the matching records of the joined datasets using a modified parallel sets visualization. Parallel sets is a visualization method for the interactive exploration of categorical data, which shows the data frequencies instead of the individual data points~\cite{kosara2006parallel}. We adopted and extended this technique for visualizing the relationship among the different categories of the privacy-relevant attributes in the joined dataset, yet retaining the granularity of the dataset at the record level. As illustrated in Figure \ref{figs:risk_and_disclosure}e, each joining attribute is represented using a stacked bar, where the height of the stacks represents the frequency of the respective categories. For numerical attributes, the stacked bar is replaced by a histogram to show their distribution. In this case, the numerical data is divided into four equal bins to map them with the categories of the other attributes. The categories in the different stacked bars are connected using weighted lines. Each line's weight/thickness represents the number of records in the joined dataset belonging to both categories.



% In Figure \ref{figs:risk_and_disclosure}g, we can observe that there is a thin line between the \textit{offenderage} $22$ and the \textit{location} "6XX Tchoupitoulas St". Further investigation shows the details of this actual record in a table pop-up view. This reveals that a $22$ year old black male was charged with attempted robbery with a gun against a $27$ year old white male at 6XX Tchoupitoulas St on $13$\textsuperscript{th} July, $2015$ at $01$:$00$ hrs and again on $30$\textsuperscript{th} April, $2016$ at $03$:$00$ hrs with attempted simple robbery. This is an example of identity disclosure where an individual was identified even when the address was partially masked (\textbf{T5}).





% \begin{figure*}
% \begin{center}
% \includegraphics[width=\textwidth]{figures/scenario1_v2.pdf}
% \vspace{-2mm}
%  \caption{\label{figs:case_study}\textbf{Case study with domain expert.} (a) the expert selected the datasets from the Albany Police Open Data portal, which are shown in the dataset joinability view, along with the popular attributes in these datasets, (b) the risk assessment view showed the pairwise combinations of these datasets and their joinability risk, (c) one of the pairs when joined on the quasi-identifiers age, sex, neighborhoodxy and date showed only $4$ matching records, (d) analyzing the records showed an example of identity disclosure where a person was stopped for field interview and was  cited just 3 minutes later~(Section \ref{section:case_study}).}
% \end{center}
% \vspace{-2mm}
% \end{figure*}

% PRIVEE uses the normalized mutual information score to find the attributes similar to these joining attributes. As shown in Figure \ref{figs:risk_and_disclosure}f, the data distribution of the attributes with the most mutual information with the joining attributes are shown in the left and right-hand side of the modified parallel sets visualization. These attributes can be used as suggestions for improving the initial set of joining attributes (\textbf{T6}).


==> sections/old/edit_casestudy.tex <==
\section{Case Study}

% \textbf{The tasks explained under the usage scenario and case study sections look quite similar. Since these are two different sections, I assume the goal of individual section is different. However the description looks same in both the cases.}

In this section, we report one of the case studies our data privacy collaborator and co-author co-developed using the web interface of \textit{PRIVEE}. He has about $20$ years of experience in the field of privacy-preserving data analysis and used PRIVEE as a privacy auditor. Specifically, he wanted to find out if there are any possible disclosure risk with the datasets published in the open data portals of police departments, where data about people committing crimes are recorded. It is important to note that some of the numbers mentioned this these usage scenarios may change if the datasets are updated by the respective data owners. 

%\subsection{Finding disclosure risk: privacy auditor's perspective (T1a, T2, T3)}
Our collaborator began by choosing the Albany Police Department\cite{AlbanyPolice:online} and observed $6$ individual-level datasets on the dataset joinability view~(Figure~\ref{figs:scenario1}a). He decided to analyze all the possible combinations of these datasets using the projection plot~(Figure~\ref{figs:scenario1}b). Datasets \textit{APD Arrests Dataset by Neighborhood} and \textit{APD Arrests Datasets by Patrol Zone} have the highest risk score and share a common unique identifier, namely \textit{arrestid}. This dataset pair has the highest risk score since they share $16$ joining attributes, including $2$ privacy-related attributes. Since \textit{arrestid} has the highest entropy among the other attributes, our collaborator decided to join these datasets based on \textit{arrestid} and observed that there may be $1607$ common records, i.e., $1607$ individuals may be present in both the datasets and new information may be disclosed by joining them~(Figure~ \ref{figs:scenario1}c) (\textbf{T3}). For example, \textit{arrestid} APD*$210001493$ mentions the arrest of a 21 year old white female in both the datasets. On closer analysis, he observed that these two are almost similar datasets, the attributes \textit{neighborhood} and \textit{patrolzone} can be disclosed by joining them, leading to potential leakage of sensitive information.

He followed this with analysis of the next pair of datasets, \textit{APD LEAD Dataset} and \textit{APD Arrests Dataset by Patrol Zone} and observed that they have common quasi-identifiers like \textit{race}, \textit{age} and \textit{sex}~Figure~\ref{figs:scenario1}b). He then joined these datasets using these quasi-identifiers but found no common records, concluding that these datasets can be combined safely without actual, record-level disclosure(\textbf{T3}). 
% She also repeats this same procedure for the next pair of datasets \textit{APD Arrests Dataset by Neighborhood} and \textit{APD LEAD Dataset} and observes that there are no common records between them, hence derives the same conclusion (see Fig \ref{figs:scenario1}b) (\textbf{T2},\textbf{T3}). 
He repeated this operation for another pair of datasets \textit{APD Arrests Dataset by Neighborhood} and \textit{APD Field Interview Cards Dataset by Neighborhood} by adding the location attribute \textit{neighborhoodxy}~(Figure~\ref{figs:scenario1}b) (\textbf{T2}). He observed $887$ common records, implying that these individuals may be identified through these datasets who were stopped for field interview and later arrested by the police. She observes that though the latter dataset does not provide any information about the reason for the field interview, joining this with the former dataset shows that a $28$-year old white male was interviewed in the Washington Park neighborhood at $09$:$08$ hrs on $1$\textsuperscript{st} December, $2020$ and was later arrested for trespassing on enclosed property at $12$:$32$ hrs (arrestid: APD*$200001760$). He found more such examples by joining the datasets \textit{APD Arrests Dataset by Patrol Zone} and \textit{APD Field Interview Cards Dataset by Neighborhood}  where an individual of the the same age and gender received a citation on the same date and at the same location at $2$:$48$ am, just $3$ minutes after the incident from the first dataset~(see the two arrows in Fig \ref{figs:scenario1}d). In his role as a privacy auditor, our collaborator flagged these datasets for record-level disclosure of sensitive information, an outcome of PRIVEE that can be used by data custodians for making decisions about applying anonymization methods for minimizing the disclosure risks. Our collaborator commented \aritra{todo}

%a $26$-year old black female was interviewed at $11$:$23$ hrs on $11$\textsuperscript{th} December, $2020$ and was later arrested at $21$:$25$ hrs for "assault with intent to cause physical injury" (arrestid: APD*$200001826$) (\textbf{T3}). Next, she joined the datasets \textit{APD Field Interview Cards Dataset by Neighborhood} and \textit{APD Traffic Citations by Neighborhood} on the attributes \textit{age}, \textit{sex}, \textit{neighborhoodxy}and  \textit{date} and observed $4$ common records between them (see Fig \ref{figs:scenario1}d) (\textbf{T2}). 




%She observed that $23$-year old male was stopped for field interview on $23$\textsuperscript{rd} January, $2021$ at $2$:$45$ am and since field interviews are normal routine stop and search activities by the police, this may seem a regular incident, but the other dataset informed her that 




% PRIVEE helped Amy rapidly implement the attack scenario with joinable datasets in order to find disclosure risks (see Section\ref{section:attack_scenario1}). Thus, she concluded that since there are several possible disclosures by linking the datasets available through the open data portal of this police department, she would recommend to the police administrators that this portal is thoroughly analyzed for further disclosures before releasing any new datasets.


% \begin{comment}

% \subsection{Finding disclosure risk: data custodian's perspective (T1a, T2, T3)} \label{section:scenario2}
% \begin{figure*}
% \begin{center}
% \includegraphics[width=\textwidth]{figures/scenario2.pdf}
% \vspace{-4mm}
%  \caption{\label{figs:scenario2}\textbf{Disclosure risk: data custodian perspective} (a) The wordcloud for the New Orleans police datasets shows victimage as a frequent attribute, hence user select victimage along with other similar attributes (b) Joins two datasets on these attributes along with the location attribute (c) Though the addresses are partially masked, it can be observed that a $22$ year-old black male was charged with attempted armed robbery and attempted simple robbery against a $27$ year-old at the same location on different dates. (Section \ref{section:scenario2}) }
% \end{center}
% \vspace{-6mm}
% \end{figure*}
% \kaustav{Tasks are similar to the first usage scenario but in this scenario, the user updates the privacy related attributes based on what he sees in the wordcloud}
% Kabir, a data custodian with the police department of the City of New Orleans is tasked with the release of the Electronic Police Report for the year $2021$. He wishes to know if there could be any disclosure risk by using the electronic police reports from the previous years. In our interface \textit{PRIVEE}, Kabir selects the open data portal of New Orleans and loads all the available datasets\cite{NewOrleans:online}. He observes from the wordcloud that the attribute \textit{victim\_age} has a higher frequency, hence selects this attribute along with other similar attributes like \textit{offender\_age}, \textit{offender\_gender}, \textit{victim\_gender}, \textit{victim\_race} and \textit{offender\_race} as the privacy-related attributes (Figure \ref{figs:scenario2}a) (\textbf{T1a}).





% Now, he selects all these datasets and analyzes all the possible combinations of these datasets in the Risk Explanation View (\textbf{T2}). Since the police electronic reports across all the years have similar attributes, he started with the datasets \textit{Electronic Police Report 2015} and \textit{Electronic Police Report 2016} and joined them on his previously-selected privacy-related attributes along with the attribute \textit{location} (see Figure \ref{figs:scenario2}b) (\textbf{T2}). At this point, Kabir made an interesting observation that though the addresses used in these datasets are partially masked (see the arrow in Figure \ref{figs:scenario2}c), there are $21$ common records when joined on these attributes. For example, a $22$ year old Black Male was charged with "ATTEMPTED ARMED ROBBERY (GUN)" against a $27$ year old White Male at 6XX Tchoupitoulas St on 2015-07-13 at 01:00 hrs and again on 2016-04-30 at 03:00 hrs with "ATTEMPT - SIMPLE ROBBERY" (see Figure \ref{figs:scenario2}c). Kabir notes this as an example of identity disclosure (\textbf{T3}).



% Next, he joins the datasets \textit{Electronic Police Report 2016} and \textit{Electronic Police Report 2017} on the same attributes and to his surprise, finds $26$ common records despite the fact that the addresses are partially masked (\textbf{T2}, \textbf{T3}). For example, a $25$ year old Black Male was charged with "VIOLATIONS OF PROTECTIVE ORDERS" against a $23$ year old Black Female at 6XX Canal St on 2016-12-10 at 12:29 hrs and again on 2017-11-27 at 02:18 hrs with "DOMESTIC ABUSE BATTERY". He again notes this an example of identity disclosure (\textbf{T3}).

% Next, he joins the datasets \textit{Electronic Police Report 2017} and \textit{Electronic Police Report 2018} on the same attributes and again finds $43$ common records (\textbf{T2}, \textbf{T3}). For example, a $41$ year old Black Male was charged with "SHOPLIFTING", witnessed by a $32$ year old Black Female at 82XX Earhart Bd on 2017-06-06 at 19:50 hrs and again on 2017-11-27 at 02:18 hrs. A similar incident was reported at the same location by the offender and witness of the same attributes on 2018-02-20 at 12:26 hrs (\textbf{T3}). Thus, Kabir concludes that there may be disclosure risk using the previous years' police report datasets, hence those risks need to be carefully analyzed before releasing a new police report dataset.

% \end{comment}


==> sections/old/interface_description.tex <==
\section{Analytical Components of PRIVEE}

\aritra{Describe the clustering algorithms and risk score here in two subsections}


PRIVEE has been designed as a guidance framework for evaluating disclosure risks. In this section, we will discuss its major components and the design procedure for them.
\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{figures/interface.pdf}
\vspace{-4mm}
 \caption{\label{figs:interface}\textbf{Different components of PRIVEE} (a) The filter area has options to select the type of dataset (individual/aggregated), type of plot (projection/histogram), filter the datasets according to the popular tags and the their data portals. (b) Users can select few privacy relevant attributes like age, gender, race etc. in order to form relevant clusters, as seen in (c) . (d) and (e) represent a word cloud and a bar chart respectively which denote the top attributes in each cluster. (f) shows some of the data portals available in this interface. (g) shows the distribution of the selected privacy-related attributes in the dataset combinations while (h) shows a distribution of their risk scores. (i) shows and the joining attributes between each dataset pair and (j) shows their corresponding risk score, normalized to a scale of 1 to 5.   }
\end{center}
\vspace{-6mm}
\end{figure*}
\subsection{Selection of datasets} \label{section:selection_of_datasets} \aritra{This subsection is unimportant, reads like a user manual and can be reduced by 75 \%}

Datasets selection is an integral part of this process since the efficacy of the task \textbf{T2} depends directly upon the type of datasets selected. This has been ameliorated by the Socrata API, a powerful tool to access datasets from open data portals\cite{SocrataAPI}. It allows the user to query the open data portals and access their data resources along with their metadata. Thus, a list of domains (data portals) available through this API was collected and only those were selected which have at least 2 data resources available. The following query was used for this activity:
\begin{verbatim}
http://api.us.socrata.com/api/catalog/v1/domains
\end{verbatim}
These portals, hosted by governments, non-profits and NGOs, contained a variety of data resources like datasets, maps etc., along with the content generated by consumers around the world who save their content like charts, maps, filtered views into these open data portals. Hence, it was decided to retain only those resources which were marked as "provenance=official" (resources uploaded by the administrators of the respective portals) and was further filtered to keep only the datasets. This process led to the collection of metadata like column names, permalink, number of rows available and tags for around $8400$ datasets, which was further filtered down to a set of $426$ datasets which contained quasi-identifiers like age, gender, race and location.

During early discussion with domain experts, it was evident that users may want to select a subset of datasets instead of all the dataset available to them, in order focus more on possible disclosure risk local to a certain type of dataset. PRIVEE has multiple filter options, baked right right at the top bar of the screen.The filter options include 

\begin{enumerate}
\item \textit{Type of dataset:} During dataset analysis, it was observed that datasets can have two type of records:
\begin{itemize}
\item \textit{individual records:} where each record corresponds to a single individual, like arrests dataset, medical records etc.
\item \textit{aggregated records:} where each record corresponds to the aggregated values for a certain category, like disease infection in a county, education levels in a district etc.
\end{itemize}
Users can filter the datasets according to their type of records (see Figure \ref{figs:interface}a). PRIVEE has a collection of around $151$ individual-record level datasets and around $275$ aggregated-record level datasets.
\item \textit{Popular tags:} The data portals label each datasets with few tags which generally portray the popular keywords related to each dataset. During the selection of datasets, the tags were analyzed for their frequency in this collected datasets. This sorted list of tags are available in the filter area (see Figure \ref{figs:interface}a) where the users can filter the datasets based on their tags/keywords of choice.
\item \textit{Data portals:} As mentioned earlier, data experts may be interested in analyzing the datasets from a certain data portal only. This can be achieved by selecting the relevant data portals from the list of the portals available in the filter area (see Figure \ref{figs:interface}f). A complete list of the portals can be found in the appendix.
\item \textit{Type of plot:} PRIVEE has two different types of plots available in order to cater to different attack scenarios. In order to implement the attack scenario through joinable datasets (Section \ref{section:attack_scenario1}), PRIVEE has projection plots along with the clusters, word cloud and the bar chart of the popular attributes. But in order to implement the attack scenario through unique records (Section \ref{section:attack_scenario2}), a different view of histograms can be loaded using the options available through the filter area (see Figure \ref{figs:interface}a)
\end{enumerate}



\subsection{Privacy-related attributes : T1} \label{section:privacy_related_attributes}

It is generally  understood that some attributes may be more relevant than others in the context of privacy \aritra{Don't write sentences that are obvious}. There has been multiple examples where quasi-identifiers like age, gender, race, location etc. were used to find disclosure in datasets. Thus, it was prudent to develop a dictionary of such privacy-related attributes which can aid in finding joinable datasets. The datasets containing these attributes may be more vulnerable for disclosure. Hence, the individual level datasets were analyzed and a list of attributes  were identified which are related to the quasi-identifiers age, gender and race.  Some of the privacy-related attributes are as follows: ["age\_group", "vic\_age\_group", "susp\_age\_group", "perp\_age\_group", "vict\_age","age\_1", "age\_at\_release", "admission\_age", "age\_class", "subject\_age", "patient\_age", "age\_range", "offender\_age", "officer\_age", "age\_at\_arrest","sex", "susp\_sex", "vic\_sex", "perp\_sex","sex\_1",  "victim\_gender", "suspect\_gender", "complainant\_sex", "officers\_sex",  "susp\_race", "vic\_race", "perp\_race", "vict\_descent",  "victim\_race", "suspect\_race", "complainant\_race", "officers\_race","subject\_race", "officer\_race"]. Users can choose any combination of these attributes through \textit{PRIVEE} (see Figure \ref{figs:interface}b) (task \textbf{T1}).



\subsection{Datasets Projection \& Clusters: T2} \label{section:datasets_projection}

% Discovering joinable datasets (task \textbf{T2}) is one the initial tasks achieved through PRIVEE. 

In order to find joinability, the datasets are projected in a $2$-dimensional scatterplot where each dot represents a dataset (refer Figure \ref{figs:interface}c). Datasets which are near to each other in this projection view are considered to be in a cluster, hence more joinable.  A wordcloud shows the most popular attributes in each cluster, followed by a bar chart showing their frequency, which aid the users in modifying the privacy-related attributes (refer Figure \ref{figs:interface}d and Figure \ref{figs:interface}e respectively). But in order to convert the datasets into dots on the 2-D projection and identify clusters with similar features, multiple algorithms were used and tested for efficiency. In this section, we discuss and compare these algorithms in details.

\subsubsection{Dataset Conversion Algorithm 1: Convert links to vectors }

\aritra{Why are you calling them dataset conversion algorithms?}

The overall assumption for finding joinability is that datasets with similar attributes can be joined together to find disclosure. Hence, the obvious way to find joinability was to find the number of possible joining attributes between two datasets.  An algorithm was developed to calculate the number of common attributes between the individual datasets and each of the other $5400$ datasets collected through the open data portals.  For example, if the individual level dataset Dataset A has the attributes ["age", "gender", "race"] and another dataset Dataset X has the attributes ["age", "gender"], so there are two common attributes between them. Similarly,  the common attributes were calculated between Dataset A and all the other datasets and it was stored as a vector of numbers, where each number represented the number of common attributes between the individual dataset and the other dataset. This vector can also be called a vector of links (common attributes), hence this method was named  \textit{Link2Vec}, a name similar to the word2vec approach used by different word embedding methods. This Link2Vec vector was calculated for all the individual datasets. But in order to visually analyze the datasets, it is prudent to plot their corresponding vectors on a 2D scatterplot. Since these vectors were of high dimension (1 X 5400), these were reduced to lower 2-dimension vectors using dimensionality reduction techniques like t-distributed Stochastic neighbor embedding (t-SNE)\cite{van2008visualizing}.  Clustering technique like DBSCAN was used to identify clusters and visually identify them using the color channel in the 2D scatterplot. In this approach, datasets which were plotted nearby in the scatterplot should be more joinable\cite{ester1996density,schubert2017dbscan}.

Since finding joinability is the first step towards finding disclosure, it is intended that the datasets which actually have more disclosure risks should be highlighted more in the 2D scatterplot. Hence a separate vector was included for the privacy-related attributes along with the Link2Vec vectors in order to emphasize  more on the datasets which may be more vulnerable for disclosure. But it was observed that using the privacy-related attributes did not change the results significantly, even after using different weights for these attributes (\textit{The process of adjusting the weights for these attributes have been explained in the further sub section \ref{section:choosing_appropriate_weights}}). Thus, it was decided that another approach to find joinability between datasets and adjust them according to the privacy related attributes should be pursued.

\subsubsection{Dataset Conversion Algorithm 2: Convert attributes to vectors}

Since Link2Vec was not performing well for the privacy-related attributes, it was decided that another method should to be developed which will respond to the extra weights added by these attributes. Since the metadata collection process (refer Section \ref{section:selection_of_datasets} already ensured the availability of all the column names for each of the datasets, these column names were converted them into numerical word embeddings using the spaCy library\cite{Spacy}. This library analyzes each of the column names and converts them into its vector representation. Then a sum of all the vectors is calculated to generate a single vector of dimension 1 X 300.  Since, again we have a high dimension vector similar to that of the Link2Vec method,  t-SNE  was used to reduce it into a lower dimension\cite{van2008visualizing}. It is to be noted here that since these vectors are merely a numerical representations of the column names, hence cosine similarity was used as the distance metric instead of the Manhattan distance in the t-SNE algorithm. DBSCAN algorithm was used to find the clusters and it was observed that  this technique performs better than the Link2Vec technique\cite{ester1996density,schubert2017dbscan}. Calinski-Harabasz Index is used to measure the performance of clustering algorithms and it is defined as the ratio of the between-cluster dispersion and the inter-cluster dispersion,  where dispersion means the sum squared distance between the samples and the barycenter\cite{calinski1974dendrite}. Higher score signifies that the clusters are far away, that implies better clusters. The Link2Vec method had a Calinski-Harabasz Index of $19.43881940249555$ while the AttributeText technique had a score of $30.420922241056488$, signifying that it was performing better than Link2Vec. Hence, this technique was chosen for further observations and was implemented in the interface \textit{PRIVEE}. A further comparison of these two techniques can be observed from Figure \ref{figs:link2vec_vs_attributetext} where Figure \ref{figs:link2vec_vs_attributetext}a, Figure \ref{figs:link2vec_vs_attributetext}b and Figure \ref{figs:link2vec_vs_attributetext}c represent the distribution of the clusters using AttributeText method while Figure \ref{figs:link2vec_vs_attributetext}d, Figure \ref{figs:link2vec_vs_attributetext}e and Figure \ref{figs:link2vec_vs_attributetext}f represent the cluster distribution for the Link2Vec method. Colors have been used to represent different clusters and it is visually evident from the figure that AttributeText method has better defined clusters. 
\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{figures/methods1_cluster_comparison.pdf}
\vspace{-4mm}
 \caption{\label{figs:link2vec_vs_attributetext}\textbf{Comparison between AttributeText and Link2Vec techniques} This figure compares the clusters of AttributeText when (a) weight=1 (b) weight=8 and (c)weight=17 with the clusters of Link2Vec when when (d) weight=1 (e) weight=8 and (f)weight=17. It can be observed that there is no significant change to the Link2Vec clusters while using different weights. Refer Section \ref{section:datasets_projection}  }
\end{center}
\vspace{-6mm}
\end{figure*}

\subsubsection{Choosing appropriate weights} \label{section:choosing_appropriate_weights}
It is assumed that adding more weights to the privacy-related attributes will help them being plotted more closely in  the 2D projection plot. This will help the user to select those dataset combinations and analyze them further for disclosure risks. Hence, an experiment was designed to adjust the weights and analyze the resulting clusters. The experiment started with a weight of 1 and a vector was created  which will highlight if a certain privacy-related attribute is present in the dataset or not. For example, if a user selects the set of privacy-related attributes [age, gender, race] and if Dataset A has only the age attribute while Dataset B has the age and race attributes, then the corresponding vectors would be $[1, 0,0]$ and $[1,0,1]$ respectively. Next, the vectors generated through the AttributeText method were appended to these vectors. These combined vectors were then reduced to a  2-dimensional vector using t-SNE dimensionality reduction algorithm and DBSCAN algorithm was used to find the clusters\cite{van2008visualizing,ester1996density,schubert2017dbscan}. Though this method showed some initial clusters, these clusters were not geared towards clustering the ones with the privacy related attributes in the same cluster.

It was realized that a mere weight of $1$ would not affect the clusters performance to a great extent.  Hence, the weights were increased in steps of $1$ in the range of $1$ to $100$ and their performance were analyzed. Other than the Calinksi-Harabasz Index (CH) described before, clustering metrics like Silhouette Score (SS) \cite{rousseeuw1987silhouettes} and Davies-Bouldin Index(DB)\cite{davies1979cluster} were also used to analyze the clusters. It was observed that almost distinct clusters start to form at $weight = 4$. At $weight=8$, the clusters were  more prominent and their scores were $SS=0.4570675$, $CH= 641.3454566125303$, $DB= 0.880139861638646$. At $weight =17$, the clusters were little bit more prominent and their scores were $SS=0.84298706$, $CH= 1055.1405222195654$, $DB= 0.15986152904$ . At higher weights, the clusters remained more or less similar. This experiment was also performed on the full set of privacy-related attributes collected earlier and it was observed that though the scores and the clusters are not that good at $weight = 8$, $weight = 17$ has excellent scores. Though  this experiment was also conducted using other combinations of the privacy related attributes, the observations were quite similar. Hence, the  weights $8$ and $17$ were chosen as the candidate weights. Figure \ref{figs:link2vec_vs_attributetext}a and Figure \ref{figs:link2vec_vs_attributetext}d show the clusters at $weight=1$, Figure \ref{figs:link2vec_vs_attributetext}b and Figure \ref{figs:link2vec_vs_attributetext}e show the clusters at $weight=8$ while Figure \ref{figs:link2vec_vs_attributetext}c and Figure \ref{figs:link2vec_vs_attributetext}f show the clusters at $weight=17$. It is clearly evident from the figure that the AttributeText method performed well at higher weights while the Link2Vec method did not respond significantly to the change in weights. Since the clusters may change with the change  in privacy-related attributes, both the candidate weights (weight = $8$ and $17$) are used to generate the clusters but the cluster with better Calinksi-Harabasz Index is then displayed in PRIVEE. This ensures that always the best cluster formation is displayed and it becomes easier for the user to find joinable datasets (task T1). More details about this experiment can be found in the supplementary materials.

\subsubsection{Selecting the clustering algorithm} \label{section:selecting_clustering_algorithms}

Since DBSCAN algorithm was already being used to generate the clusters, it was prudent to check how the other clustering algorithms perform in this scenario. Hence these four clustering algorithms were chosen :
\begin{itemize}
\item DBSCAN \cite{ester1996density,schubert2017dbscan}
\item OPTICS \cite{ankerst1999optics}
\item KMeans \cite{vassilvitskii2006k}
\item Birch \cite{zhang1996birch}
\end{itemize}

Another experiment was designed to check the performance of these algorithms with different weights and also different combinations of the privacy-related attributes. For the attribute combination [age, gender, race] and $weight =1$ , DBSCAN and OPTICS performed more or less similarly but KMeans and Birch did not give meaningful clusters. Moreover, it is not recommended to use the previously  discussed metrics for KMeans and Birch algorithms since they generally produce higher results using those metrics, hence  the quality of the clusters was checked manually instead of using those metrics for these algorithms. At higher weights, DBSCAN performed better than OPTICS and this became evident from their scores. While DBSCAN had Calinksi-Harabasz Index as $641.345466125303$, OPTICS has a Calinksi-Harabasz Index of $22.671327997926248$. The results were similar in even higher weights. Different combinations of privacy-related attributes were used and it was observed that DBSCAN and OPTICS perform almost the same when $weight = 1$, but the former performs better with higher weights like $8$ and $17$. Hence, the DBSCAN algorithm was chosen for the whole process and was implemented in the interface \textit{PRIVEE}. Further details about this experiment can be found in the supplementary materials.

\subsubsection{Risk Score calculation} \label{section:risk_score_calculation}
Joining attributes are the number of common attributes between two datasets. Since joinability of two datasets depend upon the number of the joining attributes, the risk score is calculated as a function of the number of joining attributes along with the number of privacy-related attributes between the two datasets in a pair of datasets. The formulae for the risk score can be defined as follows:
\begin{equation}
    \text{risk} = \alpha * P + (J-P)
    \label{equation:risk_score}
\end{equation}
where:
\begin{description}
\item [$\alpha$] = $50$, the empirical risk ratio,
\item [P] = number of privacy-related attributes,
\item [J] = number of joining attributes
\end{description}
For example, if two datasets have a $15$ joining attributes and only $2$ of them are privacy-related attributes, the risk score can be calculated as $113$, as per equation \ref{equation:risk_score}.

In order to determine the empirical risk ratio, an experiment was designed to calculate the risk scores of all the possible combination of datasets from the datasets collected during the selection of datasets process (section \ref{section:selection_of_datasets}). Since there are a total of 426 datasets, this experiment calculated the risk score of $\Comb{426}{2}$ i.e., $90,525$ pairwise combinations of datasets. This experiment was repeated multiple times, each time with a different value of the risk ratio, ranging from $1$ to $100$. It was observed that the value $50$ works well in order to separate the dataset pairs with privacy related attributes and the ones without them, hence risk ratio was fixed at the value $50$. 

Entropy also plays an important factor in determining the joinability of the datasets. Another experiment was developed to calculate the entropy of each of the attributes in all the datasets collected during the selection of datasets process (section \ref{section:selection_of_datasets}). Though the dataset combinations are primarily sorted according to the risk score, but if a user selects certain attributes for checking the possible matches between them, the mean entropy of these attributes are used as a secondary sorting key for the pairwise dataset combinations. 
All the Python Jupyter notebooks for these experiments can be found in the supplementary materials.


\section{PRIVEE: Visualization and Interaction Design}

\aritra{Describe the visualizations and interactions here. WHy don't you name the views, for example, risk explanation view, data joinability view and use them as section names?}

% \subsubsection{Designing the Visual Aids} \label{section:designing_visual_aids}


PRIVEE has a default selection of privacy-related attributes as [age, gender, race]. But a user may require to change these default selections in order to analyze disclosures in a specific set of datasets. Moreover, the cluster formation is highly dependent of the selected privacy-related attributes. Thus, in order to find more joinable datasets (task \textbf{T2}), a wordcloud of the most frequent attributes in each cluster is displayed below the 2D scatterplot of datasets(see Figure \ref{figs:interface}d). The most frequent attributes are shown in a larger font, thus helping the user choose the privacy-related attributes.

But a user may also be interested in understanding the frequency difference of the selected privacy-related attributes and the other highly frequent attributes. This can be fulfilled using the attribute bar chart which shows a sorted view of the frequency distribution of the top attributes(see Figure \ref{figs:interface}e). The selected privacy-related attributes are shown at the top, followed by the top-$5$ most frequent attributes in that particular cluster. After selecting the desired set of privacy-related attributes, user can select any set of dots from the 2D scatterplot and their corresponding combination of datasets will be shown on the right-hand side, as described in the next section.


\aritra{All of these subsections will change as the discussions should anchor on the visualizations and interactions}

\subsection{Assessment of Risky Datasets \& Finding joinable attributes : T4, T5)} \label{section:comparison_of_risks}
After the selection of a cluster of datasets from the 2D scatterplot, it is prudent to find out which pair of datasets have a higher risk of disclosure. For example, if a user selects a cluster with $7$ different datasets, there can be $\Comb{7}{2}$ i.e., $21$ pair-wise combinations of datasets and if the user selects a cluster with $15$ datasets, there can be a total of $\Comb{15}{2}$ i.e., $105$ pair-wise combinations of datasets. It is a cumbersome task to manually evaluate all these combinations of datasets for disclosure, hence PRIVEE has introduced a risk score which scores each dataset combination on certain parameters and the sorts them accordingly. 



\subsubsection{Design of the Visual Aids} \label{section:designing_visual_aids_risk_score}
Each pair of dataset is represented using a combination of multiple elements, including a radio button, the dataset names, and a stacked bar chart, where each bar represents the joining attributes present between these datasets(refer Figure \ref{figs:interface}i). The bars marked in light red are the privacy-related attributes selected by the user. As mentioned earlier, each of these combinations are sorted primarily according to the risk score and secondarily according to the mean entropy of the selected attributes, if any.

Using the equation \ref{equation:risk_score}, it was observed that the risk score for most of the $90,525$ pairwise dataset combinations range between $0$ to $182$. Hence, this was normalized into a scale of $0$ to $5$ and has represented by the stacked horizontal red bars, as shown in Figure \ref{figs:interface}j. Though few of these dataset combinations had a extremely high risk score, they were mapped to the highest bar in this representation.

If there are multiple pairwise dataset combinations, a user may be interested in those combinations which lie within a certain risk score range. This can be implemented using the \textit{risk score filter}, which shows a histogram distribution of the risk scores of all the dataset combinations (see Figure \ref{figs:interface}h). Moreover, the \textit{frequency bar chart} on the left-hand side of the risk score filter also helps to understand the distribution of the privacy-related attributes in these pairwise combinations of datasets (refer Figure \ref{figs:interface}g).

After comparing this risks of different pairwise combination of datasets (task \textbf{T4}), users can select any such pair using the radio button along with of the attributes of interest (task \textbf{T5}) which can be used to join the datasets. Further details about the joining of the datasets have been discussed in the next section


\subsection{Evaluation of the Risk : T6} \label{section:evaluation_of_risks}
After the selection of the datasets pair from the dataset pair and attributes of interest from the risk comparison area, a user needs to evaluate the possible risks while joining these datasets. For example, joining two datasets on few attributes may reveal that there are no common records between them, which implies these datasets can be safely joined in order to use the combined dataset for further research. Again, for example, if there are $4$ common records while joining two datasets, it implies that these datasets cannot be joined in order to prevent identity disclosure. 

A visualization framework has been developed in order to evaluate the disclosure risks of joining datasets (task \textbf{T6}). After joining a pair of datasets, if there are few common records, these records are inspected for the presence of different categories of the attributes of interest and each such category is plotted as a bar in a stacked bar chart. For example, if the common records contain two genders, namely Male and Female, the stacked bar chart will contain two bars, one of each category (see Figure \ref{figs:scenario1}d). But if there are multiple values of a numerical attribute of interest (like age), a histogram is developed with equally distributed bins. Each category of the attributes of interest is then connected using a line where the thickness of the line depicts the number of records containing these categories of these attributes (see Figure \ref{figs:scenario1}d). For example, if there are $3$ records of gender = Male and race = White while $10$ records of gender = Male and race = Black, then the line originating from gender = Male towards the race = Black will be thicker than that originating from gender = Male towards the race = White. Clicking on each of these lines will display the actual records.


\subsection{Finding datasets with lower number of records: T3}
In order to implement the attack scenario described in Section \ref{section:attack_scenario2}, a separate view was implemented in PRIVEE. Lower counts of a certain category of attributes can be detected by developing a bar chart/histogram for each of  the corresponding attributes of each dataset. Thus, a view was created where a bar chart would be developed for the selected privacy-related attributes if they were categorical in nature while a histogram would be developed if they are numerical in nature (see Figure \ref{figs:scenario3}c). The bars for the categorical attributes would show the frequency of each of the different categories of this attribute. The numerical attributes would be divided into bins of equal intervals and the corresponding bars would display the frequency of each of the bins. The bins with lower number of records would be displayed in red (\textbf{T3}).

These bar charts/histograms would be displayed for all the datasets selected through the different filters (see Section \ref{section:selection_of_datasets}) iff they have all the privacy-related attributes selected by the user. In case multiple datasets are selected, analyzing all these datasets may be a cumbersome task, hence PRIVEE sorts these datasets based on the lowest frequency of a bin and the number of such dangerous/low count bins (bins with frequency $\leq 4$). For example, if a Dataset A has only $2$ records for race="Hawaiian" while Dataset B has $1$ record for age=19-20 and 1 record for the race="Black", Dataset B will be displayed first, followed by Dataset A. Any such dataset can be selected from this view to compare the risk of disclosure with respect to each of the individual-record level datasets available in PRIVEE (see Figure \ref{figs:scenario3}e).

The bins for each of the privacy-related attributes (see Section \ref{section:datasets_projection}) were pre-calculated using an algorithm developed specifically for this purpose. This cannot be done as an on-demand basis since it would include an overhead of downloading the datasets and processing them through this algorithm, which would render the interface useless due to the unusually high processing time.



==> sections/old/privee_analytical.tex <==
% \section{Design Rationale of PRIVEE}
% \aritra{Describe the clustering algorithms and risk score here in two subsections}
% \kaustav{Used this section to describe the clustering process and the risk score. Also reduced the content from the previous version, but kept some of the scores from the metrics in order to emphasize why we chose these methods}
\begin{comment}

\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{figures/cluster_comparison_v2.pdf}
\vspace{-4mm}
 \caption{\label{figs:link2vec_vs_attributetext}\textbf{Comparison between AttributeText and Link2Vec techniques} This figure compares the clusters of (a) AttributeText with that of (b) Link2Vec at weight=17. It can be observed that AttributeText has better clusters. Refer Section \ref{section:dataset_joinability} \aritra{You need to have a better figure showing what the projection plot actually shows so that we can interpret joinability groups from the plot. Get rid of the Link2Vec figure and add that one. You will hence end up with two projection plots, one is the AttributeText and the other showing an enlarged or zoomed in version explicitly showing what inference we can make.} }
\end{center}
\vspace{-6mm}
\end{figure}
\end{comment}
%In the previous sections, we have discussed the development and importance of a visual analytic workflow in order to emulate the attack scenarios to find disclosure risk. 
% In the previous sections, we have discussed the possible attack scenarios along with the high-level tasks associated with them. 



%which are important in establishing the visual analytic workflow.


% \begin{figure*}[t]
% \begin{center}
% \includegraphics[width=\textwidth]{figures/interface.pdf}
% \vspace{-4mm}
%  \caption{\label{figs:interface}\textbf{Different visual components of PRIVEE} (a) The filter area has options to select the type of dataset (individual/aggregated), type of plot (projection/histogram), filter the datasets according to the popular tags and the their data portals. (b) Users can select few privacy relevant attributes like age, gender, race etc. in order to form relevant clusters, as seen in (c) . (d) and (e) represent a word cloud and a bar chart respectively which denote the top attributes in each cluster. (f) shows some of the data portals available in this interface. (g) shows the distribution of the selected privacy-related attributes in the dataset combinations while (h) shows a distribution of their risk scores. (i) shows and the joining attributes between each dataset pair sorted according to their entropy and (j) shows their corresponding risk score }
% \end{center}
% \vspace{-6mm}
% \end{figure*}

\section{Diagnosis of Vulnerable Entry Points~(G1)} \label{section:vulnerable_entry_points}
% \aritra{Why are you calling them dataset conversion algorithms?}
% \kaustav{Changed the name for this section and merged the previous one into this.}

%\aritra{explain the design rationale for T1 anf T2- the interplay between analytical methods and visualization in 2 sentences at most}
\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{figures/vulnerable_entry_points_v2.pdf}
\vspace{-4mm}
 \caption{\label{figs:vulnerable_entry_points}\textbf{Diagnosis of vulnerable entry points.} (a), (b), (c):  filters help in the selection of datasets based on their metadata and the data portals, and (d) exposing the vulnerabilities in the data distributions, where bins with too few records are colored in red.}
\end{center}
\vspace{-8mm}
\end{figure}

The red-teaming exercise helped us exploit multiple entry points into the open data ecosystem and demonstrated the need for guiding defenders' risk analysis strategy with meaningful selections. As a defense strategy and a corresponding design requirement, PRIVEE achieves tasks T1~(metadata-based selection) and T2~(selections based on vulnerable data sets) by providing defenders the \textit{flexibility} to explore multiple reconnaissance strategies.

\par \noindent \textbf{Selections based on tags and privacy-relevance}: We observed that the open datasets are already enriched with metadata information like the popular tags relevant to them. Thus, we designed a tag selection filter where defenders can select the tags pertinent to them. But, a defender, unaware of the popular keywords, may not effectively filter the seed datasets. Hence, PRIVEE can guide the user through the dataset selection process using a sorted bar chart view which highlights the frequency of each of the tags (\textbf{T1})~(Figure \ref{figs:vulnerable_entry_points}c). We use the red color throughout the interface to indicate risk or vulnerability.
We used a metadata dictionary of privacy-related attributes which can aid in finding datasets of interest (\textbf{T1}). Individual-level datasets were analyzed and a list of attributes was identified which are related to the quasi-identifiers age, gender, and race.  Some of the privacy-related attributes are as follows: "age\_group", "vic\_age\_group", "susp\_age\_group", "perp\_age\_group", "vict\_age","age\_1", "age\_at\_release", "admission\_age", "age\_class", "subject\_age", "patient\_age", "age\_range", "offender\_age", "officer\_age", "age\_at\_arrest","sex", etc.. Users can choose any combination of these attributes through \textit{PRIVEE} as an initial selection that can be modified later.

\par \noindent \textbf{Selections based on data granularity}: The $426$ datasets seed datasets we collected belong to $102$ data portals. In PRIVEE,  we allow defenders to analyze the risk profiles of the datasets by the specification of any preferred data portal~(Figure \ref{figs:vulnerable_entry_points}b) (\textbf{T1}).
Risk profile may be different for datasets with \textit{individual records} where each record corresponds to a single individual, like arrests dataset, medical records; or with
\textit{aggregated records, } where each record corresponds to the aggregated values for a certain category, like disease infection in a county, education levels in a district etc. PRIVEE offers the option to select a subset of these pre-labeled datasets~(i.e., as individual level or aggregate level) based on the granularity of the records, thus augmenting the dataset selection process with user's input (\textbf{T1})~(Figure \ref{figs:vulnerable_entry_points}a).  

\par \noindent \textbf{Sorting vulnerable distributions}: PRIVEE helps the data defenders discover vulnerable datasets by showing the distribution of the privacy-related attributes. The vulnerable record categories are highlighted in bright red, thus guiding the user towards selecting datasets with such vulnerabilities (\textbf{T2})~(Figure \ref{figs:vulnerable_entry_points}d). PRIVEE also performs an automatic analysis of these distributions and sorts the datasets based on the degree of vulnerability present. For example, if a Dataset A has only $2$ records for race="Hawaiian" while Dataset B has $1$ record for age=19-20 and $1$ record for the race="Black", Dataset B will be displayed first, followed by Dataset A.

% \begin{comment}

% {Filter Area} \label{section:filter_area}
% During early discussion with domain experts, it was evident that users may want to select a subset of datasets instead of all the dataset available to them, in order focus more on possible disclosure risk local to a certain type of dataset. PRIVEE has multiple filter options, baked right right at the top bar of the screen. The filter options include 

% \aritra{I included the following text but hope it is clear that we need to emphasize the functionalities better and modify the writing so that it does not read like a user manual}

% \begin{enumerate}
% \item \textit{Type of dataset:} During dataset analysis, it was observed that datasets can have two type of records:
% \begin{itemize}
% \item \textit{individual records:} where each record corresponds to a single individual, like arrests dataset, medical records etc.
% \item \textit{aggregated records:} where each record corresponds to the aggregated values for a certain category, like disease infection in a county, education levels in a district etc.
% \end{itemize}
% Users can filter the datasets according to their type of records (see Figure \ref{figs:interface}a). PRIVEE has a collection of around $151$ individual-record level datasets and around $275$ aggregated-record level datasets.
% \item \textit{Popular tags:} The data portals label each datasets with few tags which generally portray the popular keywords related to each dataset. During the selection of datasets, the tags were analyzed for their frequency in this collected datasets. This sorted list of tags are available in the filter area (see Figure \ref{figs:interface}a) where the users can filter the datasets based on their tags/keywords of choice.
% \item \textit{Data portals:} As mentioned earlier, data experts may be interested in analyzing the datasets from a certain data portal only. This can be achieved by selecting the relevant data portals from the list of the portals available in the filter area (see Figure \ref{figs:interface}f). A complete list of the portals can be found in the appendix.
% \item \textit{Type of plot:} PRIVEE has two different types of plots available in order to cater to different attack scenarios. In order to implement the attack scenario through joinable datasets (Section \ref{section:attack_scenario1}), PRIVEE has projection plots along with the clusters, word cloud and the bar chart of the popular attributes. But in order to implement the attack scenario through unique records (Section \ref{section:attack_scenario2}), a different view of histograms can be loaded using the options available through the filter area (see Figure \ref{figs:interface}a)
% \end{enumerate}




% {Attribute Selection Area} \label{section:attribute_selection_area}
% There has been multiple examples where quasi-identifiers like age, gender, race, location etc. were used to find disclosure in datasets. Thus, it was prudent to develop a dictionary of such privacy-related attributes which can aid in finding datasets of interest (\textbf{T1}). These attributes are given more weightage while finding the clusters of joinable datasets (see Section \ref{section:weight_selection}). Hence, the individual level datasets were analyzed and a list of attributes  were identified which are related to the quasi-identifiers age, gender and race.  Some of the privacy-related attributes are as follows: ["age\_group", "vic\_age\_group", "susp\_age\_group", "perp\_age\_group", "vict\_age","age\_1", "age\_at\_release", "admission\_age", "age\_class", "subject\_age", "patient\_age", "age\_range", "offender\_age", "officer\_age", "age\_at\_arrest","sex", "susp\_sex", "vic\_sex", "perp\_sex","sex\_1",  "victim\_gender", "suspect\_gender", "complainant\_sex", "officers\_sex",  "susp\_race", "vic\_race", "perp\_race", "vict\_descent",  "victim\_race", "suspect\_race", "complainant\_race", "officers\_race","subject\_race", "officer\_race"]. Users can choose any combination of these attributes through \textit{PRIVEE} (see Figure \ref{figs:interface}b).


% \end{comment}


% \par {\textit{Link2Vec algorithm:}} PRIVEE has a collection of around $151$ individual-record level datasets and around $275$ aggregated-record level datasets, thus a total of $426$ datasets.
% The overall assumption for finding joinability is that datasets with similar attributes can be joined together to find disclosure. Hence, the obvious way to find joinability was to find the number of possible joining attributes between two datasets.  An algorithm was developed to calculate the number of common attributes between the individual datasets and each of the other $5400$ datasets collected through the open data portals.  For example, if the individual level dataset Dataset A has the attributes ["age", "gender", "race"] and another dataset Dataset X has the attributes ["age", "gender"], so there are two common attributes between them. Similarly,  the common attributes were calculated between Dataset A and all the other datasets and it was stored as a vector of numbers, where each number represented the number of common attributes between the individual dataset and the other dataset. This vector can also be called a vector of links (common attributes), hence this method was named  \textit{Link2Vec}, a name similar to the word2vec approach used by different word embedding methods. This Link2Vec vector was calculated for all the individual datasets. But in order to visually analyze the datasets, it is prudent to plot their corresponding vectors on a 2D scatterplot. Since these vectors were of high dimension (1 X 5400), these were reduced to lower 2-dimension vectors using dimensionality reduction techniques like t-distributed Stochastic neighbor embedding (t-SNE)\cite{van2008visualizing}.  Clustering technique like DBSCAN was used to identify clusters and visually identify them using the color channel in the 2D scatterplot. In this approach, datasets which were plotted nearby in the scatterplot should be more joinable\cite{ester1996density,schubert2017dbscan}.

% \par {\textit{Privacy-related attributes:}} Since finding joinability can be considered as the first step towards finding disclosure(\textbf{T1a}), it is intended that the datasets which actually have more disclosure risks should be highlighted more in the 2D scatterplot. Hence a separate vector was included for the privacy-related attributes along with the Link2Vec vectors in order to emphasize  more on the datasets which may be more vulnerable for disclosure. But it was observed that using the privacy-related attributes did not change the results significantly, even after using different weights for these attributes. Thus, it was decided that another approach to find joinability between datasets and adjust them according to the privacy related attributes should be pursued.

\section{Triage Joinable Groups~(G2)} \label{section:joinable_groups}

%\aritra{commented out Link2Vec description- you need just describe in 2-3 short sentences the alternative to what worked and why ours is a better alternative}
%The first goal towards the evaluation of risks in open datasets is to bootstrap the process. PRIVEE helps in this by guiding the users to select a subset of datasets which are more joinable together. But this subset may be large enough, thus making it practically difficult to analyze all possible combinations of these datasets for disclosure risk. Hence, it is important to find even smaller sub-groups of datasets which are highly joinable. In this section, we discuss the approaches used in finding the joinable groups and their subsequent exploration.

The design requirements for addressing task T3 in the PRIVEE workflow are as follows: human-in-the-loop clustering \textit{responsive} to multiple definitions of privacy relevance, and \textit{transparency} in analyzing cluster signatures so that defenders can develop a mental model of the context and the degree of the potential vulnerability of subsequent joins.



\subsection{Finding Similar Datasets}

\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{figures/joinable_groups_v6.pdf}
 \caption{\label{figs:joinable_groups}\textbf{Analysis of Joinable Groups.} (a) a group of joinable datasets sharing the privacy-relevant attributes like \textit{age, gender, race}, (b) another group but without any of the previously defined privacy-relevant attributes. In this group, a defender observes the presence of attributes like \textit{victimgender} and \textit{victimrace} and updates the initial list of privacy-relevant attributes. (c) dynamic re-grouping based on user's input, where datasets with the new list of privacy-relevant attributes are grouped together.  }
\end{center}
\vspace{-6mm}
\end{figure}

% The most intuitive approach to finding the similarity among datasets is to analyze the similarity in their attribute space.

The intuition here is that datasets with similar attributes should be more joinable since the joinability of the two datasets is a function of their shared attributes. But the names of attributes of these open datasets are often noisy and inconsistent, making it computationally difficult to perform a binary search for the presence or absence of certain attributes. At the same time, the attribute names capture the semantic similarity between multiple datasets that might capture a similar context. We use a word-embedding approach that simultaneously satisfies the need to capture the joinability and semantic similarity of datasets.

\par \noindent \textbf{Applying Word2Vec with Data Attributes:} Word2Vec is available from the Python spaCy library. It converts each data attribute into a numeric vector form\cite{Spacy}. These vectors are then used to form a high-dimensional vector representation of the attribute space of a dataset which can be used to analyze their similarity. For example, the attributes "age" and "race" were represented by two different vectors of size 1 X 300, which were again used to form a vector representation for the attribute combination "age race". Hence, we used the t-SNE dimensionality reduction algorithm, which converts these high dimensional vectors into lower-dimensional embedding, using the cosine similarity between vectors~\cite{van2008visualizing}.  

\textit{Weight selection for privacy-related attributes:\label{subsection:weight_selection}} We use the default privacy-related attributes collected during the red-teaming activity in the process of finding joinable groups of datasets. We first created a weight vector representing the presence of these attributes, along with the vectors obtained from Word2Vec. For example, if Dataset A has only the age attribute while Dataset B has the age and race attributes, then the corresponding vectors for the presence of the privacy-related attributes [age, gender, race] would be $[x, 0,0]$ and $[x,0,x]$ respectively, where $x$ represents the weight assigned to the privacy-related attributes. Once we obtained this weight vector, we concatenated this with the vector obtained from training a Word2Vec model on our datasets. 

\par \noindent \textbf{Clustering in the projected space:} A 2-D projection of the datasets might not readily reveal dataset groupings. Hence, we used the DBSCAN clustering algorithm to computationally analyze these vectors and find groups of datasets between them\cite{ester1996density,schubert2017dbscan}.  This helped to effectively find groups of datasets joined together on their shared attributes. We also evaluated the different clustering algorithms and how they perform in this scenario. Using different values of the weights and the privacy-related attributes age, gender, and race, the DBSCAN and OPTICS clustering algorithms performed more or less similar. Still, the algorithms KMeans and Birch did not give any meaningful clusters \cite{ankerst1999optics,vassilvitskii2006k,zhang1996birch}.  But we chose DBSCAN algorithm in this interface since it has better scores than OPTICS at different combinations of the privacy-related attributes.

\par \noindent \textbf{Clustering evaluation:} We designed an experiment to ascertain the optimum value for $x$ by evaluating the cluster results using metrics like the \textit{Calinski-Harabasz Index}. The latter  is defined as the ratio of the between-cluster dispersion and the inter-cluster dispersion,  where dispersion means the sum squared distance between the samples and the barycenter\cite{calinski1974dendrite}. Higher score signifies that the clusters are far away, which implies better clusters. After comparing the results at different weights, $x=8$ and $x=17$ were chosen as the candidate weights for the vector for the privacy-related attributes. Since the clusters may change dynamically with the change in privacy-related attributes, the candidate weights (weight = $8$ and $17$) are used to generate the clusters. We also perform automated calibration of cluster quality using the Calinksi-Harabasz Index metric that ensures we can efficiently guide defenders in finding meaningful, joinable datasets.  We have included more details about these experiments in the supplementary materials.


\subsection{Dataset Joinability View}

We show the cluster signatures that help defenders focus on joinable subsets in this view. The main component is a multidimensional projection plot, where, as illustrated in Figure \ref{figs:joinable_groups}a, each red dot represents a dataset in the group of $45$ joinable datasets from the candidate set chosen by a data defender. The dots, not in this group, are represented by grey color. To drill down into the features responsible for the clusters, we use a dual-encoding approach, with a word cloud showing the most frequent attributes for each joinable group and a bar chart showing the frequency of privacy-relevant attributes first, followed by others. This encoding is to help familiarize a defender with any cluster with respect to both its general context and its privacy relevance. We use a small-multiple approach for this combination of projection, word-cloud, and bar chart. A defender can progressively inspect each cluster, starting from the top~(most vulnerable) to the bottom~(least vulnerable).

The word cloud in Figure \ref{figs:joinable_groups}b shows the presence the attributes \textit{victimgender} and \textit{victimrace}. Suppose defenders have a background knowledge that these attributes are generally present in police datasets. In that case, they can augment the initial list of privacy with these attributes along with other similar attributes like \textit{victimage} and  \textit{offenderage}. This interaction will lead to a dynamic grouping based on the user's understanding of the privacy-related attributes, which helps form a further fine-tuned group of highly joinable datasets. The fine-tuning is evident from \ref{figs:joinable_groups}c, which shows the new group with a smaller subset of $6$ datasets. The bar chart in Figure \ref{figs:joinable_groups}d shows that almost all the datasets in this group contain all the privacy-related attributes, thus helping the defender prioritize further inspection of this joinable group~(\textbf{T3}). 

% In this context, we would like to mention another procedure which was also being tested simultaneously for its efficacy. In this method, instead of converting the attributes into their Word2Vec representation, we developed vectors representing the presence of common attributes of each of the seed dataset with other datasets collected from the open data portal. This also led to the creation of a high dimensional vector and a similar procedure was used to project them on a 2-D projection plot . But using higher weights for the privacy-related attributes did not improve the results from this procedure. Hence, the Word2Vec approach is a better choice in finding groups of joinable datasets than this alternative approach.


%\aritra{You are not telling a news story, you are trying to scientifically argue and this is not one such argument--\textit{Since Link2Vec was not performing well for the privacy-related attributes, it was decided that another method should to be developed which will respond to the extra weights added by these attributes.}}Since the metadata collection process already ensured the availability of all the column names for each of the datasets, these column names were converted them into numerical word embeddings using the spaCy library\cite{Spacy}. This library analyzes each of the column names and converts them into its vector representation. Then a sum of all the vectors is calculated to generate a single vector of dimension 1 X 300.  Since, again we have a high dimension vector similar to that of the Link2Vec method,  t-SNE  was used to reduce it into a lower dimension\cite{van2008visualizing}. It is to be noted here that since these vectors are merely a numerical representations of the column names, hence cosine similarity was used as the distance metric instead of the Manhattan distance in the t-SNE algorithm. DBSCAN algorithm was used to find the clusters and it was observed that  this technique performs better than the Link2Vec technique\cite{ester1996density,schubert2017dbscan}. \textit{Calinski-Harabasz Index} is used to measure the performance of clustering algorithms and it is defined as the ratio of the between-cluster dispersion and the inter-cluster dispersion,  where dispersion means the sum squared distance between the samples and the barycenter\cite{calinski1974dendrite}. Higher score signifies that the clusters are far away, that implies better clusters. The Link2Vec method had a Calinski-Harabasz Index of $19.43881940249555$ while the AttributeText technique had a score of $30.420922241056488$, signifying that it was performing better than Link2Vec. Hence, this technique was chosen for further observations and was implemented in the interface \textit{PRIVEE}. A further comparison of these two techniques can be observed from Figure \ref{figs:link2vec_vs_attributetext} where the color channel has been used to represent different clusters and it is visually evident from the figure that AttributeText method has better defined clusters. 




%\par {\textit{Weights selection:}}\label{section:weight_selection} \aritra{shorten this by half} It is assumed that adding more weights to the privacy-related attributes will help them being plotted more closely in  the 2D projection plot. This will help the user to select those dataset combinations and analyze them further for disclosure risks. Hence, an experiment was designed to adjust the weights and analyze the resulting clusters. The experiment started with a weight of 1 and a vector was created  which will highlight if a certain privacy-related attribute is present in the dataset or not. For example, if a user selects the set of privacy-related attributes [age, gender, race] and if Dataset A has only the age attribute while Dataset B has the age and race attributes, then the corresponding vectors would be $[1, 0,0]$ and $[1,0,1]$ respectively. Next, the vectors generated through the AttributeText method were appended to these vectors. These combined vectors were then reduced to a  2-dimensional vector using t-SNE dimensionality reduction algorithm and DBSCAN algorithm was used to find the clusters\cite{van2008visualizing,ester1996density,schubert2017dbscan}. Though this method showed some initial clusters, these clusters were not geared towards clustering the ones with the privacy related attributes in the same cluster.

%A weight of $1$ would not affect the clusters performance to a great extent.  Hence, the weights were increased in steps of $1$ in the range of $1$ to $100$ and their performance were analyzed. Other than the Calinksi-Harabasz Index (CH) described before, clustering metrics like Silhouette Score (SS) \cite{rousseeuw1987silhouettes} and Davies-Bouldin Index(DB)\cite{davies1979cluster} were also used to analyze the clusters. It was observed that almost distinct clusters start to form at $weight = 4$. At $weight=8$, the clusters were  more prominent and their scores were $SS=0.4570675$, $CH= 641.3454566125303$, $DB= 0.880139861638646$. At $weight =17$, the clusters were little bit more prominent and their scores were $SS=0.84298706$, $CH= 1055.1405222195654$, $DB= 0.15986152904$ . At higher weights, the clusters remained more or less similar. This experiment was also performed on the full set of privacy-related attributes collected earlier and it was observed that though the scores and the clusters are not that good at $weight = 8$, $weight = 17$ has excellent scores. Though  this experiment was also conducted using other combinations of the privacy related attributes, the observations were quite similar. Hence, the  weights $8$ and $17$ were chosen as the candidate weights. The AttributeText method performed well at higher weights while the Link2Vec method did not respond significantly to the change in weights. Since the clusters may change with the change  in privacy-related attributes, both the candidate weights (weight = $8$ and $17$) are used to generate the clusters but the cluster with better Calinksi-Harabasz Index is then displayed in PRIVEE. This ensures that always the best cluster formation is displayed and it becomes easier for the user to find joinable datasets (\textbf{T1a}). More details about this experiment can be found in the supplementary materials.

%\par {\textit{Evaluation of Clusters:}} Since DBSCAN algorithm was already being used to generate the clusters, it was prudent to check how the other clustering algorithms perform in this scenario. Hence these four clustering algorithms were chosen :
%DBSCAN \cite{ester1996density,schubert2017dbscan}
 %OPTICS \cite{ankerst1999optics}
%KMeans \cite{vassilvitskii2006k}
 %Birch \cite{zhang1996birch}
%We designed an experiemnt to check the performance of these algorithms with different weights and also different combinations of the privacy-related attributes. For the attribute combination [age, gender, race] and $weight =1$ , DBSCAN and OPTICS performed more or less similarly but KMeans and Birch did not give meaningful clusters. Moreover, it is not recommended to use the previously  discussed metrics for KMeans and Birch algorithms since they generally produce higher results using those metrics, hence  the quality of the clusters was checked manually instead of using those metrics for these algorithms. At higher weights, DBSCAN performed better than OPTICS and this became evident from their scores. While DBSCAN had Calinksi-Harabasz Index as $641.345466125303$, OPTICS has a Calinksi-Harabasz Index of $22.671327997926248$. The results were similar in even higher weights. Different combinations of privacy-related attributes were used and it was observed that DBSCAN and OPTICS perform almost the same when $weight = 1$, but the former performs better with higher weights like $8$ and $17$. Hence, the DBSCAN algorithm was chosen for the whole process and was implemented in the interface \textit{PRIVEE}. Further details about this experiment can be found in the supplementary materials.







%After finding groups of dataset and analyzing through them, scatterplot becomes the most intuitive choice to visualize these groups of dataset. We used 2D scatterplots to plot all the datasets, with a plot for each of the groups. The plots were then sorted according to their Calinski-Harabasz Index with the most joinable group of dataset being at the top. This will guide the user towards selecting those groups of datasets which are highly joinable. In each plot, datasets belonging to each cluster are highlighted in bright red.


%Finding joinable datasets is one of the critical tasks required to emulate the attack scenarios. After filtering the datasets based on their type of records, tags and the data portals, multiple methods have been used to find the optimum process to find datasets which are similar in their attribute space(see Section \ref{section:dataset_joinability} and the most intuitive method to show a cluster of datasets is using a 2-D scatterplot(see Figure \ref{figs:interface}c). In this scatterplot, the datasets are projected as dots while the best cluster of dots are highlighted in red color. PRIVEE has a default selection of privacy-related attributes as [age, gender, race]. But a user may require to change these default selections in order to analyze disclosures in a specific set of datasets. Moreover, the cluster formation is highly dependent of the selected privacy-related attributes. Thus, in order to find more joinable datasets (task \textbf{T1a}), a wordcloud of the most frequent attributes in each cluster is displayed below the 2D scatterplot of datasets(see Figure \ref{figs:interface}d). The most frequent attributes are shown in a larger font, thus helping the user choose the privacy-related attributes. This human interaction and continuous feedback loop is quite important since defenders may have domain expertise to observe attributes which are important in the privacy parlance.

%But a user may also be interested in understanding the frequency difference of the selected privacy-related attributes and the other highly frequent attributes. This can be fulfilled using the attribute bar chart which shows a sorted view of the frequency distribution of the top attributes(see Figure \ref{figs:interface}e). The selected privacy-related attributes are shown at the top, followed by the top-$5$ most frequent attributes in that particular cluster. A combination of the scatterplot, wordcloud and the bar chart is displayed for all the possible clusters of joinable datasets, ranked by the clustering metrics so that best cluster is always shown at the top. After selecting the desired set of privacy-related attributes, user can select any set of dots from the 2D scatterplot and their corresponding combination of datasets will be shown on the right-hand side, so that the defenders can compare the risk of these dataset combinations, as described in Section \ref{section:risk_explanation_view}.

%In order to implement the attack scenario described in Section \ref{section:attack_scenario2}, a separate view was implemented in PRIVEE. Lower counts of a certain category of attributes can be detected by developing a bar chart/histogram for each of  the corresponding attributes of each dataset. Thus, a view was developed where a bar charts would be shown for the selected privacy-related attributes if they were categorical in nature while a histogram would be shown if they are numerical in nature (see Figure \ref{figs:scenario3}c). The bars for the categorical attributes would show the frequency of each of the different categories of this attribute. The numerical attributes would be divided into bins of equal intervals and the corresponding bars would display the frequency of each of the bins. The bins with lower number of records would be displayed in red (\textbf{T1b}).

%These bar charts/histograms would be displayed for all the datasets selected through the different filters iff they have all the privacy-related attributes selected by the user. In case multiple datasets are selected, PRIVEE sorts these datasets based on the lowest frequency of a bin and the number of such dangerous/low count bins (bins with frequency $\leq 4$) . For example, if a Dataset A has only $2$ records for race="Hawaiian" while Dataset B has $1$ record for age=19-20 and 1 record for the race="Black", Dataset B will be displayed first, followed by Dataset A. Any such dataset can be selected from this view to compare the risk of disclosure with respect to each of the individual-record level datasets available in PRIVEE (see Figure \ref{figs:scenario3}e).

%The bins for each of the privacy-related attributes were pre\-calculated using an algorithm developed specifically for this purpose. This cannot be done as an on-demand basis since it would include an overhead of downloading the datasets and processing them through this algorithm, which would render the interface useless due to the unusually high processing time.


\section{Compare Joinability Risks of Dataset Pairs~(G3)} \label{section:joinability_risk}

The design requirement for addressing G3 is to facilitate \textit{efficient visual comparison} of the risk profile of dataset pairs and guide defenders towards focusing on high-risk dataset pairs. 
This section describes the metrics that can help a data defender quantify the risk of joinability between the candidate datasets and the subsequent use of visual cues to compare and prioritize the joinable pairs. 

\subsection{Metrics for evaluating joinability risk} \label{section:risk_score_calculation}

\textbf{Based on attribute profile:} Shannon’s entropy is a measure of the uncertainty of a random variable ~\cite{cover1999elements}. It has been used as a privacy metric~\cite{serjantov2002towards,diaz2002towards,oganian2003posteriori,alfalayleh2014quantifying}, as higher entropy of an attribute in a dataset means more unique values for that attribute, thus resulting in higher disclosure risk. We used this metric to help defenders find joinable attributes for a pair of candidate datasets. For each pair of datasets, we calculated Shannon's entropy of each of their shared attributes according to equations \ref{equation:entropy_A} and \ref{equation:entropy_B}. We used equation \ref{equation:entropy} to calculate the final entropy score for that attribute. The intuition here is that the attributes with higher entropy can be offered as suggestions to the defender for the join key; hence the shared attributes are sorted according to their final entropy score in descending order.
\begin{equation}
    H(X_{A}) = -\sum_{i=1}^{n} P(x_{A_{i}}) \ln P(x_{A_{i}})
    \label{equation:entropy_A}
\end{equation}
\begin{equation}
    H(X_{B}) = -\sum_{j=1}^{m} P(x_{B_{j}}) \ln P(x_{B_{j}})
    \label{equation:entropy_B}
\end{equation}
\begin{equation}
    H(X) = \max\{H(X_{A}), H(X_{B})\}
    \label{equation:entropy}
\end{equation}
where:
\begin{description}
\item [$H(X)$] = entropy of an attribute present in two datasets A and B
\item [$X_{A}$] = attribute X in dataset A,
\item [$X_{B}$] = attribute X in dataset B,
\item [$x_{A_{i}}$] = each category of the attribute $X_{A}$ in dataset A,
\item [$x_{B_{j}}$] = each category of  the attribute $X_{B}$ in dataset B.
\item 
\end{description}
\textbf{Based on dataset pairs in a join:}
%Joining attributes are the number of common attributes between two datasets. 
Since the joinability of two datasets depends upon the number of shared features/attributes between them, the joinability risk score can be calculated as a function of the number of shared attributes and the number of privacy-related attributes between a pair of candidate datasets. The formulae for the joinability risk score can be defined as follows:
\begin{equation}
    \text{risk} = \alpha * p + (c-p)
    \label{equation:risk_score}
\end{equation}
where:
\begin{description}
\item [$\alpha$] = a constant, representing the empirical risk ratio
\item [p] = the number of privacy-related attributes,
\item [c] = the number of shared attributes
\end{description}

\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{figures/risk_assessment_v2.pdf}
 \caption{\label{figs:risk_and_disclosure}\textbf{Comparison of joinability risk and detection of disclosures.} (a) the distribution of the privacy-relevant attributes in the joinable dataset pairs and (b) their risk score distribution. (c) a joinable pair with a sorted bar chart of the shared attributes between them while (d) their joinability risk. (e) visualizing the shared records when the datasets are joined using the privacy-relevant attributes while (f) the data distribution of the attributes having high mutual information with the joining attributes. (g) a record with where an individual can be identified even if the location is partially masked.}
\end{center}
\vspace{-2mm}
\end{figure*}

The joinability risk score depends on the empirical risk ratio, and to determine its value, we designed an experiment to calculate the risk scores of all the possible combinations of joinable pairs from the seed datasets ($\Comb{426}{2} = 90,525$ combinations). 
%Since there are a total of $426$ datasets, this experiment calculated the risk score of $\Comb{426}{2}$ i.e., $90,525$ pairwise combinations of datasets. 
This experiment was repeated multiple times, each time with a different value of the risk ratio, ranging from $1$ to $100$. We observed that the value $\alpha = 50$ works well to separate the dataset pairs with privacy-related attributes and pairs without them. Hence the empirical risk ratio was fixed at the value of $50$. If two datasets have $15$ shared attributes and only $2$ of them are privacy-related attributes, the risk score can be calculated as $113$, as per equation \ref{equation:risk_score}. A higher joinability risk score signifies that this dataset pair is highly joinable, which can be a step closer to finding disclosures.
 We have included further details about these experiments in the supplementary materials.

\subsection{Risk Assessment View} \label{section:risk_explanation_view}


The number of possible pairwise combinations of the candidate datasets can be pretty high and PRIVEE can help a data defender analyze the risk of these datasets at the dataset and feature levels. The Risk Assessment View uses visual analytic components to encode these metrics so that data defenders can pro-actively analyze the risk between the candidate datasets.

Each dataset pair is represented using a sorted bar chart, where the x-axis represents the shared attributes between them and the y-axis means the entropy score of each of these attributes. This encoding helps the user visually compare the number of shared attributes present in each dataset pair along with their risk profile. The bars for the privacy-related attributes are colored in salmon red to provide a quick visual guide towards understanding the relative importance of these attributes compared to the other shared attributes. Users can select any attribute combinations from this bar chart to join the datasets and evaluate them for actual disclosures. As illustrated in Figure \ref{figs:risk_and_disclosure}c,  the datasets \textit{Electronic Police Report 2016} and \textit{Electronic Police Report 2015} have $21$ shared attributes, including all of the $4$ privacy-related attributes.

This high number of shared attributes leads to a high joinability risk score, as determined from equation \ref{equation:risk_score}. This information has been encoded in a colored gradient bar, as shown in Figure \ref{figs:risk_and_disclosure}e. The color gradient helps abstract the actual joinability risk score into a normalized format so that data defenders can visually determine the severity of the risk. Each of the dataset pairs is ranked according to their joinability risk score so that the ones with the higher joinability risk are shown at the top.

PRIVEE also has a risk description section which can help the data defenders understand the overall risk profile of the dataset pairs in a joinable group of candidate datasets. Figure \ref{figs:risk_and_disclosure}a shows the distribution of the privacy-related attributes and highlights the fact that the privacy-related attributes are present in $10$ of the dataset pairs in this view. Figure \ref{figs:risk_and_disclosure}b shows the distribution of the actual risk score so that the user can map their real joinability risk to the abstracted version shown in the colored gradient bar (Figure \ref{figs:risk_and_disclosure}b). This distribution can also be used as a filter to view only those pairs of datasets within a specific range of risk scores (high/low).

Ranking the different dataset combinations helps the defender to analyze the risk associated with each of the combinations (\textbf{T4}). The visual cues can help the defender choose a combination more prone to disclosure risk. After comparing these risks of the different pairwise combinations of datasets, defenders can select any pair with some of the joining attributes to understand the eventual join outcome.






%As mentioned earlier, each of these combinations are sorted primarily according to the risk score and secondarily according to the average entropy of the selected attributes, if any.


%After the selection of a cluster of datasets from the dataset joinability view (see Section \ref{section:dataset_joinability}), it is prudent to find out which pair of datasets have a higher risk of disclosure. For example, if a user selects a cluster with $7$ different datasets, there can be $\Comb{7}{2}$ i.e., $21$ pair-wise combinations of datasets and if the user selects a cluster with $15$ datasets, there can be a total of $\Comb{15}{2}$ i.e., $105$ pair-wise combinations of datasets.In order to rank all these combinations of datasets for disclosure, hence PRIVEE has introduced a joinability risk score which scores each dataset combination on certain parameters and the sorts them accordingly. 

%Each pair of dataset is represented using a combination of multiple elements, including a radio button, the dataset names, and a sorted bar chart, where each bar represents the joining attributes present between these datasets(refer Figure \ref{figs:interface}i) and its height denotes the entropy of that attribute. The bars marked in salmon red are the privacy-related attributes selected by the user. As mentioned earlier, each of these combinations are sorted primarily according to the risk score and secondarily according to the mean entropy of the selected attributes, if any.

%Using the equation \ref{equation:risk_score}, it was observed that the joinability risk score for most of the $90,525$ pairwise dataset combinations range between $0$ to $182$. This is represented by a linear gradient from the color grey to red, where grey marks the lower end while red marks the higher end (see Figure \ref{figs:interface}j). The position of the black bar signifies the joinability risk of each pair of dataset. 

%If there are multiple pairwise dataset combinations, a user may be interested in those combinations which lie within a certain risk score range. This can be implemented using the \textit{risk score filter}, which shows a histogram distribution of the risk scores of all the dataset combinations (see Figure \ref{figs:interface}h). Moreover, the \textit{frequency bar chart} on the left-hand side of the risk score filter also helps to understand the distribution of the privacy-related attributes in these pairwise combinations of datasets (refer Figure \ref{figs:interface}g).

%Ranking the different dataset combinations helps the defender to analyze the risk associated with each of the combinations (\textbf{T2}). The visual cues can help the defender choose a dataset combination more prone to disclosure risk. After comparing this risks of different pairwise combination of datasets, defenders can select any such pair using the radio button along with of the attributes of interest which can be used to join the datasets. Further details about the joining the datasets at the record-level have been discussed in the next section.

\begin{figure*}[ht]
\begin{center}
\includegraphics[width=\textwidth]{figures/scenario3_v2.pdf}
\vspace{-4mm}
 \caption{\label{figs:scenario3}\textbf{Usage Scenario for data subjects.} (a) selecting datasets based on their metadata like the popular tag "health" and their granularity of records, (b) diagnosing the vulnerable data distributions and observing that there is only $1$ record for the race "Hawaiian/Alaskan", (c) comparing the joinability risk with the individual record-level datasets and (d) evaluating the disclosures with the top $4$ individual-level datasets and observing that there is no disclosure~(Section \ref{section:scenario3}). }
\end{center}
\vspace{-6mm}
\end{figure*}

\section{Detection of Disclosure at a Record-Level (G4)} \label{section:disclosure_detection}



The design requirement for addressing T5 and T6 is to let defenders \textit{judge the degree of sensitive information} that can ultimately be disclosed through the joins. Since an apriori definition of risky features is insufficient, PRIVEE also suggests additional features to defenders for diagnosing sensitive matches.

\subsection{Metrics for evaluation of disclosures} \label{section:mutual_information}


\textbf{Based on the low frequency of matching records:} Matching records are the number of records in the joined dataset. The presence of matching records can indicate the possible disclosures at the record level. But the number of matching records may vary according to the choice of joining attributes and the type of records present in the datasets. For example, Dataset $A$ and Dataset $B$, when joined on attributes $x$ and $y$, may have $200$ matching records, but when joined on the attributes $x$, $y$ and $z$, may have only $20$ matching records. This implies that the attribute combination $x$, $y$, and $z$ have a better chance of discovering an actual disclosure than the combination $x$ and $y$. We have also observed that the number of matching records may contain duplicates if the original datasets have duplicate or blank entries. 




\noindent\textbf{Based on the mutual information between the joining attributes:} The selection of the joining attributes is an iterative process in PRIVEE. We use normalized mutual information to suggest other features which defenders can use for detecting disclosures. Mutual information is the measure of the amount of information one random variable contains about another~\cite{cover1991entropy} and quantifies the mutual dependence of the two attributes of a dataset. We calculated the normalized mutual information between the joining attributes and the other attributes of the joined dataset. Next, we find the top-$5$ attributes with the highest mutual information score and let defenders consider those features for detecting matches.




\subsection{Disclosure Evaluation View}

In this view, we visualize the matching records of the joined datasets using a modified parallel sets visualization. Parallel sets is a visualization method for the interactive exploration of categorical data, which shows the data frequencies instead of the individual data points~\cite{kosara2006parallel}. We adopted and extended this technique for visualizing the relationship among the different categories of the privacy-relevant attributes in the joined dataset, yet retaining the granularity of the dataset at the record level. As illustrated in Figure \ref{figs:risk_and_disclosure}e, each joining attribute is represented using a stacked bar, where the height of the stacks represents the frequency of the respective categories. For numerical attributes, the stacked bar is replaced by a histogram to show their distribution. In this case, the numerical data is divided into four equal bins to map them with the categories of the other attributes. The categories in the different stacked bars are connected using weighted lines. Each line's weight/thickness represents the number of records in the joined dataset belonging to both categories.



In Figure \ref{figs:risk_and_disclosure}g, we can observe that there is a thin line between the \textit{offenderage} $22$ and the \textit{location} "6XX Tchoupitoulas St". Further investigation shows the details of this actual record in a table pop-up view. This reveals that a $22$ year old black male was charged with attempted robbery with a gun against a $27$ year old white male at 6XX Tchoupitoulas St on $13$\textsuperscript{th} July, $2015$ at $01$:$00$ hrs and again on $30$\textsuperscript{th} April, $2016$ at $03$:$00$ hrs with attempted simple robbery. This is an example of identity disclosure where an individual was identified even when the address was partially masked (\textbf{T5}).





\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{figures/scenario1_v2.pdf}
\vspace{-2mm}
 \caption{\label{figs:case_study}\textbf{Case study with domain expert.} (a) the expert selected the datasets from the Albany Police Open Data portal, which are shown in the dataset joinability view, along with the popular attributes in these datasets, (b) the risk assessment view showed the pairwise combinations of these datasets and their joinability risk, (c) one of the pairs when joined on the quasi-identifiers age, sex, neighborhoodxy and date showed only $4$ matching records, (d) analyzing the records showed an example of identity disclosure where a person was stopped for field interview and was  cited just 3 minutes later~(Section \ref{section:case_study}).}
\end{center}
\vspace{-2mm}
\end{figure*}

PRIVEE uses the normalized mutual information score to find the attributes similar to these joining attributes. As shown in Figure \ref{figs:risk_and_disclosure}f, the data distribution of the attributes with the most mutual information with the joining attributes are shown in the left and right-hand side of the modified parallel sets visualization. These attributes can be used as suggestions for improving the initial set of joining attributes (\textbf{T6}).
%se pairs of datasets within a specific range of risk scores (high/low).




%Ranking the different dataset combinations helps the defender analyze the risk associated with each of the combinations (\textbf{T4}). The visual cues can help the defender choose a combination more prone to disclosure risk. After comparing these risks of the different pairwise combinations of datasets, defenders can select any pair with some of the joining attributes to understand the eventual join outcome.


%After the selection of the datasets pair and attributes of interest from the risk assessment view, defenders need to evaluate the possible disclosures after joining these datasets. For example, joining two datasets on few attributes may reveal that there are no common records between them, which implies these datasets can be safely joined in order to use the combined dataset for further research. Again, for example, if there are $4$ common records while joining two datasets, it implies that these datasets cannot be joined in order to prevent identity disclosure. 





%After joining a pair of datasets, if there are few common records, these records are inspected for the presence of different categories of the attributes of interest and each such category is plotted as a bar in a stacked bar chart. For example, if the common records contain two genders, namely Male and Female, the stacked bar chart will contain two bars, one of each category (see Figure \ref{figs:scenario1}d). But if there are multiple values of a numerical attribute of interest (like age), a histogram is developed with equally distributed bins. Each category of the attributes of interest is then connected using a line where the thickness of the line depicts the number of records containing these categories of these attributes (see Figure \ref{figs:scenario1}d). For example, if there are $3$ records of gender = Male and race = White while $10$ records of gender = Male and race = Black, then the line originating from gender = Male towards the race = Black will be thicker than that originating from gender = Male towards the race = White. Clicking on each of these lines will display the actual records. Moreover, in order to aid the selection of joining attributes, PRIVEE calculates the mutual information between the selected joining attributes and the other attributes of the joined dataset. The top-5 attributes with highest mutual information with the joining attributes are shown on the either side of this view. The connections between these attributes and the joining attributes can also be further explored by selecting these attributes.



==> sections/old/privee_visualization.tex <==
\section{PRIVEE: Visualization and Interaction Design}
% \aritra{Describe the visualizations and interactions here. WHy don't you name the views, for example, risk explanation view, data joinability view and use them as section names?}
% \kaustav{Updated this section with different names for the different views}
% \kaustav{Also updated according to the new design}



In this section, we describe the different visual components of PRIVEE and their rationale behind the design choices. 
\begin{comment}


\subsection{Filter Area} \label{section:filter_area}
During early discussion with domain experts, it was evident that users may want to select a subset of datasets instead of all the dataset available to them, in order focus more on possible disclosure risk local to a certain type of dataset. PRIVEE has multiple filter options, baked right right at the top bar of the screen. The filter options include 

\begin{enumerate}
\item \textit{Type of dataset:} During dataset analysis, it was observed that datasets can have two type of records:
\begin{itemize}
\item \textit{individual records:} where each record corresponds to a single individual, like arrests dataset, medical records etc.
\item \textit{aggregated records:} where each record corresponds to the aggregated values for a certain category, like disease infection in a county, education levels in a district etc.
\end{itemize}
Users can filter the datasets according to their type of records (see Figure \ref{figs:interface}a). PRIVEE has a collection of around $151$ individual-record level datasets and around $275$ aggregated-record level datasets.
\item \textit{Popular tags:} The data portals label each datasets with few tags which generally portray the popular keywords related to each dataset. During the selection of datasets, the tags were analyzed for their frequency in this collected datasets. This sorted list of tags are available in the filter area (see Figure \ref{figs:interface}a) where the users can filter the datasets based on their tags/keywords of choice.
\item \textit{Data portals:} As mentioned earlier, data experts may be interested in analyzing the datasets from a certain data portal only. This can be achieved by selecting the relevant data portals from the list of the portals available in the filter area (see Figure \ref{figs:interface}f). A complete list of the portals can be found in the appendix.
\item \textit{Type of plot:} PRIVEE has two different types of plots available in order to cater to different attack scenarios. In order to implement the attack scenario through joinable datasets (Section \ref{section:attack_scenario1}), PRIVEE has projection plots along with the clusters, word cloud and the bar chart of the popular attributes. But in order to implement the attack scenario through unique records (Section \ref{section:attack_scenario2}), a different view of histograms can be loaded using the options available through the filter area (see Figure \ref{figs:interface}a)
\end{enumerate}




\subsection{Attribute Selection Area} \label{section:attribute_selection_area}
There has been multiple examples where quasi-identifiers like age, gender, race, location etc. were used to find disclosure in datasets. Thus, it was prudent to develop a dictionary of such privacy-related attributes which can aid in finding datasets of interest (\textbf{T1}). These attributes are given more weightage while finding the clusters of joinable datasets (see Section \ref{section:weight_selection}). Hence, the individual level datasets were analyzed and a list of attributes  were identified which are related to the quasi-identifiers age, gender and race.  Some of the privacy-related attributes are as follows: ["age\_group", "vic\_age\_group", "susp\_age\_group", "perp\_age\_group", "vict\_age","age\_1", "age\_at\_release", "admission\_age", "age\_class", "subject\_age", "patient\_age", "age\_range", "offender\_age", "officer\_age", "age\_at\_arrest","sex", "susp\_sex", "vic\_sex", "perp\_sex","sex\_1",  "victim\_gender", "suspect\_gender", "complainant\_sex", "officers\_sex",  "susp\_race", "vic\_race", "perp\_race", "vict\_descent",  "victim\_race", "suspect\_race", "complainant\_race", "officers\_race","subject\_race", "officer\_race"]. Users can choose any combination of these attributes through \textit{PRIVEE} (see Figure \ref{figs:interface}b).

\end{comment}
\subsection{Dataset Joinability View}
Finding joinable datasets is one of the critical tasks required to emulate the attack scenarios. After filtering the datasets based on their type of records, tags and the data portals, multiple methods have been used to find the optimum process to find datasets which are similar in their attribute space(see Section \ref{section:dataset_joinability} and the most intuitive method to show a cluster of datasets is using a 2-D scatterplot(see Figure \ref{figs:interface}c). In this scatterplot, the datasets are projected as dots while the best cluster of dots are highlighted in red color. PRIVEE has a default selection of privacy-related attributes as [age, gender, race]. But a user may require to change these default selections in order to analyze disclosures in a specific set of datasets. Moreover, the cluster formation is highly dependent of the selected privacy-related attributes. Thus, in order to find more joinable datasets (task \textbf{T1a}), a wordcloud of the most frequent attributes in each cluster is displayed below the 2D scatterplot of datasets(see Figure \ref{figs:interface}d). The most frequent attributes are shown in a larger font, thus helping the user choose the privacy-related attributes. This human interaction and continuous feedback loop is quite important since defenders may have domain expertise to observe attributes which are important in the privacy parlance.

But a user may also be interested in understanding the frequency difference of the selected privacy-related attributes and the other highly frequent attributes. This can be fulfilled using the attribute bar chart which shows a sorted view of the frequency distribution of the top attributes(see Figure \ref{figs:interface}e). The selected privacy-related attributes are shown at the top, followed by the top-$5$ most frequent attributes in that particular cluster. A combination of the scatterplot, wordcloud and the bar chart is displayed for all the possible clusters of joinable datasets, ranked by the clustering metrics so that best cluster is always shown at the top. After selecting the desired set of privacy-related attributes, user can select any set of dots from the 2D scatterplot and their corresponding combination of datasets will be shown on the right-hand side, so that the defenders can compare the risk of these dataset combinations, as described in Section \ref{section:risk_explanation_view}.

\subsection{Dataset Unicity View} \label{section:dataset_unicity_view}







==> sections/old/problem_characterization.tex <==
\section{Problem Statement \& Tasks Characterization {\aritra{You don't write problem statement in a section name}}}

\aritra{Overall Comment: We don't need a separate problem and task characterization. These are natural derivatives of our red-teaming activities and must be framed as such. Try to think and articulate: for the attack scenarios identified, what role can visual analytics play? which tasks can be fully automated? which tasks need human intervention and why? how can visualization help in summarizing and explaining risks? how can visualization help spot risks that a data custodian might not know apriori, i.e., how can visualizations surprise a data custodian/owner with new insights?}

Removing explicit identifying information like name, social security number (SSN) etc. may not be enough in order to protect the identity of the individuals in a dataset. Linking attacks can still use a combination of quasi-identifiers like birthdate, gender, zip etc. to re-identify individuals. Moreover, open data portals have improved the access of these datasets, hence any information leaked from these datasets maybe shared with people all over the world. On top of that, the release and forget model practised by the data custodians does not help to protect the individuals against such attacks. Thus, it is important to pro-actively look out for such possible attacks and protect against these attacks. We propose a framework for visually identifying the such combinations of datasets and evaluate their risks.   In section section, we delve deeper into the problem and analyze the tasks required to solve it.

\subsection{Problem of re-identification in open datasets}

\begin{itemize}
\item \textbf{Data Discovery} In order to analyze the disclosure risk related to the linking attacks, it is very important to discover datasets which can be joined in order to extract meaningful information. As we know, open data portals hosts multiple datasets and they offer a search option too. But the search functionality is limited to basic keyword search along with some filters, in most of the portals. This won't be helpful in finding out joinable datasets which can lead to disclosure. This paper proposes methods to find joinable datasets from open data portals.
\item \textbf{Risk Analysis} Even if multiple joinable datasets are discovered, an attacker needs to analyze these combinations of datasets for their riskiness. For example, if there are $10$ such joinable datasets, this can lead to \textsuperscript{10}C\textsubscript{2} or $45$ pairwise combinations of these datasets. Our paper proposes visual aids and risk scoring methods to highlight those datasets with higher chances of disclosure through joining.
\end{itemize}

\subsection{Visual Analytic Tasks}\label{section:visual_analytic_tasks}

\aritra{These tasks are too granular, and T2 and T5 look very similar. The term "risky" dataset does not make sense. Also, are the tasks always in a sequence?}

% \begin{itemize}
\par \noindent \textbf{\textit{Find privacy-related attributes (T1):}} All attributes may not be equally important in the context of privacy. Selection of such attributes is an important factor in the analysis of disclosure risk since it acts as a pivot in the rest of the tasks. \aritra{How are we achieving this task in PRIVEE? To the best of my understanding, this is outside of the PRIVEE workflow.}

\par \noindent \textbf{\textit{Find joinable datasets (T2)}:} In order to find risky datasets, an attacker needs to find datasets which can be joined together. Due to the large size of the candidate dataset space, it becomes quite difficult to find such datasets. This task relates to finding datasets which are quite similar in the attribute space so that they can be joined together to find potential disclosure. \aritra{You are again making this error of framing this around making something easy for the attacker. Are we helping the attacked find joinable data sets?}

\par \noindent \textbf{\textit{Find datasets with lower number of records (T3):}} According to the attack scenario (Section \ref{section:attack_scenario2}), finding datasets with very low count of certain attribute categories may still lead to disclosure. Datasets which are aggregated in order to suppress individual level records can still be used to identify an individual if a certain attribute has a very low count of a certain category. This task relates to finding such datasets and the corresponding attribute which can lead to such disclosures.

\par \noindent \textbf{\textit{Assess risky dataset combinations (T4):}} After finding such risky datasets, it is necessary to understand which dataset combinations possess higher risk of disclosure. The risk may vary between different dataset combinations based on the number of joining attributes, privacy-relevant attributes and their entropy. This can be formulated using a risk score, which can be used to compare the risk of the different combinations of datasets and select the ones which are more prone to disclosure.

\par \noindent \textbf{\textit{Find joinable attributes (T5):}} Each pair of dataset combination can have different risk based on the joining attributes. For example, two datasets may have multiple common records when joined on the attributes age and race but may not have any common records when joined on age, race and location. This implies that the datasets can be joined together safely, based on these attributes. hence selection of joinable attributes is an important task towards finding disclosure.

\par \noindent \textbf{\textit{Evaluate disclosure (T6):}} For each pair of datasets, it is necessary to evaluate if joining them based on certain attributes would lead to any disclosure or not. Linking attack on the datasets may lead to identity disclosure of the individuals present in a dataset or disclosure of sensitive attributes for some of these individuals. This paper proposes a set of \aritra{visualizations} to evaluate the potential disclosures when joining these datasets. 
% \end{itemize}

==> sections/old/relatedWork.tex <==

\section{Background and Related Work}

Privacy-preserving data publishing and mining research has developed a suite of anonymization methods~\cite{fung2010privacy} addressing the problem of linking among public and private datasets, for example, between Census data and hospital records. The most promising among those methods is the notion of differential privacy that has recently been adopted by the US Census. However, besides US Census data, which is just one of the sources of openly available data about people and their behavior, there are now a plethora of open data portals. The adoption of open data portals is a recent phenomenon, with the promise of transparency and utility as depicted by the FAIR principles~\cite{wilkinson2016fair}, and at the same time, with the need for adherence to emerging privacy laws~\cite{nouwens2020dark}. The unrestricted availability of open data~\cite{green2017open} naturally raises the question: what if datasets within the open data ecosystem are linked even without any other sensitive information from private datasets? Researchers have recently expressed the need to investigate privacy issues in open data portals. Lavrenovs and Podins showed how the privacy of passengers can be violated through the public transportation open data, released by the city municipal of Riga, Latvia\cite{lavrenovs2016privacy}. Recent studies have demonstrated how even heavily anonymized datasetscan be used to re-identify about $99\%$ of Americans~\cite{rocher2019estimating}. Re-identification or disclosure of sensitive information is a challenge that has been previously explored by multiple researchers\cite{de2015unique, de2013unique, zang2011anonymization}. Risk of re-identification can be considered as a temporal function which is dependent on the datasets available at the time of analysis. Sekara et al. have recently performed a study which shows that this risk varies over time for the re-identification using smartphone app usage dataset with publicly available information\cite{sekara2021temporal}. But, data owners often practice the ``release and forget" model where datasets, once released, are not analyzed further for potential privacy risks with respect to the newly released datasets\cite{ohm2009broken, rubinstein2016anonymization}. This may lead to inadvertent breach of privacy when new datasets are released which, when joined with the existing datasets, can leak sensitive information. Thus it is necessary for the data owners to proactively monitor the the risks of their datasets with respect to other datasets available through the various open data portals and keep checking on a regular basis. We developed the PRIVEE workflow and visualization interface with this specific goal of realizing a defender-in-the-loop analytical framework that can be privy to the disclosure risks or possibility of accidental leakage of sensitive information whenever new datasets are released. The target users of PRIVEE are mainly data custodians or data owners but even data subjects~\cite{bhattacharjee2020privacy} themselves can use the workflow to inspect how vulnerable their identity or personal information might be, in the presence of multiple, linked data sets. We use the concept of dataset joinability~\cite{miller2018making} in the presence of quasi-identifiers as a means for calibrating discloure risks that are communicated using interactive visualizations throughout the PRIVEE workflow. While we do find examples of visualization techniques for expressing disclosure risks of individual datasets~\cite{kao2017using,dasgupta2019}, visualizing disclosure risk among multiple datasets, with input from data defenders, is largely an open problem that we address in PRIVEE.

% We first conduct a red-teaming study for linking open datasets among themselves with no additional information, starting from the universally agreed upon yet narrow definition of quasi-identifiers or protected attributes like age, race, gender, etc. 





% GDPR~ aim to protect data subjects against such malicious attacks by enforcing strict regulations for releasing data,

% WHO is PRIVEE for:
% A data custodian, like Cambridge Analytica, needs to have checks and balances in place to ensure people's identities are not revealed due to the use of demographic data. Data consumers, like a social scientist trying to understand the correlation between demographics and economic indicators of a region, need to derive value out of anonymized data and overcome the potential loss of value due to suppression or omission of sensitive information.



% % This proliferation and easy accessibility of open data has also provided an opportunity to all these users to collect multiple datasets and join them to find disclosures. Thus, it is necessary to analyze the potential privacy risks of open datasets so that the private information of the citizens participating in these datasets are protected against data leakage.




% Data owners thus need to rigorously identify risks before releasing the data. Kao et al.~\cite{kao2017using} presents a novel visualization interface named ODD visualizer which will help in open data de-identification, i.e, if  there is any privacy leakage in the dataset. It uses heat maps to display $k$-anonymity and $l$-diversity distributions. This is similar to the approaches of Castellani et al.~\cite{castellani2015urban}, who propose a visualization based data profiler for understanding potential vulnerabilities in openly available city data, and Deeb-Swihart et al., where they evaluate strategies to help law enforcement officials combat human trafficking while ensuring privacy protection~\cite{deeb2019understanding}.

==> sections/old/techniques.tex <==
\section{Techniques \& Methods}

 Open data portals host multitudes of datasets across different topics ranging from restaurant inspections to arrests and criminal records, available openly to anyone, including an attacker and a defender. But finding datasets to join still remains a challenge. In traditional way, an attacker interested in finding such datasets needs to visit each open data portal, search for relevant keywords and then analyze each of the datasets for joinability. We decided to partially automate this process and improve it with the help of user inputs. In this section, we describe our process for the selection of the datasets and the subsequent techniques used to find joinability among them. 

\subsection {Selection of Datasets}
Socrata' s API (\url{https://dev.socrata.com/})is a powerful tool to collect relevant datasets from the open data portals. It allows the user to query the open data portals and access their data resources along with their metadata.  We collected a list of domains (data portals) available through this API and selected those which have at least 2 resources available (\textit{query}: "\url{http://api.us.socrata.com/api/catalog/v1/domains}"). These portals, by governments, non-profits and NGOs, contain variety of the data resources like datasets, maps etc., along with content generated by consumers around the world who save their content like charts, maps, filtered views into these open data portals. Hence, we decided to keep only the resources which were marked "provenance=official", i.e., these resources have been uploaded by the administrators of the respective portals and further filtered them to keep only the datasets. In this process, we collected metadata like column names, permalink, number of rows and the tags for around 8400 datasets. This set of datasets was further filtered to a set of 5400 datasets which contained some form of quasi-identifiers like age, gender, race and location. After carefully analyzing the datasets, it was observed that most of them are of aggregate level, instead of being individual level. Individual level datasets generally have records where each record correspond to a certain individual, like arrests, medical records etc., while aggregate level datasets are generally aggregated for a certain category, like disease infection in a county, education levels in a district etc. Hence, we categorized these datasets into two explicit parts:
- individual level datasets: identified around 150 datasets
- aggregate level datasets: identified around 289 datasets which have at least one of attributes from age, gender and race.

\subsection {Selection of Privacy-related attributes}
It is generally  understood that some attributes may be more relevant in the context of privacy than others. There have been examples where quasi-identifiers like age, gender, race, location etc. have been used to find disclosure between datasets. Thus, it is prudent to create a dictionary of such privacy-related attributes which can help in finding join-able datasets  with those attributes. The datasets containing these attributes may be more vulnerable for disclosure if they contain these attributes. Hence, the individual level datasets were analyzed and a list of attributes  were identified which are related to the quasi-identifiers age, gender and race.  The list is as follows: ["age\_group", "vic\_age\_group", "susp\_age\_group", "perp\_age\_group", "vict\_age","age\_1", "age\_at\_release", "admission\_age", "age\_class", "subject\_age", "patient\_age", "age\_range", "offender\_age", "officer\_age", "age\_at\_arrest","sex", "susp\_sex", "vic\_sex", "perp\_sex","sex\_1",  "victim\_gender", "suspect\_gender", "complainant\_sex", "officers\_sex",  "susp\_race", "vic\_race", "perp\_race", "vict\_descent",  "victim\_race", "suspect\_race", "complainant\_race", "officers\_race","subject\_race", "officer\_race"]. This gave us an initial list of privacy-related attributes to start with and it can be further modified from the user interface \textit{PRIVEE}.

\subsection {Techniques for finding joinability} \label{techniques_for_finding_joinability}
\subsubsection {Link2Vec}

The overall assumption for finding joinability is that datasets with similar attributes can be joined together to find disclosure. Hence, the obvious way to find joinability was to find the number of possible joining attributes between two datasets.  An algorithm was developed to calculate the number of common attributes between the individual datasets and each of the other 5400 datasets collected through the open data portals.  For example, if the individual level dataset Dataset A has the attributes ["age", "gender", "race"] and another dataset Dataset X has the attributes ["age", "gender"], so there are two common attributes between them. Similarly,  the common attributes were calculated between Dataset A and all the other datasets and it was stored as a vector of numbers, where each number represented the number of common attributes between the individual dataset and the other dataset.. This vector can also be called a vector of links (common attributes), hence we named this method as Link2Vec, a name similar to the word2vec approach used by different word embedding methods. This Link2Vec vector was calculated for all the individual datasets. But in order to visually analyze the datasets, it is prudent to plot their corresponding vectors on a 2D scatterplot. Since these vectors were of high dimension (1 X 5400), these were reduced to lower 2-dimension vectors using dimensionality reduction techniques like t-distributed Stochastic neighbor embedding (t-SNE)\cite{van2008visualizing}.  Clustering technique like DBSCAN was used to identify clusters and visually identify them using the color channel in the 2D scatterplot. In this approach, datasets which were plotted nearby in the scatterplot should be more joinable.

Since finding joinability is the first step towards finding disclosure, it is intended that the datasets which actually have more disclosure risks should be highlighted more in the 2D scatterplot. Hence we included the privacy-related attributes along with the Link2Vec vectors to emphasize  more on the datasets which may be more vulnerable  for disclosure. But it was observed that using the privacy-related attributes did not change the results significantly, even after using different weights for these attributes (\textit{The process of adjusting the weights for these attributes have been explained in the further sub section \ref{choosing_appropriate_weights}}). Thus, we decided to pursue another approach to find joinability between datasets and adjust them according to the privacy related attributes.

\subsubsection {AttributeText}
Since Link2Vec was not performing well for the privacy relevant attributes, we intended to find another method which will respond to the extra weights added by these attributes. Since we already had a the column names for each of the datasets, they converted them into numerical word embeddings using the spaCy library. This library analyzes each of the column names and converts them into a vector representing it. Then a sum of all the vectors is calculated to generate a single vector of dimension 1 X 300.  Since, again we have a high dimension vector similar to that of the Link2Vec method,  t-SNE  was to reduce it into a lower dimension. It is to be noted here that since these vectors are merely a numerical representations of the column names, hence cosine similarity was used as the distance metric instead of the Manhattan distance in the t-SNE algorithm. DBSCAN algorithm was used to find the clusters and it was observed that  this technique performs better than the Link2Vec technique. Calinski-Harabasz Index is used to measure the performance of clustering algorithms and it is defined as the ratio of the between-cluster dispersion and the inter-cluster dispersion,  where dispersion means the sum squared distance between the samples and the barycenter. Higher score signifies that the clusters are far away, that implies better clusters. The Link2Vec method had a Calinski-Harabasz Index of $19.43881940249555$ while the AttributeText technique had a score of $30.420922241056488$, signifying that it was performing better than Link2Vec. Hence, we chose this technique for further observations and implemented the same in the interface \textit{PRIVEE}. A further comparison of these two techniques can be observed from Fig. \ref{figs:methods1}
\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{figures/methods1_cluster_comparison.pdf}
\vspace{-4mm}
 \caption{\label{figs:methods1}\textbf{\textcolor{red}{(To be updated)} Comparison between Link2Vec and AttributeText techniques} This figure compares the clusters of AttributeText when (a) weight=1 (b) weight=8 and (c)weight=17 with the clusters of Link2Vec when when (d) weight=1 (e) weight=8 and (f)weight=17. It can be observed that there is no significant change to the Link2Vec clusters while using different weights. Refer Section \ref{techniques_for_finding_joinability}  }
\end{center}
\vspace{-6mm}
\end{figure*}

\subsection {Choosing appropriate weights } \label{choosing_appropriate_weights}
It is assumed that adding more weights to the privacy related attributes will help them being plotted more closely in  the 2D projection plot. This will help the user  to select those dataset combinations and analyze them further for disclosure risks. Hence, we designed an experiment to adjust the weights and analyze the resulting clusters. the experiment started with a weight of 1 and created a vector  which will highlight if a certain privacy-related attribute is present in the dataset or not. For example, if a user selects the set of privacy-related attributes [age, gender, race] and if Dataset A has only the age attribute while Dataset B has the age and race attributes, then the corresponding vectors would be $[1, 0,0]$ and $[1,0,1]$ respectively. Next, we appended  the vectors generated through the AttributeText method to these vectors. These combined vectors were then reduced in to  2-dimension vector s using t-SNE dimensionality reduction algorithm and DBSCAN algorithm was used to find clusters\cite{ester1996density,schubert2017dbscan}. Though this showed some initial clusters, these clusters were not geared towards clustering the ones with the privacy related attributes in the same cluster.

It was realized that a mere weight of 1 would not affect the clusters performance to a great extent.  Hence the weights were increased and their performance was analyzed. We tried with all the weights in the range $1$ to $100$ and checked the corresponding clusters. Other than the Calinksi-Harabasz Index (CH) described before, clustering metrics like Silhouette Score (SS) and Davies-Bouldin Index(DB) were also used to analyze the clusters. It was observed that almost distinct clusters start to form at weight=$4$. At weight=$8$, the clusters were  more prominent and their scores were S=$0.4570675$, CH= $641.3454566125303$, DB= $0.880139861638646$. At weight =$17$, the clusters were little bit more prominent and their scores were S=$0.84298706$, CH= $1055.1405222195654$, DB= $0.15986152904$ . At higher weights, the clusters remained more or less similar. This experiment was also tried on the full set of privacy related attributes collected earlier and observed that though the scores and the clusters are not that good at weight =$8$, weight =$17$ has excellent scores. Though  this experiment was also conducted using other combinations of the privacy related attributes, the observations were quite similar. Hence ,the  weights $8$ and $17$ were chosen as the candidate weights.

\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{figures/methods2_weights.pdf}
\vspace{-4mm}
 \caption{\label{figs:methods2}\textbf{Comparison between different weights} This figure compares the clusters of AttributeText at different weights  }
\end{center}
\vspace{-6mm}
\end{figure}

\subsection {Choosing clustering algorithms}
Since DBSCAN algorithm was already being used to generate the clusters, it was decided to check how the other clustering algorithms perform in this scenario. Hence these four clustering algorithms were chosen :
\begin{itemize}
\item DBSCAN \cite{ester1996density,schubert2017dbscan}
\item OPTICS \cite{ankerst1999optics}
\item KMeans \cite{vassilvitskii2006k}
\item Birch \cite{zhang1996birch}
\end{itemize}

We designed another experiment to check the performance of these algorithms with different weights and also different combinations of the privacy related attributes. For the attribute combination [age, gender, race] and weight =$1$ , DBSCAN and OPTICS performed more or less similarly but KMeans and Birch did not give meaningful clusters. Moreover,  is not recommended to use the previously  discussed metrics for KMeans and Birch algorithms since they generally produce higher results, hence  the quality of the clusters was checked instead of using those metrics for these algorithms. At higher weights, DBSCAN performed better than OPTICS and this is proved by their scores. While DBSCAN had Calinksi-Harabasz Index as $641.345466125303$, OPTICS has a Calinksi-Harabasz Index of $22.671327997926248$. The results were similar in even higher weights. Different combinations of privacy-related attributes were used and it was observed that DBSCAN and OPTICS perform almost the same when weight =1, but the former performs better with higher weights like $8$ and $17$. Hence, the DBSCAN algorithm was chosen for the whole process and was implemented in the interface \textit{PRIVEE}.

\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{figures/methods3_clustering_algorithms.pdf}
\vspace{-4mm}
 \caption{\label{figs:methods3}\textbf{Comparison between different clustering algorithms} This figure compares the different clustering algorithms.  }
\end{center}
\vspace{-6mm}
\end{figure} 

==> sections/old/usage_scenarios.tex <==

\section{Usage Scenario for Data Subjects} \label{section:scenario3}
\label{section:scenario1}


Sophia is a resident of San Mateo County in California. The county officials assured her that the citizens' data are not published directly to its open data portal \cite{SMCDatahub:online}, instead they are aggregated using different attributes like age, race, sex etc. Sophia was worried if her health data could be disclosed online, so she selected the aggregated datasets tagged with the keyword "health" in the interface PRIVEE and then selected the data portal of the San Mateo county (see Figure \ref{figs:scenario3}a). She also selected few privacy-related attributes like \textit{age}, \textit{sex} and \textit{race} since she was informed that the datasets are aggregated using these attributes (Figure \ref{figs:scenario3}b) (\textbf{T1}). 
While analyzing the vulnerabilities in the data distributions, Sophia observed that the dataset \textit{Whole Person Care Demographics 2} \cite{WholePersonDemographics2:online} had only $1$ record where the race was "Hawaiian/Alaskan" (Figure \ref{figs:scenario3}c) (\textbf{T2}). This finding was a great cause of concern for Sophia since she identified herself as Hawaiian, and any dataset with a similar race category could potentially expose her health records. Thus, she started analyzing the risk of joining this dataset with all the individual-record level datasets available through PRIVEE, as shown in Figure \ref{figs:scenario3}c (\textbf{T4}). Since there would be around 151 dataset combinations (the number of individual-record level datasets available), she decided to filter those combinations with a higher risk score ($\geq 130$), using the filter available in the risk score distribution histogram. She decided to join these dataset pairs on the privacy-related attributes along with the location attribute \textit{geocodedcolumnn} since she wished to find datasets that contain information relevant to her location. She observed that none of the top-4 dataset pairs yield any common record when joined on these attributes (Figure \ref{figs:scenario3}d). Thus, Sophia concluded that though the aggregated dataset \textit{Whole Person Care Demographics 2} has a meager count of a particular race, it does not lead to any disclosure (\textbf{T5}).

\section{Case Study} \label{section:case_study}
% Refer to Lam et al.'s "Empirical studies in information visualization: Seven scenarios" and Sedlmair et al.'s "Design Study Methodology: Reflections from the Trenches and the Stacks" to justify that there are two forms of validation: Case study and Informal usability testing and analyst feedback
In this section, we report one of the case studies which our data privacy collaborator and co-author co-developed using the web interface of \textit{PRIVEE}. He is a senior researcher with more than  $15$ years of experience in privacy-preserving data analysis and used PRIVEE as a privacy auditor. Specifically, he wanted to find out if there are any possible disclosure risks with the datasets published in the open data portals of police departments, where data about people committing crimes are recorded. It is important to note that some of the numbers mentioned this these usage scenarios might change if the respective data owners update the datasets. 

%\subsection{Finding disclosure risk: privacy auditor's perspective (T1a, T2, T3)}
Our collaborator began by choosing the Albany Police Department\cite{AlbanyPolice:online} and observed $6$ individual-level datasets on the dataset joinability view~(Figure~\ref{figs:case_study}a) (\textbf{T1}). He decided to analyze all the possible combinations of these datasets using the projection plot. Datasets \textit{APD Arrests Dataset by Neighborhood} and \textit{APD Arrests Datasets by Patrol Zone} had the highest risk score and shared a common unique identifier, namely \textit{arrestid} ~(Figure~\ref{figs:case_study}b) (\textbf{T4}). This dataset pair had the highest risk score since they shared $16$ joining attributes, including $2$ privacy-related attributes. Since \textit{arrestid} had the highest entropy among the other attributes, our collaborator decided to join these datasets based on \textit{arrestid} and observed that there may be $1607$ common records, i.e., $1607$ individuals may be present in both the datasets and new information may be disclosed by joining them (\textbf{T5}). For example, \textit{arrestid} APD*$210001493$ mentioned the arrest of a 21 year old white female in both the datasets. On closer analysis, he observed that these two are almost similar datasets, and the attributes \textit{neighborhood} and \textit{patrolzone} can be disclosed by joining them, leading to potential leakage of sensitive information. Our collaborator appreciated the triage capability of PRIVEE and commented:  ``these visualizations are helping people to quickly identify what they would like to focus on".

He followed this with analysis of the next pair of datasets, \textit{APD LEAD Dataset} and \textit{APD Arrests Dataset by Patrol Zone} and observed that they have common quasi-identifiers like \textit{race}, \textit{age} and \textit{sex}~Figure~\ref{figs:case_study}b). He then joined these datasets using these quasi-identifiers but found no common records, concluding that these datasets can be combined safely without actual, record-level disclosure (\textbf{T5}). 

He repeated this operation for another pair of datasets \textit{APD Arrests Dataset by Neighborhood} and \textit{APD Field Interview Cards Dataset by Neighborhood} by adding the location attribute \textit{neighborhoodxy}~(Figure~\ref{figs:case_study}b) (\textbf{T2}). He observed $887$ common records, implying that these individuals may be identified through these datasets who were stopped for field interview and later arrested by the police. He observed that the latter dataset does not provide any information about the reason for the field interview. But, joining this with the former dataset shows that a $28$-year old white male was interviewed in the Washington Park neighborhood at $09$:$08$ hrs on $1$\textsuperscript{st} December, $2020$ and was later arrested for trespassing on enclosed property at $12$:$32$ hrs (arrestid: APD*$200001760$). He found similar examples by joining the datasets \textit{APD Field Interview Cards Dataset by Neighborhood} and \textit{APD Traffic Citations by Neighborhood} ~(Figure~\ref{figs:case_study}b), where an individual of the the same age and gender received a citation on the same date and at the same location at $2$:$48$ am, just $3$ minutes after the incident from the first dataset~(see the two arrows in Fig \ref{figs:case_study}d)(\textbf{T5}). 

In his role as a privacy auditor, our collaborator flagged these datasets for record-level disclosure of sensitive information, an outcome of PRIVEE that can be used by data custodians for making decisions about applying anonymization methods for minimizing the disclosure risks. Our collaborator observed that he had not seen a tool with similar capabilities for interactive risk calibration and triage, and  commented: "\textit{this is a great visual tool to explore privacy risks of open data, with the ability to visualize privacy risk and see matches across datasets in a dynamic manner}".
%"This is very useful because it gives you direct visualization of what is there in the these datasets and the extent to which it can potentially lead to privacy breaches."

%"The visualization are helping people to quickly identify what they would like to focus on"

 

% \section{Case Study}



% In this section, we discuss a case study we developed using our tool \textit{PRIVEE} in conjunction with a domain expert who is also a co-author of this paper. Their expertise is in information privacy and secure computation technologies. \aritra{who is this expert what is his background and experience, is he a co-author?)}It is important to note that some of the numbers mentioned this these usage scenarios may change if the datasets are updated by the respective data owners.

% %\subsection{Finding disclosure risk: privacy auditor's perspective (T1a, T2, T3)}


 
% Police datasets can potentially damage an individual's social life if their sensitive information is disclosed. Amy, an independent privacy auditor, wants to find out if there are any possible disclosure risk with the datasets published in the open data portals of police departments. She selects the data portal for Albany Police Department\cite{AlbanyPolice:online} in \textit{PRIVEE} and observes $6$ individual-level datasets on the dataset joinability view (see Fig \ref{figs:scenario1}a) \textbf{(T1a)}. She decides to analyze all the possible combinations of these datasets by selecting all the dots in the projection plot. This shows all the possible dataset combinations along with their joining attributes but sorted according to their risk scores (see Fig \ref{figs:scenario1}b) (refer Section \ref{section:risk_score_calculation}) for detailed description). She observes that the datasets \textit{APD Arrests Dataset by Neighborhood} and \textit{APD Arrests Datasets by Patrol Zone} have the highest risk score and share a common unique identifier, namely \textit{arrestid} (\textbf{T2}). This dataset pair has the highest risk score since they share $16$ joining attributes, including $2$ privacy-related attributes (refer Section \ref{section:risk_score_calculation} for detailed calculation). Since \textit{arrestid} has the highest entropy among the other attributes, Amy decides to join these datasets based on \textit{arrestid} and observes that there may be $1607$ common records, i.e., $1607$ individuals may be present in both the datasets and new information may be disclosed by joining them (see Fig \ref{figs:scenario1}c) (\textbf{T3}). For example, \textit{arrestid} APD*$210001493$ mentions the arrest of a 21 year old white female in both the datasets. On closer analysis, she observes that these two are almost similar datasets, the attributes \textit{neighborhood} and \textit{patrolzone} can be disclosed by joining these datasets. This is an example of attribute disclosure using datasets from open data portals.

% Now she analyzes the next pair of datasets \textit{APD LEAD Dataset} and \textit{APD Arrests Dataset by Patrol Zone} and observes that they have common quasi-identifiers like \textit{race}, \textit{age} and \textit{sex} (see Fig \ref{figs:scenario1}b) (\textbf{T2}). Amy tries to join these datasets using these quasi-identifiers but finds that there are no common records, thus implying that these datasets can be combined safely on these quasi-identifiers (\textbf{T3}). She also repeats this same procedure for the next pair of datasets \textit{APD Arrests Dataset by Neighborhood} and \textit{APD LEAD Dataset} and observes that there are no common records between them, hence derives the same conclusion (see Fig \ref{figs:scenario1}b) (\textbf{T2},\textbf{T3}). She performs this operation one more time for the next pair of datasets \textit{APD Arrests Dataset by Neighborhood} and \textit{APD Field Interview Cards Dataset by Neighborhood} and also adds the location attribute \textit{neighborhoodxy} (see Fig \ref{figs:scenario1}b) (\textbf{T2}). She observes $887$ common records, which implies that these individuals may be identified through these datasets who were stopped for field interview and later arrested by the police. She observes that though the later dataset does not provide any information about the reason for the field interview, joining this with the former dataset shows that a $28$-year old white male was interviewed in the Washington Park neighborhood at $09$:$08$ hrs on $1$\textsuperscript{st} December, $2020$ and was later arrested for trespassing on enclosed property at $12$:$32$ hrs (arrestid: APD*$200001760$). This is an example of disclosure using quasi-identifiers present in open datasets (\textbf{T3}). She found more such examples by joining the datasets \textit{APD Arrests Dataset by Patrol Zone} and \textit{APD Field Interview Cards Dataset by Neighborhood}  where a $26$-year old black female was interviewed at $11$:$23$ hrs on $11$\textsuperscript{th} December, $2020$ and was later arrested at $21$:$25$ hrs for "assault with intent to cause physical injury" (arrestid: APD*$200001826$) (\textbf{T3}). Next, she joined the datasets \textit{APD Field Interview Cards Dataset by Neighborhood} and \textit{APD Traffic Citations by Neighborhood} on the attributes \textit{age}, \textit{sex}, \textit{neighborhoodxy}and  \textit{date} and observed $4$ common records between them (see Fig \ref{figs:scenario1}d) (\textbf{T2}). 




% She observed that $23$-year old male was stopped for field interview on $23$\textsuperscript{rd} January, $2021$ at $2$:$45$ am and since field interviews are normal routine stop and search activities by the police, this may seem a regular incident, but the other dataset informed her that an individual of the same same age and gender received a citation on the same date and at the same location at $2$:$48$ am, just $3$ minutes after the incident from the first dataset (see the two arrows in Fig \ref{figs:scenario1}d). Since these both records seem to belong to the same person, this is a possible identity disclosure and it was discovered using a combination of date and quasi-identifiers like location coordinates, age and gender (\textbf{T3}).

% \begin{comment}

% As a domain expert, Amy believed that this kind of disclosures may be present in other police data portals too. Hence, she selected the Fort Lauderdale Police Open Data Portal\cite{FortLauderdaleOpenData:online} and selected all the 5 datasets for analysis. 
% %She observed that the datasets Adult Arrests and Arrests have the highest risk score and also share unique identifiers like incidentid and caseid. She joined these datasets on these unique identifiers and other quasi-identifiers like race, age and sex, and observed 27479 common records. This implies that sensitive information about 27479 individuals may be compromised by joining these datasets (not loaded on interface). She also observed that the next pair of datasets Arrests and Juvenile Arrests also share the unique identifiers like incidentid and caseid and observed 5180 common records, i.e., 5180 individuals may be identified by joining these datasets and their sensitive information can be compromised.<insert example; interface does not show all of the lines>
% She joined datasets \textit{Adult Arrests} and \textit{Juvenile Arrests} based on the unique identifiers \textit{incidentid} and \textit{caseid} and observed $347$ common records. Though adult arrests and juvenile arrests should not have any common records as they serve completely different age groups, Amy observed that for the incident id $341803044797$ and caseid $341803044797$, the Adult Arrests dataset lists the age as $21$ while the Juvenile Arrests dataset lists the age as $15$. This implies that two people, age $15$ and $21$ were involved in larceny on $20$\textsuperscript{th} March, $2018$ with the exact charge being "LARC-GRAND THEFT 300 LESS THAN 5K DOLS".  More sensitive information like this can also be observed in other common records where the \textit{incidentid} and \textit{caseid} are $341807108870$ and it discloses the fact that two people, aged $17$ and $21$, were involved in a theft of motor vehicle (VEH THEFT-GRAND THEFT OF MOTOR VEHICLE) on $8$\textsuperscript{th} of July, $2018$. She also joins the dataset pair \textit{Arrest} and \textit{Citations} on the unique identifier \textit{case\_id} and observes $2760$ common records. For example, a $28$ year old black male was arrested for larceny on $26$\textsuperscript{th} September $2021$ at NW $10$\textsuperscript{th} Ave, was also cited for disobeying stop/yield sign and driving while license is suspended at NW $9$\textsuperscript{th} Street, around $3$ miles away from the arrest location(case\_id: $342109159680$). Other dataset pairs like \textit{Citations} and \textit{Juvenile Arrests} have $90$ common records when joined on the unique identifier \textit{case\_id}, where a $17$-year old white male was first charged with disobeying red light and was later arrested for possession of cannabis over $20$ grams on $4$\textsuperscript{th} August, $2015$, both at N Federal Hwy, Fort Lauderdale.
% \end{comment}



% PRIVEE helped Amy rapidly implement the attack scenario with joinable datasets in order to find disclosure risks (see Section\ref{section:attack_scenario1}). Thus, she concluded that since there are several possible disclosures by linking the datasets available through the open data portal of this police department, she would recommend to the police administrators that this portal is thoroughly analyzed for further disclosures before releasing any new datasets.


% \begin{comment}

% \subsection{Finding disclosure risk: data custodian's perspective (T1a, T2, T3)} \label{section:scenario2}
% \begin{figure*}
% \begin{center}
% \includegraphics[width=\textwidth]{figures/scenario2.pdf}
% \vspace{-4mm}
%  \caption{\label{figs:scenario2}\textbf{Disclosure risk: data custodian perspective} (a) The wordcloud for the New Orleans police datasets shows victimage as a frequent attribute, hence user select victimage along with other similar attributes (b) Joins two datasets on these attributes along with the location attribute (c) Though the addresses are partially masked, it can be observed that a $22$ year-old black male was charged with attempted armed robbery and attempted simple robbery against a $27$ year-old at the same location on different dates. (Section \ref{section:scenario2}) }
% \end{center}
% \vspace{-6mm}
% \end{figure*}
% \kaustav{Tasks are similar to the first usage scenario but in this scenario, the user updates the privacy related attributes based on what he sees in the wordcloud}
% Kabir, a data custodian with the police department of the City of New Orleans is tasked with the release of the Electronic Police Report for the year $2021$. He wishes to know if there could be any disclosure risk by using the electronic police reports from the previous years. In our interface \textit{PRIVEE}, Kabir selects the open data portal of New Orleans and loads all the available datasets\cite{NewOrleans:online}. He observes from the wordcloud that the attribute \textit{victim\_age} has a higher frequency, hence selects this attribute along with other similar attributes like \textit{offender\_age}, \textit{offender\_gender}, \textit{victim\_gender}, \textit{victim\_race} and \textit{offender\_race} as the privacy-related attributes (Figure \ref{figs:scenario2}a) (\textbf{T1a}).





% Now, he selects all these datasets and analyzes all the possible combinations of these datasets in the Risk Explanation View (\textbf{T2}). Since the police electronic reports across all the years have similar attributes, he started with the datasets \textit{Electronic Police Report 2015} and \textit{Electronic Police Report 2016} and joined them on his previously-selected privacy-related attributes along with the attribute \textit{location} (see Figure \ref{figs:scenario2}b) (\textbf{T2}). At this point, Kabir made an interesting observation that though the addresses used in these datasets are partially masked (see the arrow in Figure \ref{figs:scenario2}c), there are $21$ common records when joined on these attributes. For example, a $22$ year old Black Male was charged with "ATTEMPTED ARMED ROBBERY (GUN)" against a $27$ year old White Male at 6XX Tchoupitoulas St on 2015-07-13 at 01:00 hrs and again on 2016-04-30 at 03:00 hrs with "ATTEMPT - SIMPLE ROBBERY" (see Figure \ref{figs:scenario2}c). Kabir notes this as an example of identity disclosure (\textbf{T3}).



% Next, he joins the datasets \textit{Electronic Police Report 2016} and \textit{Electronic Police Report 2017} on the same attributes and to his surprise, finds $26$ common records despite the fact that the addresses are partially masked (\textbf{T2}, \textbf{T3}). For example, a $25$ year old Black Male was charged with "VIOLATIONS OF PROTECTIVE ORDERS" against a $23$ year old Black Female at 6XX Canal St on 2016-12-10 at 12:29 hrs and again on 2017-11-27 at 02:18 hrs with "DOMESTIC ABUSE BATTERY". He again notes this an example of identity disclosure (\textbf{T3}).

% Next, he joins the datasets \textit{Electronic Police Report 2017} and \textit{Electronic Police Report 2018} on the same attributes and again finds $43$ common records (\textbf{T2}, \textbf{T3}). For example, a $41$ year old Black Male was charged with "SHOPLIFTING", witnessed by a $32$ year old Black Female at 82XX Earhart Bd on 2017-06-06 at 19:50 hrs and again on 2017-11-27 at 02:18 hrs. A similar incident was reported at the same location by the offender and witness of the same attributes on 2018-02-20 at 12:26 hrs (\textbf{T3}). Thus, Kabir concludes that there may be disclosure risk using the previous years' police report datasets, hence those risks need to be carefully analyzed before releasing a new police report dataset.

% \end{comment}



==> sections/system_architecture_and_design.tex <==
\section{System Implementation}
PRIVEE has been built using Python and Javascript. The front-end designs have been constructed using Javascript frameworks React.js and D3.js . React.js helped in creating and maintaining the front-end server while D3.js helped in designing the visualizations. The Flask's Python library was used to create an API which responds to different requests and calculations based on the different parameters passed through the interface's front-end. This helps us in responding to user inputs and make the PRIVEE's interface more dynamic.
